Reconstructing Missing EHRs Using Time-Aware Within- and Cross-Visit Information for Septic Shock Early Prediction

Real-world Electronic Health Records (EHRs) are often plagued by a high rate of missing data. In our EHRs, for example, the missing rates can be as high as 90% for some features, with an average missing rate of around 70% across all features. We propose a Time-Aware Dual-Cross-Visit missing value imputation method, named TA-DualCV, which spontaneously leverages multivariate dependencies across features and longitudinal dependencies both within- and cross-visit to maximize the information extracted from limited observable records in EHRs. Specifically, TA-DualCV captures the latent structure of missing patterns across measurements of different features and it also considers the time continuity and capture the latent temporal missing patterns based on both time-steps and irregular time-intervals. TA-DualCV is evaluated using three large real-world EHRs on two types of tasks: an unsupervised imputation task by varying mask rates up to 90% and a supervised 24-hour early prediction of septic shock using Long Short-Term Memory (LSTM). Our results show that TA-DualCV performs significantly better than all of the existing state-of-the-art imputation baselines, such as DETROIT and TAME, on both types of tasks.

==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/Task1.tex <==
\label{sec:task1}


% \begin{table}[]
% \caption{Missing rates of overall 22 features in CCHS, Mayo, and MIMIC-III. }
% \label{tab:mssingrate}
% \begin{threeparttable}
% \begin{tabularx}{\columnwidth}{cccc|ccc}
% \hline
% \multicolumn{1}{c|}{\multirow{Feature}} & \multicolumn{3}{c|}{Cross-Visit} & \multicolumn{3}{c}{Within-Visit} \\
% \multicolumn{1}{c|}{}                    & MIMIC     & CCHS            & Mayo           &MIMIC           & CCHS     & Mayo      \\ \hline
% \multicolumn{1}{c|}{CI}             & 26\%                &      -           &   99\%      & 26\%        &   -       &  98\%  \\
% \multicolumn{1}{c|}{K}                     & 21\%               &      -           &         99\%        & 20\%     &      -           &    98\%      \\
% \multicolumn{1}{c|}{HCO3}                   & 27\%                   &       -          &     -     & 27\%         &    -      &   -  \\ 
% \multicolumn{1}{c|}{Na}            & 24\%                       &      -           &  99\%   & 24\%          &       -   &   98\% \\
% \multicolumn{1}{c|}{Hct}                 & 18\%                      &        -         &       -          & 19\%          &    -             &   -       \\
% \multicolumn{1}{c|}{Hb}             & 30\%                     &     -            &       99\%       & 30\%
% &    -      & 98\%  \\
% \multicolumn{1}{c|}{MCV}            & 31\%              &       -         &   99\%  & 31\%          &     -     &  99\% \\
% \multicolumn{1}{c|}{PLT}           & 28\%                      &     93\%       &  99\%   & 28\%           &  93\%   &  99\%  \\
% \multicolumn{1}{c|}{WBC}            & 30\%                      &     94\%       &   99\%  & 30\%          &  93\%   &  99\%  \\
% \multicolumn{1}{c|}{RDW}                  & 31\%                      &      -         &    -     & 30\%          &     -     &  -  \\ 
% \multicolumn{1}{c|}{BUN}           & 26\%                      &    93\%       &   99\%  & 25\%          &  93\%   & 98\%  \\
% \multicolumn{1}{c|}{Cr}           & 25\%                       &     93\%       &  99\%   & 25\%          &  93\%    &   99\% \\
% \multicolumn{1}{c|}{GLC}            & 30\%                      &       -          &  97\%   & 30\%          &      -   &  96\% \\
% \multicolumn{1}{c|}{Temp}           & 97\%                     & 81\%           & 91\%           & 95\%          & 82\%           & 88\%          \\
% \multicolumn{1}{c|}{RespRate}           & 45\%                 & 63\%          & 49\%           & 61\%          & 65\%           & 54\%          \\
% \multicolumn{1}{c|}{HeartRate}           & 44\%                & 61\%           & 54\%           & 61\%           & 64\%           & 55\%         \\

% \multicolumn{1}{c|}{FiO2}           & 84\%                     & 85\%           & 94\%           & 96\%          & 84\%           & 91\%          \\

% \multicolumn{1}{c|}{PulseOx}           & 45\%                 & 64\%           & 34\%            & 62\%        & 68\%           & 40\%          \\
% \multicolumn{1}{c|}{OFlow}           & 94\%                    & 78\%           & 97\%            & 94\%         & 87\%           & 92\%          \\
% \multicolumn{1}{c|}{DBP}           & 33\%                      & 72\%           & 63\%           & 25\%          & 82\%           & 64\%          \\ 
% \multicolumn{1}{c|}{SBP}           & 33\%                      & 72\%           & 63\%           & 25\%          & 72\%           & 64\%          \\
% \multicolumn{1}{c|}{MAP}           & 33\%                      & 77\%           & 63\%            & 25\%         & 77\%           & 68\%          \\\hline
% \multicolumn{1}{c|}{Median}           & 39\%      & 93\%           & 99\%          & 29\%          & 93\%           & 98\%           \\ 
% \multicolumn{1}{c|}{Mean}           & 38\%      & 88\%           & 86\%           & 40\%          & 89\%           & 86\%          \\ \hline
% \end{tabularx}
% \begin{tablenotes}
%       \scriptsize
%       \item - The ``-'' in table means the feature is not contained in the dataset.
%       \item - The median/mean refers to the median/average missing rate of the \emph{selected features}, which can be different from the median/average missing rate across all features within the EHRs.
%     \end{tablenotes}
% \end{threeparttable}
% \end{table}

\begin{table}[]
\caption{Missing rates of overall 22 features in CCHS, Mayo, and MIMIC-III. }
\label{tab:mssingrate}
\begin{threeparttable}
\begin{tabularx}{\columnwidth}{cccc|ccc}
\hline
\multicolumn{1}{c|}{Feature} & \multicolumn{3}{c|}{Cross-Visit} & \multicolumn{3}{c}{Within-Visit} \\
\multicolumn{1}{c|}{}                    & MIMIC     & CCHS            & Mayo           &MIMIC           & CCHS     & Mayo      \\ \hline
\multicolumn{1}{c|}{CI}             & 26\%                &                 &         & 26\%        &          &    \\
\multicolumn{1}{c|}{K}                     & 21\%               &                 &                 & 20\%     &                 &          \\
\multicolumn{1}{c|}{HCO3}                   & 27\%                   &                 &          & 27\%         &          &     \\ 
\multicolumn{1}{c|}{Na}            & 24\%                       &                 &     & 24\%          &          &    \\
\multicolumn{1}{c|}{Hct}                 & 18\%                      &                 &                 & 19\%          &                 &          \\
\multicolumn{1}{c|}{Hb}             & 30\%                     &                 &              & 30\%
&          &   \\
\multicolumn{1}{c|}{MCV}            & 31\%              &                &     & 31\%          &          &   \\
\multicolumn{1}{c|}{PLT}           & 28\%                      &            &     & 28\%           &     &    \\
\multicolumn{1}{c|}{WBC}            & 30\%                      &            &     & 30\%          &     &    \\
\multicolumn{1}{c|}{RDW}                  & 31\%                      &               &         & 30\%          &          &    \\ 
\multicolumn{1}{c|}{BUN}           & 26\%                      &            &     & 25\%          &     &   \\
\multicolumn{1}{c|}{Cr}           & 25\%                       &            &     & 25\%          &     &    \\
\multicolumn{1}{c|}{GLC}            & 30\%                      &                 &     & 30\%          &         &   \\ \hline
\multicolumn{1}{c|}{Temp}           & 97\%                     & 81\%           & 91\%           & 95\%          & 82\%           & 88\%          \\
\multicolumn{1}{c|}{RespRate}           & 45\%                 & 63\%          & 49\%           & 61\%          & 65\%           & 54\%          \\
\multicolumn{1}{c|}{HeartRate}           & 44\%                & 61\%           & 54\%           & 61\%           & 64\%           & 55\%         \\

\multicolumn{1}{c|}{FiO2}           & 84\%                     & 85\%           & 94\%           & 96\%          & 84\%           & 91\%          \\

\multicolumn{1}{c|}{PulseOx}           & 45\%                 & 64\%           & 34\%            & 62\%        & 68\%           & 40\%          \\
\multicolumn{1}{c|}{OFlow}           & 94\%                    & 78\%           & 97\%            & 94\%         & 87\%           & 92\%          \\
\multicolumn{1}{c|}{DBP}           & 33\%                      & 72\%           & 63\%           & 25\%          & 82\%           & 64\%          \\ 
\multicolumn{1}{c|}{SBP}           & 33\%                      & 72\%           & 63\%           & 25\%          & 72\%           & 64\%          \\
\multicolumn{1}{c|}{MAP}           & 33\%                      & 77\%           & 63\%            & 25\%         & 77\%           & 68\%          \\\hline
\multicolumn{1}{c|}{Median}           & 31\%      & 72\%           & 63\%          & 29\%          & 77\%           & 64\%           \\ 
\multicolumn{1}{c|}{Mean}           & 39\%      & 73\%           & 68\%           & 40\%          & 76\%           & 68\%          \\ \hline
\end{tabularx}
\begin{tablenotes}
      \scriptsize
      \item - The median/mean refers to the median/average missing rate of the \emph{selected features}, which can be different from the median/average missing rate across all features.
    \end{tablenotes}
\end{threeparttable}
\end{table}



% \begin{table}[]
% \caption{Missing rates of overall 22 features in CCHS, Mayo, and MIMIC-III. }
% \label{tab:mssingrate}
% \begin{threeparttable}
% \begin{tabularx}{\columnwidth}{cccc|ccc}
% \hline
% \multicolumn{1}{c|}{\multirow{Feature}} & \multicolumn{3}{c|}{Cross-Visit} & \multicolumn{3}{c}{Within-Visit} \\
% \multicolumn{1}{c|}{}                    & MIMIC     & CCHS            & Mayo           &MIMIC           & CCHS     & Mayo      \\ \hline
% \multicolumn{1}{c|}{Temp}           & 97\%                     & 81\%           & 91\%           & 95\%          & 82\%           & 88\%          \\
% \multicolumn{1}{c|}{RespRate}           & 45\%                 & 63\%          & 49\%           & 61\%          & 65\%           & 54\%          \\
% \multicolumn{1}{c|}{HeartRate}           & 44\%                & 61\%           & 54\%           & 61\%           & 64\%           & 55\%         \\

% \multicolumn{1}{c|}{FiO2}           & 84\%                     & 85\%           & 94\%           & 96\%          & 84\%           & 91\%          \\

% \multicolumn{1}{c|}{PulseOx}           & 45\%                 & 64\%           & 44\%            & 62\%        & 68\%           & 40\%          \\
% \multicolumn{1}{c|}{OFlow}           & 94\%                    & 78\%           & 97\%            & 94\%         & 87\%           & 92\%          \\
% \multicolumn{1}{c|}{DBP}           & 33\%                      & 72\%           & 63\%           & 25\%          & 82\%           & 64\%          \\ 
% \multicolumn{1}{c|}{SBP}           & 33\%                      & 72\%           & 63\%           & 25\%          & 72\%           & 64\%          \\
% \multicolumn{1}{c|}{MAP}           & 33\%                      & 77\%           & 63\%            & 25\%         & 77\%           & 68\%          \\
% \multicolumn{1}{c|}{PLT}           & 28\%                      &     93\%       &  99\%   & 28\%           &  93\%   &  99\%  \\
% \multicolumn{1}{c|}{WBC}            & 30\%                      &     94\%       &   99\%  & 30\%          &  93\%   &  99\%  \\
% \multicolumn{1}{c|}{BUN}           & 26\%                      &    93\%       &   99\%  & 25\%          &  93\%   & 98\%  \\
% \multicolumn{1}{c|}{Cr}           & 25\%                       &     93\%       &  99\%   & 25\%          &  93\%    &   99\% \\
% \multicolumn{1}{c|}{CI}             & 26\%                &      -           &   99\%      & 26\%        &   -       &  98\%  \\
% \multicolumn{1}{c|}{K}                     & 21\%               &      -           &         99\%        & 20\%     &      -           &    98\%      \\
% \multicolumn{1}{c|}{Na}            & 24\%                       &      -           &  99\%   & 24\%          &       -   &   98\% \\
% \multicolumn{1}{c|}{Hb}             & 30\%                     &     -            &       99\%       & 30\%
% &    -      & 98\%  \\
% \multicolumn{1}{c|}{MCV}            & 31\%              &       -         &   99\%  & 31\%          &     -     &  99\% \\
% \multicolumn{1}{c|}{GLC}            & 30\%                      &       -          &  97\%   & 30\%          &      -   &  96\% \\
% \multicolumn{1}{c|}{HCO3}                   & 27\%                   &       -          &     -     & 27\%         &    -      &   -  \\
% \multicolumn{1}{c|}{Hct}                 & 18\%                      &        -         &       -          & 19\%          &    -             &   -       \\
% \multicolumn{1}{c|}{RDW}                  & 31\%                      &      -         &    -     & 30\%          &     -     &  -  \\ 
% \hline
% \multicolumn{1}{c|}{Median}           & 31\%      & 78\%           & 97\%          & 29\%          & 82\%           & 96\%           \\ 
% \multicolumn{1}{c|}{Mean}           & 39\%      & 79\%           & 85\%           & 40\%          & 81\%           & 84\%          \\ \hline
% \end{tabularx}
% \begin{tablenotes}
%       \scriptsize
%       \item - The ``-'' in table means the feature is not contained in the dataset.
%       \item - Features are sorted in descending order according to the numbers of datasets containing the features. 
%       \item - The median/mean refers to the median/average missing rate of the \emph{selected features}, which can be different from the median/average missing rate across all features within the EHRs.
%     \end{tablenotes}
% \end{threeparttable}
% \end{table}



% \begin{table*}[!htbp]
% \small
% \centering
% \caption{Imputation results (in nRMSE) with various masking rates on 13 lab analytes features of MIMIC-III.}
% \label{tab:nrmse}
% \begin{tabular}{c|cc|cccc|c}
% \hline
% Mask Rate & MeanFill & ECF   & MICE  & 3D-MICE & DETROIT & TAME  & TA-DualCV         \\ \hline
% 90\%      & 3.373    & \textbf{0.278} & 0.296 & \textbf{0.260}   & 2.380   & 0.424 & \textbf{0.227}* \\
% 80\%      & 3.037    & \textbf{0.275} & 0.293 & \textbf{0.263}   & 6.616   & 0.491 & \textbf{0.228}* \\
% 70\%      & 2.088    & \textbf{0.264} & 0.284 & \textbf{0.247}   & 5.097   & 0.346 & \textbf{0.225}* \\
% 60\%      & 1.540    & \textbf{0.257} & 0.276 & \textbf{0.236}   & 2.581   & 0.291 & \textbf{0.222}* \\ \hline
% \end{tabular}
% \end{table*}

\input{sections/table/nrmse}

% \begin{table*}[!htbp]
% \small
% \centering
% \caption{Imputation results (in nRMSE) on 9 sepsis-related features of CCHS, Mayo, and MIMIC-III.}
% \label{tab:nrmse-sepsis}
% \begin{tabular}{c|cc|cccc|c}
% \hline
% Dataset   & MeanFill & ECF   & MICE  & 3D-MICE & DETROIT & TAME  & TA-DualCV         \\ \hline
% CCHS      & \textbf{2.285}    & 2.785 & 1.043 & \textbf{0.984}   & N/A     & 0.995 & \textbf{0.285}* \\
% Mayo      & 7.109    & \textbf{6.942} & 3.617 & \textbf{3.592}   & N/A     & 4.806 & \textbf{0.305}* \\
% MIMIC-III & 1.455    & \textbf{1.231} & 0.829 & \textbf{0.823}   & N/A     & 0.914 & \textbf{0.289}* \\ \hline
% \end{tabular}
% \end{table*}

\begin{table*}[!htbp]
% \scriptsize
\small
% \fontsize{3}{6}\selectfont
\centering
\caption{Imputation results (nRMSE) with classic masking rates on 9 sepsis-related features of CCHS, Mayo, and MIMIC-III.}
\label{tab:nrmse-sepsis}
% \resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{lcccccccccc}
\hline
\multicolumn{1}{l|}{Model} & \multicolumn{1}{l}{Temp} & \multicolumn{1}{l}{RespRate} & \multicolumn{1}{l}{HeartRate} & \multicolumn{1}{l}{FiO2} & \multicolumn{1}{l}{PulseOx} & \multicolumn{1}{l}{OFlow} & \multicolumn{1}{l}{DBP} & \multicolumn{1}{l}{SBP} & \multicolumn{1}{l}{MAP} & \multicolumn{1}{l}{Average} \\ \hline

\multicolumn{11}{l}{\textbf{CCHS}}  \\ \hline
\multicolumn{1}{l|}{MeanFill} &  1.929 & 0.624 & 1.704 & \textbf{2.267} & \textbf{0.655} & \textbf{12.927} & \textbf{1.092} & \textbf{1.404} & \textbf{0.867} & 2.825  \\  
\multicolumn{1}{l|}{ECF}     & \textbf{1.872} & \textbf{0.564} & \textbf{1.498} & \textbf{2.267} & \textbf{0.655} & \textbf{12.927} & \textbf{1.092} & \textbf{1.404} & \textbf{0.867} & \textbf{2.785}\\ \cline{2-11} 
\multicolumn{1}{l|}{MICE}    & 1.224 & 0.644 & 0.744 & 0.391 & 0.572 & 0.557 & 2.564 & 1.644 & 1.268 & 1.043\\
\multicolumn{1}{l|}{3D-MICE} & 1.219 & 0.637 & \textbf{0.714} & \textbf{0.311} & \textbf{0.549} & \textbf{0.473} & 2.485 & 1.483 & \textbf{1.179} & \textbf{0.984} \\
\multicolumn{1}{l|}{TAME}    & \textbf{0.808} & \textbf{0.631} & 0.986 & 0.980 & 0.880 & 1.484 & \textbf{0.790} & \textbf{1.401} & 1.801 & 1.085\\ \hline

\multicolumn{1}{l|}{TA-DualCV$^{-C}$}     & 0.355 & \textbf{0.218}** & 0.487 & 0.343 & 0.374 & \textbf{0.236}** & 0.303 & 0.281 & 0.222 &  0.313 \\
\multicolumn{1}{l|}{TA-DualCV$^{-I}$} & 0.397 & 0.337 & 0.522 & 0.399 & 0.471 & 0.516 & 0.380 & 0.416 & 0.409 & 0.427 \\
\multicolumn{1}{l|}{TA-DualCV} & \textbf{0.314}** & 0.222 & \textbf{0.334}** & \textbf{0.303}** & \textbf{0.346}** & 0.295 & \textbf{0.272}** & \textbf{0.267}** & \textbf{0.211}** &  \textbf{0.285}** \\ \hline  



\multicolumn{11}{l}{\textbf{Mayo}}  \\ \hline
\multicolumn{1}{l|}{MeanFill}    & 0.710 & 0.680 & 1.998 & \textbf{45.391} & \textbf{0.684} & \textbf{5.217} & \textbf{0.880} & \textbf{1.310} & \textbf{1.662} & 7.109 \\  
\multicolumn{1}{l|}{ECF}     & \textbf{0.640} & \textbf{0.467} & \textbf{0.949} & \textbf{45.391} & \textbf{0.684} & \textbf{5.217} & \textbf{0.880} & \textbf{1.310} & \textbf{1.662} & \textbf{6.942} \\ \cline{2-11}
\multicolumn{1}{l|}{MICE}    & \textbf{0.812} & 0.460 & 0.716 & 24.445 & 0.645 & 0.435 & 0.652 & 0.775 & 0.780 & 3.617\\
\multicolumn{1}{l|}{3D-MICE}  & 0.820 & \textbf{0.452} & \textbf{0.716} & \textbf{24.445} & \textbf{0.546} & \textbf{0.427} & \textbf{0.549} & 0.778 & 0.779 & \textbf{3.592}\\
\multicolumn{1}{l|}{TAME}    & \textbf{0.812} & 1.526 & 1.101 & 31.405 & 0.955 & 1.329 & 0.587 & \textbf{0.730} & \textbf{0.743} & 4.806\\ \hline

\multicolumn{1}{l|}{TA-DualCV$^{-C}$}       & 0.677 & 0.397 & 0.542 & 0.528 & 0.469 & \textbf{0.246}** & 0.490 & 0.692 & 0.702 & 0.527         \\
\multicolumn{1}{l|}{TA-DualCV$^{-I}$} & 0.541 & 0.372 & 0.543 & 0.530 & 0.554 & 0.660 & 0.543 & 0.517 & 0.506 & 0.530 \\
\multicolumn{1}{l|}{TA-DualCV} &  \textbf{0.363}** & \textbf{0.276}** & \textbf{0.321}** & \textbf{0.329}** & \textbf{0.326}** & 0.310 & \textbf{0.316}** & \textbf{0.295}** & \textbf{0.209}** & \textbf{0.305}** \\ \hline  



\multicolumn{11}{l}{\textbf{MIMIC-III}}  \\ \hline
\multicolumn{1}{l|}{MeanFill}    & 1.094 & 0.780 & 4.273 & \textbf{0.847} & \textbf{0.946} & \textbf{1.286} & \textbf{1.400} & \textbf{1.345} & \textbf{1.122} & 1.455\\  
\multicolumn{1}{l|}{ECF}     & \textbf{0.375} & \textbf{0.587} & \textbf{3.171} & \textbf{0.847} & \textbf{0.946} & \textbf{1.286} & \textbf{1.400} & \textbf{1.345} & \textbf{1.122} & \textbf{1.231}\\ \cline{2-11}
\multicolumn{1}{l|}{MICE}    & 0.656 & 0.647 & 0.618 & 0.739 & 0.769 & 0.792 & 1.050 & 0.878 & 1.312 & 0.829\\
\multicolumn{1}{l|}{3D-MICE} & 0.607 & 0.642 & 0.684 & \textbf{0.712} & 0.759 & 0.729 & 1.076 & 0.895 & 1.305 & 0.823 \\
\multicolumn{1}{l|}{TAME}    & \textbf{0.287} & \textbf{0.291} & \textbf{0.253} & 0.747 & \textbf{0.246} & \textbf{0.451} & \textbf{0.140}** & \textbf{0.179} & \textbf{0.089}** & \textbf{0.297}\\ \hline

\multicolumn{1}{l|}{TA-DualCV$^{-C}$}     & \textbf{0.228}** & 0.380 & 0.400 & 0.431 & 0.291 & 0.319 & 0.213 & 0.209 & 0.288 & 0.293 \\
\multicolumn{1}{l|}{TA-DualCV$^{-I}$}  & 0.475 & 0.497 & 0.336 & 0.477 & 0.378 & 0.406 & 0.262 & 0.283 & 0.351 & 0.384 \\
\multicolumn{1}{l|}{TA-DualCV} & 0.240 & \textbf{0.278}** & \textbf{0.226}** & \textbf{0.333}** & \textbf{0.223}** & \textbf{0.306}** & \textbf{0.189} & \textbf{0.174}** & \textbf{0.228} & \textbf{0.244}** \\ \hline  
\end{tabular}
\begin{tablenotes}
      \small
      \item - For each block, the best approach is in \textbf{bold}; The best model across ALL is labeled with **.
      \item - DETROIT cannot produce results so we don't include it in the table.
    \end{tablenotes}
\end{threeparttable}
% }
\end{table*}



In this section, we first compare TA-DualCV with baselines in unsupervised learning tasks, imputation, by masking the observations with two commonly-used strategies separately: 

1) Following~\cite{miao2021generative},  we vary random mask rates on 13 general laboratory analyse features from  60\% up to 90\% of observed values using widely-used MIMIC-III so as to evaluate the performance of imputation methods when the missing rate is high and close to the general clinical data. 

2) Following~\cite{luo20183d}, we randomly mask one measurement per feature per visit using 9 sepsis-related features in EHRs from three healthcare systems, CCHS, Mayo, and MIMIC-III, to study the performance of imputation and to btain complete data for supervised learning tasks: septic shock early prediction. 


\noindent\textbf{Features} 22 features, including 13 lab analyte and 9 sepsis-related features, are investigated in this study. The 13 lab analyte features are commonly used in existing works \cite{luo20183d, xu2020multi, zhang2020predicting, yin2020identifying}: Chloride, Potassium, Bicarb, Sodium, Hematocrit, Hemoglobin, MCV, Platelet, WBC, RDW, BUN, Creatinine, and Glucose. We use short forms CI, K, HCO3, Na, Hct, Hb, MCV, PLT, WBC, RDW, BUN, Cr, GLC, respectively, to represent these features for simplicity. The 9 sepsis-related features \cite{yang2018time} are from four categories: 1) \textit{Vital Signs}: Temperature, RespiratoryRate, HeartRate; 2) \textit{Respiratory System}: FiO2, PulseOx; 3) \textit{Cardiovascular System}: DiastolicBP, SystolicBP, MAP; 4) \textit{Others}: OxygenFlow. %Missing rates of the features are shown in table \ref{tab:mssingrate}
%\footnote{For simplicity, we use abbreviations: CI, K, HCO3, Na, Hct, Hb, MCV, PLT, WBC, RDW, BUN, Cr, GLC, for 13 lab analyte features; Temp, RespRate, HeartRate, MAP, DBP, SBP, FiO2, PulseOx, OFlow, for 9 sepsis-related features.}

\subsection{Datasets}
\label{sec:imputation-data}
\begin{itemize}
    \item \textbf{MIMIC-III} \cite{johnson2016mimic}\footnote{Dataset is available at http://mimic.physionet.org.} contains admissions of adult patients (i.e., age $>$ 16) who are admitted to intensive care units (ICU) at a tertiary referral hospital between 2001 and 2012, corresponding to 53,423 visits containing $\sim$11 million events. % Moreover, sepsis patients are selected strictly following \cite{zhang2017lstm, yang2018time} which combines International Classification of Diseases, Ninth Revision, and the Third International Consensus Definitions for Sepsis and Septic Shock \cite{singer2016third}. Considering the imbalanced ratio between shock positive and negative visits, we further employ stratified random sampling on both positive and negative visits so that the final numbers of shock positive and negative visits are equal in each dataset. With the selected 9 sepsis-related features, 772 sepsis visits are obtained. The lengths of time series range from 1 to 923. The native missing rate across-visit is $38\%$ on average.     
    \item \textbf{Christiana Care Health System (CCHS)} contains visit records of adult patients (i.e., age $>$ 18) admitted to the Christiana Care hospital from July 2013 to December 2015, corresponding to 210,289 visits containing $\sim$9 million events. %In this work, 1,124 sepsis visits are obtained. The lengths of time series range from 1 to 827. The native missing rate across-visit is $88\%$ on average.
    \item \textbf{Mayo} contains visit records of adult patients (i.e., age $>$ 18) admitted to Mayo Clinic Hospital from July 2013 to December 2015, corresponding to 121,019 visits containing $\sim$52 million events. %In this work, 2,176 sepsis visits are obtained. The lengths of time series range from 1 to 4,863. The native missing rate across-visit is $86\%$ on average.
\end{itemize}

\subsubsection{Data Preprocessing for Imputation with Varied Masking Rates}
With the selected 13 lab analyte features, to provide sufficient data for evaluation with high masking rates and to meet the base implementing requirements of baselines such as those that need a sliding window, we apply exclusion criteria for data sampling in MIMIC-III: i) exclude visits that have less than 11 events; ii) exclude events if they contain more than half missing measurements. Thus, 19,693 visits containing 658,690 events are obtained from MIMIC-III. %The number of events across visits varies from 11 to 1191.


\begin{figure}[t]
\centerline{\includegraphics[scale=0.42]{sections/figure/sepsis-prediction.png}}
\caption{Illustration of septic shock early prediction setting.}
\label{fig:rightalign}
\end{figure}


\subsubsection{Ground Truth Labeling \& Data Preprocessing for Septic Shock}
\vspace{0.05in}
Supervised learning models depend heavily on the accurate label of the training set. However, acquiring the true label (i.e., septic shock and non-shock) can be challenging. Although diagnosis codes, such as International Classification of Diseases, Ninth Revision (ICD-9), are widely used for clinical labeling, solely relying on ICD-9 can be problematic as it has been proven to have limited reliability due to the fact that its coding practice is used mainly for administrative and billing purpose. Indeed, it has been widely argued that ICD-9 cannot be used for establishing reliable gold standards for various clinical conditions \cite{sepsis:ho, zhang2017lstm}. More importantly, ICD-9 cannot tell when septic shock occurs at event level, which is essential for our task. On the basis of the Third International Consensus Definitions for Sepsis and Septic Shock \cite{singer2016third}, our domain experts identified septic shock as any of the following conditions are met: 
\vspace{0.05in}
\begin{itemize}
\item Persistent hypertension as shown through two consecutive readings ($\le$ 30 minutes apart).
    \SubItem{Systolic Blood Pressure (SBP) $<$ 90 mmHg}
    \SubItem{Mean Arterial Pressure (MAP) $<$ 65 mmHg}
    \SubItem{Decrease in SBP $\geq$ 40 mmHg with an 8-hour period}
\item Any vasopressor administration. 
\end{itemize}
\vspace{0.05in}
When combing both ICD-9 and the domain experts' rules, we identify: i) 4,918 visits (2,459 shock positive visits and 2,459 negative visits) containing $\sim$1 million events from MIMIC-III. ii) 144,119 visits (2,963 shock positive visits and 141,156 negative visits) containing 795,314 events from CCHS. iii) 84,897 visits (3,499 shock positive visits and 81,398 negative visits) containing 7,612,360 events from Mayo. We are given all of a patient's EHRs until 24 hours before the septic shock onset (shock group) or end of the sequences (non-shock group), and supervised learning task is to use the complete data to predict whether or not the patient will develop septic shock exactly 24 hours later. To conduct this task, we \emph{right aligned} all the shock sequences by septic shock onset and all non-shock by the end of their sequences and include all the EHRs until 24 hours before the end of sequences (see Fig.~\ref{fig:rightalign}). Our \emph{prediction window} here is 24-hour window before the onset of septic shock or end of sequence. To simulate early prediction in practice, we exclude events in prediction window, accordingly the visits that contain no events in observation window are excluded for both imputation and septic shock prediction tasks. As a result, the final datasets have: i) 772 visits (386 shock positive visits and 386 negative visits) containing 37,246 events from MIMIC-III. Notably, MIMIC-III is ICU-specific and sepsis onset can present itself early, thus the number of remaining visits in MIMIC-III is relatively small after applying a 24-hour cut before the onset. ii) 2,842 visits (1,347 shock positive visits and 1,495 negative visits) containing 376,887 events from CCHS. iii) 6,836 visits (3,457 shock positive visits and 3,379 negative visits) containing 1,547,893 events from Mayo. Note that the labels are not used for imputation tasks, but only for septic shock prediction tasks in Section~\ref{sec:task2}.

% Notably, for nine sepsis-related features imputation, we don't apply strict exclusion criteria as the ones described in former imputation task with 13 lab features, because we would like to investigate imputation performance with native data characteristics, where missing rates can be relatively high and lengths of trajectories can be varied a lot.

\vspace{0.1in}
\subsubsection{Missing Data Analysis}
\vspace{0.05in}
Since different features are measured at different events, plenty of missing entries exist in EHRs. For instance, vital signs are generally measured every 8 hours, while lab values are measured every 24 hours. Hence there may not be available readings for lab results when a new event is created for vital signs. Table~\ref{tab:mssingrate} shows both cross-visit and within-visit missing rates of 22 features selected from the three datasets in our study. We also calculate median and mean value of cross-visit and within-visit missing rates across features. The missingness across visits within one medical system and across different medical systems can diff a lot.

% \subsection{Data Preprocessing}

% \textbf{In task 1}, we validate imputation methods in the context where a large range of mask rates occurs, i.e. $60\% - 90\%$, as the native missing rates of MIMIC-III are relatively low compared to general clinical data (e.g., CCHS). Also, to meet the base implementing requirements of baselines, we apply exclusion criteria for data sampling: i) exclude visits that have less than 11 events, and ii) exclude events if they contain more than half missing measurements. Our final data consists of $\sim$17 million events of 19,693 visits. The number of events across visits varies from 11 to 1191. Aside from the native missing values, we mask values with rates $60\% - 90\%$. Both native and masked values will be imputed to form the final complete data.

% \noindent\textbf{In task 2}, we validate imputation methods in the context where the complete data is needed as inputs to predict septic shock. Specifically, we preprocess the data by three steps as follows:

% \textit{Labeling}.
% The target population of datasets are patients with suspected infection, which is identified by the presence of antiviral, antibiotic, etc. To label our visits, we strictly follow domain experts' identification rule \cite{zhang2017lstm, yang2018time}, which is a combination of International Classification of Diseases, Ninth Revision (ICD-9), and the Third International Consensus Definitions for Sepsis and Septic Shock \cite{singer2016third}. The labels are only used for sampling to balance the sample size of shock positive and negative visits in prediction. 


% \textit{Aggregation}.
% As the sepsis-related features are mainly recorded on every $\sim$30 minutes, we aggregate them into 30 minutes window by taking median values on both features and elapsed time (e.g., minutes) from patients' arrival.


% \textit{Events Exclusion}.
% To simulate early prediction in practice, we constrain the data from start to the point when the prediction is supposed to make, by excluding events after the last event occurring 24-hour before the septic shock.

% After that, we employ a commonly-used method in existing imputation studies (i.e., randomly masking one measurement per feature within each visit \cite{luo20183d, xu2020multi, zhang2020predicting, yin2020identifying}) to mask a slight number of measurements for model training and validation.

% Considering the imbalanced ratio between shock positive and negative visits, we employ stratified random sampling on both positive and negative visits so that the final numbers of shock positive and negative visits are equal in each dataset. Finally, in CCHS, we get 1,124 visits. The number of events per visit ranges from 1 to 827. In Mayo, we include 2,176 visits. The number of events per visit ranges from 1 to 4,863. In MIMIC-III, we get 772 visits. The number of events per visit ranges from 1 to 923. Specifically, MIMIC-III is ICU-specific and onset can present early, thus the number of remaining visits is relatively smaller after applying a 24-hour cut before onset. We randomly split samples from both groups into the training, validation, and test sets, and impute both native and masked values to form final complete data.

% \noindent\textbf{Normalization.}
% We normalize the data by within-visit min-max such that all values are scaled to be within [0, 1] interval throughout events before imputation and de-normalize it to obtain final complete data and evaluation matrix. 


\subsection{Baselines}
\label{sec:imputation-baseline}

We compare TA-DualCV with six imputation approaches for comparison, which are originally designed towards either supervised or unsupervised learning tasks. \footnote{Note that Missing indicator (MI) is not included as a baseline in this task, as it only indicates whether a measurement is missing without imputation.}  \\
\textit{Approaches towards supervised learning tasks:}
\begin{itemize}
    \item \textbf{MeanFill} imputes missing values by mean values cross-visit on each feature.
    \item \textbf{Expert Carry Forward (ECF)} \cite{kim2018temporal} fills the missing values by the last value within a fixed-length window (i.e., 24 hours for lab analytes and 8 hours for vital signs). Then it fills the remaining with the mean value of the corresponding features. ECF is a strong method for both imputation and disease diagnosis in~\cite{kim2018temporal}. 
\end{itemize}
%ECF is a strong method for both clinical data imputation and prediction in existing work \cite{kim2018temporal}. 
\textit{Approaches towards unsupervised learning tasks:}

\textit{Non-NN-Based:}
\begin{itemize}
    \item \textbf{MICE} \cite{buuren2010mice} imputes missing values by capturing multivariate dependencies cross-visit.
    \item \textbf{3D-MICE} \cite{luo20183d} imputes missing values by integrating multivariate dependencies cross-visit and time-interval dependencies within-visit.
    \end{itemize}
    
\textit{NN-Based:}
\begin{itemize}
    \item \textbf{DETROIT} \cite{yan2019detroit} prefills missing values with means and impute missing values based on neural networks by leveraging multivariate and time-aware dependencies from observed values within a 5-length window. 
    \item \textbf{TAME} \cite{yin2020identifying} imputes missing values based on bidirectional RNNs and within-visit multi-modal embedding that takes data including demographics, diagnosis, medication, features, and time-intervals as inputs.     
\end{itemize}
% \textbf{CATSI} \cite{yin2020context} imputes missing values from a fusion layer by integrating multivariate and time-aware dependencies cross-visits. \\

% \textbf{TA-DualCV} is our proposed model for missing values imputation. 
To evaluate the performance of our proposed modules, we implement another two variant versions of TA-DualCV. 
\begin{itemize}
  \item \textbf{TA-DualCV$^{-C}$} removes DualCV but imputes based on within-visit time-aware information.
  \item\textbf{TA-DualCV$^{-I}$} removes within-visit time-aware augmentation that is used to augmenting results from DualCV. 
\end{itemize}


\subsection{Experimental Setup}
To obtain results of baselines, for ECF, we implement the code strictly following the instructions in the authors' paper. For MICE, we use R package \textit{mice} with 10 iterations. For 3D-MICE, DETROIT and TAME, we use the source code provided by the authors with their default parameter settings as suggested in~\cite{miao2021generative}. We implement our proposed work with R and Python. %All experiments are conducted on a machine with two 6-core Xeon E5-2620 CPUs $@2$ GHz and four NVIDIA TITAN Xp / 12GB RAM, running on CentOS 7.8 (64-bit). 
For parameters settings, we use 10 iteration with multiple chain equations. In compromising layer, we use $w_1=w_2=0.5$ for all experiments, to provide a general view of TA-DualCV's performance taking balanced efforts from both cross-visit and within-visit imputation in this study.  




\subsubsection{Evaluation Metric}
Following~\cite{luo20183d,yin2020identifying}, normalized root-mean-square error (nRMSE) is used to evaluate the imputation performance of the methods.
We evaluate the imputation performance of all methods on masked values by calculating a popular matrix, normalized root-mean-square error (nRMSE). nRMSE assigns large residuals with a disproportionately large effect, thus more sensitive to outliers \cite{pontius2008components}. 
nRMSE is widely adopted in clinical data imputation tasks that contain different scales of values \cite{luo20183d, yin2020identifying}. As normalization of RMSE has different calculations in different approaches. In this study, we used the common choice of range normalization as in~\cite{luo20183d}.

% The nRMSE of a feature $d\inD$ is calculated as:
% \begin{equation}
%     nRMSE_d = \sqrt{\frac{\sum_{i,t}(\frac{(\hat{Y}_{d,i,t} - Y_{d,i,t})}{max(Y_{d,i}) - min(Y_{d,i})})^2}{\mid T \mid}}
% \end{equation}

% \noindent where $i \in [1, N]$, $t \in \sum_i{X_{i,\cdot,d}^{imp}}$. $N$ is the total number of visits in the data, $T$ is a list of time points with missing values of feature $d$ for patient $i$. $\hat{Y}$ represents the estimated value while $Y$ represents the actual value.

\begin{figure}[t]
\centerline{\includegraphics[scale=0.3]{sections/figure/oxygenflow.png}}
\caption{Value distribution of OxygenFlow on CCHS, Mayo, and MIMIC-III. The blue-shaded area represents the density of the data. Blue-vertical lines represent the maximum, mean, and minimum values of the data.}
\label{fig:violindist}
\end{figure}




\subsection{Results}
\label{sec:imputation-result}

Table \ref{tab:nrmse}  compares the various approaches' average nRMSE of 13 general lab analytes features across different masking rates on MIMIC-III. The best approaches for each block is indicated in \textbf{bold}; the best approaches across all blocks is indicated by **. In approaches towards supervised learning tasks, ECF outperforms MeanFill at all masking rates and performance holds steady. For approaches towards unsupervised learning tasks, in non-NN-based approaches, 3D-MICE outperforms MICE at all masking rates. In NN-based approaches, TAME can outperform DETROIT when masking rate is as high as 90\%, while DETROIT outperforms TAME when masking rate is 60\%. The nRMSE of DETROIT is increased faster when masking rate increased. A possible reason is that DETROIT needs to prefill missing values, which can introduce more bias when masking rate is high. 3D-MICE achieves the best performance among four unsupervised learning imputation methods. To our surprise, DETROIT and TAME, especially DETROIT, perform worse than 3D-MICE. There is a possible reason that the datasets in our experiments are highly sparse across visits. DETROIT predicts missing values according to neighboring measurements, so it may be difficult to obtain reliable results when the data is highly sparse and even fails to provide results when the number of events is small (e.g., 1). TAME can take in multi-modal information including demographics, diagnosis, medication, and lab analytes, and it has achieved superior performance in its original settings using multi-modal inputs containing 29 features with 54\% average missing rate, as described in~\cite{yin2020identifying}. However, its performance can suffer when highly sparse 9 features are provided, as information is too limited to construct NN model. Finally, Table \ref{tab:nrmse} shows that TA-DualCV achieves the best performance in terms of average nRMSE across all masking rates on this task. 

%Specifically, TA-DualCV wins with the least nRMSE on all 13 features on 90\% and 80\% mask rates, and 11 features on 70\% mask rate. TA-DualCV is more capable with a high mask rate when it's close to missing rate in general clinical data, with an average of 0.227 nRMSE across features, which is 46\% better than state-of-the-art benchmarks TAME (i.e., 0.424), 90\% better than DETROIT (i.e., 2.380), and 13\% better than 3D-MICE (i.e., 0.260). More importantly, across all features, our proposed TA-DualCV is the least sensitive to the mask rate. Intuitively, TA-DualCV has a smaller range of nRMSE average nRMSE across mask rates. It indicates that TA-DualCV is the most robust to mask rates and features. %By calculating $\hat{V}_{IMDS}$, our proposed evaluation estimator (the lower, the more robust), we have 0.00016 for TA-DualCV, 6.79645 for DETROIT, 0.06978 for TAME, and 0.00019 for 3D-MICE. It indicates that TA-DualCV is the most robust to mask rates and features, which is identical to statistical trends in Table \ref{tab:nrmse}.  
On the CCHS, Mayo, and MIMIC-III datasets, Table \ref{tab:nrmse-sepsis}  provides the overall average nRMSE across nine sepsis-related features for the compared methods. Across all three medical systems, these approaches performances varied considerably. One explanation for this could be that the features are distributed differently in the three medical systems (e.g., OxygenFlow). ECF scores better than MeanFill across the three medical systems. 3D-MICE again performs well among four unsupervised learning imputation methods on CCHS and Mayo, while TAME performs well on MIMIC-III. Note that we were unable to make DETROIT converge to produce results. Moreover, 3D-MICE outperforms ECF across all three medical systems, and all methods perform better on CCHS and MIMIC-III than Mayo. Finally, Table \ref{tab:nrmse-sepsis} shows that TA-DualCV outperforms all baselines as it not only achieves the least overall nRMSE among all three medical systems but its performance is relatively stable. 

In summary, Table \ref{tab:nrmse} and Table \ref{tab:nrmse-sepsis}  show that TA-DualCV is capable of handling a diverse set of feature imputation tasks in both general and ICU-specific real-world medical systems when missing rate is high and achieving state-of-the-art performance. 

%Another reason is that the features can be divergently distributed across the three medical systems (e.g., OxygenFlow visualized in Figure~\ref{fig:violindist}), while both DETROIT and TAME are carefully designed towards ICU-specific medical system (e.g., MIMIC-III).
%Finally, Table \ref{tab:nrmse} shows that TA-DualCV achieves the best performance in terms of nRMSE across all mask rates. More importantly TA-DualCV has a minimal performance variation across different mask rates. It indicates that TA-DualCV can perform more stable to missing rates. 


%Interestingly, the recent methods, DETROIT and TAME, perform significantly worse than our method and can perform even worse than the benchmark MICE. A possible reason is that the datasets in our experiments are highly sparse across samples without external information such as demographics of patients. DETROIT directly predicts missing values based on latest measurements’ values, thus it can be hard to capture reliable information when the data is highly sparse and even failed to produce results when the number of events is very small (e.g., 1). TAME can take external information including demographics, diagnosis, and medications of patients as a part of model inputs as described in~\cite{yin2020identifying}, thus its performance can deteriorate when only measurements information is provided. Another reason is that the features can be divergently distributed across the three medical systems (e.g., OxygenFlow visualized in Figure~\ref{fig:violindist}), while both DETROIT and TAME are carefully designed towards ICU-specific medical system (e.g., MIMIC-III).


% move to appendix
% TA-DualCV outperforms all baselines with the least overall nRMSE across types of features, mask rates, and three medical systems. Comparing different imputation methods, those targeting unsupervised learning perform better than methods targeting supervised learning on most features across mask rates, while both are worse than TA-DualCV especially when the missingness is large. Moreover, TA-DualCV imputes data more accurately with fewer outliers compared to the baselines. When imputing sepsis-related features, each baseline introduces many outliers (i.e., nRMSE $>$ 1.0) on at least one feature, while TA-DualCV can stably impute data within general value ranges (i.e., nRMSE $\leq$ 0.363) on each feature. Additionally, the nRMSE (average 43.455) of DETROIT on Creatinine is hundreds worse than other imputation methods. This could reveal that such visit-specific approaches perform worse on makers of organ dysfunction (MOD) \cite{yin2020identifying} that may contain more cross-visit information, where DETROIT's worse performance on Platelets, which is another member of MOD, further supports this finding.






==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/Task2.tex <==
\label{sec:task2}
% \begin{table*}[h!]
% \small
% \centering
% \caption{Septic shock 24-hour early prediction results (in average AUC$\pm$std) on 9 sepsis-related features of CCHS, Mayo, and MIMIC-III.}
% \label{tab:pred}
% \begin{tabular}{c|cc|ccc|c}
% \hline
% Dataset   & MeanFill      & ECF           & MICE          & 3D-MICE       & TAME          & TA-DualCV                 \\ \hline
% CCHS      & \textbf{.679$\pm$.021} & .676$\pm$.023 & \textbf{.729$\pm$.033} & .726$\pm$.034 & .513$\pm$.039 & \textbf{.741$\pm$.020}* \\
% Mayo      & \textbf{.783$\pm$.016} & .770$\pm$.014 & \textbf{.786$\pm$.016} & .778$\pm$.007 & .549$\pm$.028 & \textbf{.795$\pm$.018}* \\
% MIMIC-III & .889$\pm$.028 & \textbf{.899$\pm$.023} & .887$\pm$.026 & \textbf{.890$\pm$.017} & .581$\pm$.058 & \textbf{.905$\pm$.018}* \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[h!]
% \small
% \centering
% \caption{Septic shock 24-hour early prediction results (in average AUC$\pm$std) on 9 sepsis-related features of CCHS, Mayo, and MIMIC-III with missing indicator (MI).}
% \label{tab:pred+mi}
% \begin{tabular}{c|cc|ccc|c}
% \hline
% Dataset   & \begin{tabular}[c]{@{}c@{}}MeanFill\\  +MI\end{tabular} & \begin{tabular}[c]{@{}c@{}}ECF\\  +MI\end{tabular} & \begin{tabular}[c]{@{}c@{}}MICE\\  +MI\end{tabular} & \begin{tabular}[c]{@{}c@{}}3D-MICE\\  +MI\end{tabular} & \begin{tabular}[c]{@{}c@{}}TAME\\  +MI\end{tabular} & \begin{tabular}[c]{@{}c@{}}TA-DualCV\\  +MI\end{tabular} \\ \hline
% CCHS      & \textbf{.740$\pm$.026}                                           & .729$\pm$.023                                      & \textbf{.770$\pm$.038}                                       & .766$\pm$.054                                          & .707$\pm$.016                                       & \textbf{.777$\pm$.031}*                                \\
% Mayo      & .805$\pm$.014                                           & \textbf{.816$\pm$.022}                                      & .814$\pm$.011                                       & \textbf{.819$\pm$.009}                                          & .787$\pm$.010                                       & \textbf{.830$\pm$.010}*                                \\
% MIMIC-III & .901$\pm$.010                                           & \textbf{.907$\pm$.018}                                      & .904$\pm$.011                                       & \textbf{.906$\pm$.014}                                          & .845$\pm$.142                                       & \textbf{.909$\pm$.011}*                                \\ \hline
% \end{tabular}
% \end{table*}

\begin{table*}[h!]
\centering
\caption{Septic Shock 24-Hour Early Prediction Results (mean$\pm$std) using 9 sepsis-related features on CCHS, Mayo, and MIMIC-III.}
\label{tab:pred}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{l|lllll|lllll}
\hline
Method & \multicolumn{5}{c|}{Raw}                                                                                                                                       & \multicolumn{5}{c}{Combined with Missing Indicators}                                                                                                \\ \cline{2-11} 
                        & \multicolumn{1}{c}{Accuracy}        & \multicolumn{1}{c}{Precision}          & \multicolumn{1}{c}{Recall}       & \multicolumn{1}{c}{F1}              & \multicolumn{1}{c|}{AUC}            & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC}    \\ \hline

\multicolumn{11}{l}{\textbf{CCHS}}   \\ \hline                     
MeanFill    & \textbf{.632$\pm$.025}	& \textbf{.637$\pm$.032}	 & \textbf{.611$\pm$.036}  & 	\textbf{.623$\pm$.036}  &	\textbf{.679$\pm$.021}	&	\textbf{.682$\pm$.019}	&  \textbf{.673$\pm$.031}  &	\textbf{.710$\pm$.058}	&  \textbf{.689$\pm$.058}  &	\textbf{.740$\pm$.026}\\  
ECF     &	.631$\pm$.023  &	.636$\pm$.024   & 	.602$\pm$.079   &	.617$\pm$.079	&   .676$\pm$.023	 &	.673$\pm$.020   &	.668$\pm$.018	&   .687$\pm$.044	&   .677$\pm$.044	&  .729$\pm$.023				\\ \cline{2-11}
MICE    &  \textbf{.672$\pm$.020}    &	\textbf{.670$\pm$.026}	&   \textbf{.680$\pm$.048}$^\ddag$	&   \textbf{.673$\pm$.048}   &	\textbf{.729$\pm$.033}	&	\textbf{.708$\pm$.043}	&   \textbf{.713$\pm$.059}	&   .692$\pm$.050	&   \textbf{.703$\pm$.050}	&  \textbf{.770$\pm$.038}$^\ddag$				\\
3D-MICE  &	.666$\pm$.024	&    .673$\pm$.015	&   .643$\pm$.058	&   .656$\pm$.058	&   .726$\pm$.034	&	.704$\pm$.049	&   .707$\pm$.056	&   .692$\pm$.086	&   .697$\pm$.086	& .766$\pm$.054				\\
TAME    &  .482$\pm$.010  & 	.291$\pm$.238   &	.600$\pm$.490	&   .392$\pm$.490   &	.513$\pm$.039   &	.643$\pm$.032   &	.633$\pm$.048	&   \textbf{.714$\pm$.074}$^\ddag$   &	.666$\pm$.074   &	.707$\pm$.016				\\ \hline

TA-DualCV$^{-C}$   &  .679$\pm$.024   &	.688$\pm$.032   &	.652$\pm$.055   &	.668$\pm$.055   &	.726$\pm$.026   &	.714$\pm$.017$^\ddag$   &	.714$\pm$.018$^\ddag$   &	.711$\pm$.027   &	.712$\pm$.027$^\ddag$   &	.769$\pm$.025				              \\
TA-DualCV$^{-I}$  &	\textbf{.690$\pm$.025}**   &  .691$\pm$.024$^\ddag$   &	\textbf{.689$\pm$.051}**   &	\textbf{.689$\pm$.051}**   &	.730$\pm$.036$^\ddag$   &	.701$\pm$.033   &	.701$\pm$.041   &	.701$\pm$.039   &	.700$\pm$.039   &	.765$\pm$.044				\\
TA-DualCV &	.687$\pm$.037$^\ddag$  & \textbf{.700$\pm$.033}**   &	.662$\pm$.034   &	.674$\pm$.034$^\ddag$  &	\textbf{.741$\pm$.020}**   &	\textbf{.721$\pm$.035}**   &	\textbf{.716$\pm$.039}**	&   \textbf{.729$\pm$.044}**   &	\textbf{.721$\pm$.055}**   &	\textbf{.777$\pm$.031}**				\\ \hline  



\multicolumn{11}{l}{\textbf{Mayo}}  \\ \hline
MeanFill    &   .695$\pm$.020   &	\textbf{.699$\pm$.033}   &	.690$\pm$.025   &	.693$\pm$.025   &	\textbf{.783$\pm$.016}   &	.722$\pm$.020   &	.711$\pm$.039   &	\textbf{.752$\pm$.055}	&   .729$\pm$.055   &	.805$\pm$.014				\\  
ECF     &   \textbf{.701$\pm$.014}   &	.699$\pm$.023   &	\textbf{.705$\pm$.026}   &	\textbf{.702$\pm$.026}   &	.770$\pm$.014   &	\textbf{.733$\pm$.021}   &	\textbf{.730$\pm$.033}   &	.739$\pm$.029   &	\textbf{.734$\pm$.029}   &	\textbf{.816$\pm$.022}				 \\ \cline{2-11}
MICE    &	\textbf{.711$\pm$.014}  &	\textbf{.715$\pm$.015}  &	.701$\pm$.044  &	\textbf{.707$\pm$.044}  &	\textbf{.786$\pm$.016}  &	.727$\pm$.009  &	.726$\pm$.027  &	.735$\pm$.032  &	.729$\pm$.032  &	.814$\pm$.011				\\
3D-MICE  & 	.697$\pm$.016  &	.706$\pm$.030  &	.673$\pm$.036  &	.689$\pm$.036  &	.778$\pm$.007  &	\textbf{.735$\pm$.009}  &	\textbf{.732$\pm$.023}  &	.743$\pm$.018  &	.737$\pm$.018  &	\textbf{.819$\pm$.009}				\\
TAME    &   .515$\pm$.034   &	.523$\pm$.029   &	.576$\pm$.268   &	.510$\pm$.268   &	.549$\pm$.028   &	.730$\pm$.017   &	.710$\pm$.033   &	\textbf{.780$\pm$.041}**   &	\textbf{.742$\pm$.041}   &	.787$\pm$.010				\\ \hline

TA-DualCV$^{-C}$ &	.713$\pm$.021	&   .717$\pm$.035$^\ddag$   &	.703$\pm$.043   &	.709$\pm$.043   &	.793$\pm$.018	&	.735$\pm$.016   &	.735$\pm$.028   &	.739$\pm$.050   &	.735$\pm$.050   &	.819$\pm$.013				                 \\
TA-DualCV$^{-I}$  &	\textbf{.722$\pm$.014}**	&   .716$\pm$.007   &	\textbf{.733$\pm$.052}**   &	\textbf{.724$\pm$.052}**   &	\textbf{.796$\pm$.013}**   &	.746$\pm$.006$^\ddag$  &	.740$\pm$.028$^\ddag$   &	\textbf{.762$\pm$.047}$^\ddag$    &	.749$\pm$.047$^\ddag$   &	\textbf{.834$\pm$.005}**				\\
TA-DualCV &	.717$\pm$.017$^\ddag$	&   \textbf{.732$\pm$.022}**   &	.724$\pm$.026$^\ddag$   &	.719$\pm$.026$^\ddag$  &	.795$\pm$.018$^\ddag$	&	\textbf{.752$\pm$.009}**   &	\textbf{.760$\pm$.023}**   &	.751$\pm$.043   &	\textbf{.750$\pm$.043}**   &	.830$\pm$.010$^\ddag$				\\ \hline  




\multicolumn{11}{l}{\textbf{MIMIC-III}}  \\ \hline
MeanFill    &	\textbf{.816$\pm$.037}   &	.836$\pm$.039   &	.789$\pm$.084   &	.808$\pm$.084   &	.889$\pm$.028	&	\textbf{.848$\pm$.025}   &	.839$\pm$.036   &	\textbf{.863$\pm$.047}   &	\textbf{.850$\pm$.047}   &	.901$\pm$.010				\\  
ECF     &	.834$\pm$.041	&   \textbf{.848$\pm$.052}	&   \textbf{.813$\pm$.061}   &	\textbf{.829$\pm$.061}   &	\textbf{.899$\pm$.023}	&	\textbf{.845$\pm$.034}	&   .845$\pm$.022   &	.846$\pm$.088   &	.842$\pm$.088   &	\textbf{.907$\pm$.018}$^\ddag$				\\ \cline{2-11}
MICE    &	\textbf{.837$\pm$.037}   &	\textbf{.850$\pm$.059}$^\ddag$  &	\textbf{.826$\pm$.046}   &	\textbf{.835$\pm$.046}   &	.887$\pm$.026	&	\textbf{.846$\pm$.020}   &	\textbf{.855$\pm$.028}$^\ddag$   &	.836$\pm$.061   &	.844$\pm$.061   &	.904$\pm$.011				\\
3D-MICE  &	.825$\pm$.015	&   .831$\pm$.053   &	.823$\pm$.045   &	.824$\pm$.045   &	\textbf{.890$\pm$.017}	&	.846$\pm$.022   &	.847$\pm$.024   &	.847$\pm$.050   &	\textbf{.846$\pm$.050}   &	\textbf{.906$\pm$.014}				\\
TAME    & 	.510$\pm$.025   &	.616$\pm$.196   &	.493$\pm$.349   &	.436$\pm$.349   &	.581$\pm$.058	&	.782$\pm$.144   &	.739$\pm$.128   &	\textbf{.957$\pm$.042}   &	.825$\pm$.042   &	.845$\pm$.142				\\ \hline

TA-DualCV$^{-C}$  &   .825$\pm$.021   &   .846$\pm$.036   &	.796$\pm$.036   &	.819$\pm$.036   &	.892$\pm$.021	&	.845$\pm$.032   &	.851$\pm$.034   &	.839$\pm$.072   &	.842$\pm$.072   &	.905$\pm$.015				 \\
TA-DualCV$^{-I}$  &	.838$\pm$.035$^\ddag$   &	.844$\pm$.030   &	.829$\pm$.058$^\ddag$   &	.836$\pm$.058$^\ddag$   &	.900$\pm$.025$^\ddag$	&	.854$\pm$.021$^\ddag$   &   .847$\pm$.037   &	.863$\pm$.038	&   .854$\pm$.038$^\ddag$   &	.903$\pm$.015				\\
TA-DualCV     &   \textbf{.856$\pm$.024}**   &	\textbf{.852$\pm$.028}**   &	\textbf{.864$\pm$.034}**   &	\textbf{.858$\pm$.034}**   &	\textbf{.905$\pm$.018}**   &	\textbf{.863$\pm$.032}**   &	\textbf{.856$\pm$.026}**   &	\textbf{.880$\pm$.045}$^\ddag$   &	\textbf{.864$\pm$.049}**   &	\textbf{.909$\pm$.011}**				\\ \hline  
\end{tabular}
\begin{tablenotes}
      \small
      \item - For each block, the best model is in \textbf{bold}; The best and the second-best models across ALL are labeled with ** and \ddag, respectively.
    \end{tablenotes}
\end{threeparttable}
}
\end{table*}


To examine how our proposed approach performs on a supervised task, we utilize the complete data with nine sepsis-related features generated by implementing different imputation methods, to build an LSTM network to predict an extremely challenging condition in practice, septic shock. We predict septic shock 24 hours before its onset, as suggested by domain experts to enable early treatments that can prevent 80\% of deaths \cite{DBLP:conf/bigdataconf/SohnPC20, henry2015targeted, zhang2019time}.
Furthermore, we combine each imputation method with missing indicator (MI), for prediction and exploit \textit{to what extent the missing pattern information can affect the prediction results}. The missing indicator $\mathbf{MI}_{i,j,k}$ of a missing value $X_{i,j,k}$ is represented as
\begin{center}
    %$MI_{i,j,k}$ = $\begin{cases} 1 &$ if $X_{i,j,k}$ is missing $\\ 0 & otherwise \end{cases}$
    $MI_{i,j,k} = \mathds{1}\{X_{i,j,k}$ is missing$\}$.
\end{center}







\subsection{Experimental Setup}
In this experiment, we use the three datasets that containing events within their observation window as described in Section~\ref{sec:imputation-data} and the same baselines as the ones from Section~\ref{sec:imputation-baseline} except DETROIT, as it does not produce complete data as described in Section~\ref{sec:imputation-result}.
%\subsubsection{Visits Cut and Pad} 
% When conducting the septic shock early prediction, we are given EHRs of a patient's visit until 24 hours before an endpoint to predict whether or not this patient will develop septic shock 24 hours later. For septic shock visits, the endpoint is the onset of septic shock; whereas for non-septic shock visits, the endpoint is a randomly cut point such that the distribution of their length is similar to the shock visits. As shown in Figure~\ref{OWFW}, from the start of a visit until 24 hours before the endpoint is denoted as \emph{observation window}, while the 24-hour leading up to the endpoint is denoted as \emph{prediction window}. 
For parameters settings, in LSTM, we use a general setting with 1 hidden layer with 128 hidden neurons, 0.005 initial learning rate. We adapt Adam optimizer \cite{kingma2014adam} with 64 batches and 25 epochs. 


\subsubsection{Evaluation Matrix}
Metrics of accuracy (Acc), recall, precision (Prec), F-score (F1) and area under the ROC curve (AUC) were employed for evaluating our models. Accuracy is the proportion of patients whose labels are correctly identified. Recall indicates what proportion of patients that actually have septic shock can be correctly diagnosed by the model as septic shock. Precision tells what proportion of patients who are diagnosed as septic shock actually have septic shock. F1 is the harmonic mean of precision and recall that sets their trade-off. AUC calculates the tradeoff between recall and specificity. Experiment results are averaged from 5-fold cross-validation.
% Our evaluation metrics include accuracy, recall, precision, $F_1$ score (F1), and area under ROC curve (AUC) obtained from 5-fold cross-validation.

% \subsubsection{Implementation Details}

% In LSTM, we use 1 hidden layer with 128 hidden neurons, 0.005 initial learning rate, and 70 maximum sequence-length. We adapt Adam optimizer \cite{kingma2014adam} with 64 batches and 25 epochs.






% \begin{table*}[h!]
% % \label{tab:pred}
% \centering
% \caption{Septic Shock 24-Hour Early Prediction Results (mean$\pm$std) on CCHS, Mayo, and MIMIC-III Data.}
% \label{tab:pred}
% \resizebox{\textwidth}{!}{%
% % \begin{threeparttable}
% \begin{tabular}{l|lllll|lllll}
% \hline
% \multirow{Method} & \multicolumn{5}{c|}{Raw}                                                                                                                                       & \multicolumn{5}{c}{Combined with Missing Indicators}                                                                                                \\ \cline{2-11} 
%                         & \multicolumn{1}{c}{Accuracy}        & \multicolumn{1}{c}{Precision}          & \multicolumn{1}{c}{Recall}       & \multicolumn{1}{c}{F1}              & \multicolumn{1}{c|}{AUC}            & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC}    \\ \hline
% \multicolumn{11}{l}{\textbf{CCHS}}   \\ \hline                     
% MeanFill    & .632$\pm$.025	& .637$\pm$.032	 & .611$\pm$.036  & 	.623$\pm$.036  &	.679$\pm$.021	&	.682$\pm$.019	&  .673$\pm$.031  &	.710$\pm$.058	&  .689$\pm$.058  &	.740$\pm$.026\\  
% ECF     &	.631$\pm$.023  &	.636$\pm$.024   & 	.602$\pm$.079   &	.617$\pm$.079	&   .676$\pm$.023	 &	.673$\pm$.020   &	.668$\pm$.018	&   .687$\pm$.044	&   .677$\pm$.044	&  .729$\pm$.023				\\ \cline{2-11}
% MICE    &  \textbf{.672$\pm$.020}    &	\textbf{.670$\pm$.026}	&   \textbf{.680$\pm$.048}^\ddag	&   \textbf{.673$\pm$.048}   &	\textbf{.729$\pm$.033}	&	\textbf{.708$\pm$.043}	&   \textbf{.713$\pm$.059}	&   .692$\pm$.050	&   \textbf{.703$\pm$.050}	&  \textbf{.770$\pm$.038}^\ddag				\\
% 3D-MICE  &	.666$\pm$.024	&    .673$\pm$.015	&   .643$\pm$.058	&   .656$\pm$.058	&   .726$\pm$.034	&	.704$\pm$.049	&   .707$\pm$.056	&   .692$\pm$.086	&   .697$\pm$.086	& .766$\pm$.054				\\
% TAME    &  .482$\pm$.010  & 	.291$\pm$.238   &	.600$\pm$.490	&   .392$\pm$.490   &	.513$\pm$.039   &	.643$\pm$.032   &	.633$\pm$.048	&   \textbf{.714$\pm$.074}^\ddag   &	.666$\pm$.074   &	.707$\pm$.016				\\ \hline

% TA-DualCV$^{-C}$   &  .679$\pm$.024   &	.688$\pm$.032   &	.652$\pm$.055   &	.668$\pm$.055   &	.726$\pm$.026   &	.714$\pm$.017^\ddag   &	.714$\pm$.018^\ddag   &	.711$\pm$.027   &	.712$\pm$.027^\ddag   &	.769$\pm$.025				              \\
% TA-DualCV$^{-I}$  &	\textbf{.690$\pm$.025}**   &  .691$\pm$.024$^\ddag$   &	\textbf{.689$\pm$.051}**   &	\textbf{.689$\pm$.051}**   &	.730$\pm$.036^\ddag   &	.701$\pm$.033   &	.701$\pm$.041   &	.701$\pm$.039   &	.700$\pm$.039   &	.765$\pm$.044				\\
% TA-DualCV &	.687$\pm$.037^\ddag  & \textbf{.700$\pm$.033}**   &	.662$\pm$.034   &	.674$\pm$.034^\ddag   &	\textbf{.741$\pm$.020}**   &	\textbf{.721$\pm$.035}**   &	\textbf{.716$\pm$.039}**	&   \textbf{.729$\pm$.044}**   &	\textbf{.721$\pm$.055}**   &	\textbf{.777$\pm$.031}**				\\ \hline  



% \multicolumn{11}{l}{\textbf{Mayo}}  \\ \hline
% MeanFill    &   .695$\pm$.020   &	.699$\pm$.033   &	.690$\pm$.025   &	.693$\pm$.025   &	.783$\pm$.016   &	.722$\pm$.020   &	.711$\pm$.039   &	.752$\pm$.055	&   .729$\pm$.055   &	.805$\pm$.014				\\  
% ECF     &   .701$\pm$.014   &	.699$\pm$.023   &	\textbf{.705$\pm$.026}   &	.702$\pm$.026   &	.770$\pm$.014   &	.733$\pm$.021   &	.730$\pm$.033   &	.739$\pm$.029   &	.734$\pm$.029   &	.816$\pm$.022				 \\ \cline{2-11}
% MICE    &	\textbf{.711$\pm$.014}  &	\textbf{.715$\pm$.015}  &	.701$\pm$.044  &	\textbf{.707$\pm$.044}  &	\textbf{.786$\pm$.016}  &	.727$\pm$.009  &	.726$\pm$.027  &	.735$\pm$.032  &	.729$\pm$.032  &	.814$\pm$.011				\\
% 3D-MICE  & 	.697$\pm$.016  &	.706$\pm$.030  &	.673$\pm$.036  &	.689$\pm$.036  &	.778$\pm$.007  &	\textbf{.735$\pm$.009}  &	\textbf{.732$\pm$.023}  &	.743$\pm$.018  &	.737$\pm$.018  &	\textbf{.819$\pm$.009}				\\
% TAME    &   .515$\pm$.034   &	.523$\pm$.029   &	.576$\pm$.268   &	.510$\pm$.268   &	.549$\pm$.028   &	.730$\pm$.017   &	.710$\pm$.033   &	\textbf{.780$\pm$.041}**   &	\textbf{.742$\pm$.041}   &	.787$\pm$.010				\\ \hline

% TA-DualCV$^{-C}$ &	.713$\pm$.021	&   .717$\pm$.035^\ddag   &	.703$\pm$.043   &	.709$\pm$.043   &	.793$\pm$.018	&	.735$\pm$.016   &	.735$\pm$.028   &	.739$\pm$.050   &	.735$\pm$.050   &	.819$\pm$.013				                 \\
% TA-DualCV$^{-I}$  &	\textbf{.722$\pm$.014}**	&   .716$\pm$.007   &	\textbf{.733$\pm$.052}**   &	\textbf{.724$\pm$.052}**   &	\textbf{.796$\pm$.013}**   &	.746$\pm$.006^\ddag  &	.740$\pm$.028^\ddag   &	\textbf{.762$\pm$.047}^\ddag    &	.749$\pm$.047^\ddag   &	\textbf{.834$\pm$.005}**				\\
% TA-DualCV &	.717$\pm$.017^\ddag	&   \textbf{.732$\pm$.022}**   &	.724$\pm$.026^\ddag   &	.719$\pm$.026^\ddag   &	.795$\pm$.018^\ddag	&	\textbf{.752$\pm$.009}**   &	\textbf{.760$\pm$.023}**   &	.751$\pm$.043   &	\textbf{.750$\pm$.043}**   &	.830$\pm$.010^\ddag				\\ \hline  




% \multicolumn{11}{l}{\textbf{MIMIC-III}}  \\ \hline
% MeanFill    &	.816$\pm$.037   &	.836$\pm$.039   &	.789$\pm$.084   &	.808$\pm$.084   &	.889$\pm$.028	&	.848$\pm$.025   &	.839$\pm$.036   &	.863$\pm$.047   &	\textbf{.850$\pm$.047}   &	.901$\pm$.010				\\  
% ECF     &	.834$\pm$.041	&   .848$\pm$.052	&   .813$\pm$.061   &	.829$\pm$.061   &	\textbf{.899$\pm$.023}	&	.845$\pm$.034	&   .845$\pm$.022   &	.846$\pm$.088   &	.842$\pm$.088   &	\textbf{.907$\pm$.018}^\ddag				\\ \cline{2-11}
% MICE    &	\textbf{.837$\pm$.037}   &	\textbf{.850$\pm$.059}^\ddag  &	\textbf{.826$\pm$.046}   &	\textbf{.835$\pm$.046}   &	.887$\pm$.026	&	\textbf{.846$\pm$.020}   &	\textbf{.855$\pm$.028}^\ddag   &	.836$\pm$.061   &	.844$\pm$.061   &	.904$\pm$.011				\\
% 3D-MICE  &	.825$\pm$.015	&   .831$\pm$.053   &	.823$\pm$.045   &	.824$\pm$.045   &	.890$\pm$.017	&	.846$\pm$.022   &	.847$\pm$.024   &	.847$\pm$.050   &	.846$\pm$.050   &	.906$\pm$.014				\\
% TAME    & 	.510$\pm$.025   &	.616$\pm$.196   &	.493$\pm$.349   &	.436$\pm$.349   &	.581$\pm$.058	&	.782$\pm$.144   &	.739$\pm$.128   &	\textbf{.957$\pm$.042}   &	.825$\pm$.042   &	.845$\pm$.142				\\ \hline

% TA-DualCV$^{-C}$  &   .825$\pm$.021   &   .846$\pm$.036   &	.796$\pm$.036   &	.819$\pm$.036   &	.892$\pm$.021	&	.845$\pm$.032   &	.851$\pm$.034   &	.839$\pm$.072   &	.842$\pm$.072   &	.905$\pm$.015				 \\
% TA-DualCV$^{-I}$  &	.838$\pm$.035^\ddag   &	.844$\pm$.030   &	.829$\pm$.058$^\ddag$   &	.836$\pm$.058$^\ddag$   &	.900$\pm$.025$^\ddag$	&	.854$\pm$.021$^\ddag$   &   .847$\pm$.037   &	.863$\pm$.038	&   .854$\pm$.038$^\ddag$   &	.903$\pm$.015				\\
% TA-DualCV     &   \textbf{.856$\pm$.024}**   &	\textbf{.852$\pm$.028}**   &	\textbf{.864$\pm$.034}**   &	\textbf{.858$\pm$.034}**   &	\textbf{.905$\pm$.018}**   &	\textbf{.863$\pm$.032}**   &	\textbf{.856$\pm$.026}**   &	\textbf{.880$\pm$.045}^\ddag   &	\textbf{.864$\pm$.049}**   &	\textbf{.909$\pm$.011}**				\\ \hline  

% \end{tabular}
% % \begin{tablenotes}
% %       \small
% %       \item - For each block, the best model is in \textbf{bold}; The best and the second-best models across ALL are labeled with ** and \ddag, respectively.
% %     \end{tablenotes}
% % \end{threeparttable}
% }
% \end{table*}




\subsection{Results}


Table \ref{tab:pred} presents the 24-hours early prediction results of septic shock without and with missing indicators. 
Either without or with missing indicators, there is no clear winner between the two approaches towards supervised learning tasks. Among the three approaches towards unsupervised learning tasks, in general, MICE and 3D-MICE perform better than TAME. Interestingly, TAME performs worse than other baselines without missing indicators, probably because it outputs tensor-shape data and some useful information regarding septic shock prediction is discarded. Across Table \ref{tab:pred},  TA-DualCV is the best approach across all approaches and MI settings. 
%Specifically, the three TA-DualCV-based models without MI generally outperform all baselines in that for each dataset, the highest score across all metrics  generally comes from one of the three TA-DualCV-based models. Among the three TA-DualCV-based models, either TA-DualCV or TA-DualCV$^{-I}$ perform the best on various measures across the datasets. This result indicates that capturing across-visits dependencies within sepsis-related features can effectively help model predictive variables as both TA-DualCV$^{-I}$ and TA-DualCV can capture both multivariate and temporal information across-visits. 
When combined with MI, the performance of each imputation approach is improved compared to the original corresponding approach without MI. This suggests that the missing pattern is indeed an important characteristic of EHRs for prediction. For example, when a patient is in a severe condition, events are likely to be recorded more frequently than when a patient is in a relatively ``healthier" condition. Also, TA-DualCV generally benefits less from MI compared to other methods. For example, on MIMIC-III, the AUC of TA-DualCV only increases by $0.4\%$ after combined with MI, while the AUC of TAME increases by $45\%$. The reason might be TA-DualCV has already captured various dependencies within data, which could contain missing pattern information revealed by MI. Moreover, imputation methods benefit more from MI on CCHS and Mayo, but not much on MIMIC-III probably because the former two contain much more native missing values compared to MIMIC-III. 




% some advanced imputation models such as Mix-MI \cite{xue2019mixture} and CATSI \cite{yin2020context} could not be implemented in our experiments. With the limited training data (e.g., 1,124 visits in total including only 9 features and 85.7\% missing values in CCHS), some deep learning based methods such as BRITS \cite{cao2018brits} also could not be implemented. These further indicate that TA-DualCV is a more general and robust imputation method that can better handle incomplete clinical data with a mixed type of missing mechanisms and varied underlying data distributions.  


% For example, tensor-based approaches, such as GP-VAE \cite{fortuin2020gpvae}, require a fixed number of events across visits. They exclude visits that contain fewer events and truncate the visits that contain more events, while in clinical practice visits under different health conditions can have a varied number of events. Window-based approaches, such as DETROIT\cite{yan2019detroit}, require a lower bound on the number of events to form a sliding window and specific density of observed neighboring measurements to predict missing values within the window. However, these approaches are data-driven that are designed for datasets with known characteristics, while clinical data across medical systems can vary dramatically \cite{khoshnevisan2020adversarial}. Deep-learning based imputation approaches, such as BRITS \cite{cao2018brits}, achieve promising results. However, these approaches rely on high-quality representations that are extracted from substantial data, while their imputation performance can be marked attenuate with limited training data in practice as discussed in \cite{xu2020multi}.


==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/background-v2.tex <==



\subsection{Septic Shock Prediction}

Various machine learning approaches, such as Temporal Belief Memory (TBM) \cite{kim2018temporal} and Time-aware subGroup Basis Approach with Forecasted events (TGBA-F) \cite{yang2018time}, have been applied to missing EHRs to predict septic shock. For example,  TBM \cite{kim2018temporal} captures latent missing patterns based on irregular time intervals of EHRs and imputes missing values within a time window during recurrent neural network (RNN) based classifier training for septic shock prediction. TGBA-F \cite{yang2018time} utilizes matrix decomposition for data imputation by considering forecasting future events, irregular time intervals, and patients subgroups, which is concurrent with RNN classifier training for septic shock prediction. Though both approaches can impute missing values, these need to combine a classifier and cannot be standalone for missing EHRs imputation. As our main focus is constructing a standalone imputing method that can be used for both unsupervised and supervised learning tasks, we don't compare TA-DualCV to these approaches.   

\subsection{Missing EHRs Imputation}

Existing approaches of missing EHRs imputation in general can be divided into \emph{those evaluated on unsupervised learning tasks} and \emph{those designed towards supervised learning tasks}. 

\subsubsection{Approaches evaluated on unsupervised learning tasks} Table~\ref{tab:prelim} summarizes the characteristics of some recently proposed imputation approaches. These approaches can be categorized into \emph{non-Neutral Network (NN)-} and \emph{NN-based approaches}. For example, MICE \cite{buuren2010mice} captures multivariate dependencies using chained equations, and 3D-MICE \cite{luo20183d} combines MICE and Gaussian process to integrate multivariate dependencies cross-visit and time-aware dependencies within-visit. Both MICE and 3D-MICE are non-NN-based and evaluated on MIMIC-III with a moderate missing rate (i.e., 17\%) across their selected 13 features in~\cite{luo20183d}. Benefiting from chained equations, both approaches do not require specific characteristics or assumptions to be followed in EHRs, which motives us to use chained equations for EHRs imputation. 

More recently, NN-based approaches have been proposed and achieved better performance than existing non-NN-based approaches. For example, DETROIT~\cite{yan2019detroit} prefills missing values with means and impute missing values based on neural networks by leveraging multivariate and time-aware dependencies from observed values within a 5-length sliding window, and it is evaluated on a subset of MIMIC-III with a small missing rate (i.e., 7\%) across 13 lab analyte features. GP-VAE~\cite{fortuin2020gpvae} takes tensor-shape data (i.e., a fixed number of events across visits) as model inputs and uses deep variational autoencoders to map the missing data into a latent space without missingness, where it models the low-dimensional dynamics with a Gaussian process. It is evaluated on PhysioNet data~\cite{silva2012predicting} with 78\% missing rate across 35 features. BRITS~\cite{cao2018brits} and CATSI~\cite{yin2020context} prefill missing values and adopt bidirectional recurrent neural networks (RNNs) to model data. BRITS is evaluated on PhysioNet data, and CATSI is evaluated on the same subset of MIMIC-III as DETROIT. BRITS further evaluates their work on in-hospital death classification, however, diseases diagnosis would be more desirable as important supervised learning tasks in healthcare that can guide clinicians construct treatments and intervention. Without prefilling, TAME~\cite{yin2020identifying} utilizes bidirectional RNNs and within-visit multi-modal embedding that takes data including demographics, diagnosis, medication, features, and time-intervals as inputs, and it outputs tensor-shape data without missingness. It is evaluated on MIMIC-III data with 54\% average missing rate across 29 features. 

Despite NN-based approaches' superior performance in imputation, they have at least one of the three major limitations: i) \emph{Tensor-shape input/output}. They require tensor-shape data as input or output, while in clinical practice visits under different health conditions can have a varied number of events. Truncating data into tensor shape can exclude substantial information. ii) \emph{Sliding window}. They impute each missing value using observations within a fixed number of time steps around the missing value, which may not work on highly sparse data. iii) \emph{Prefill}. They need to prefill the missing values to provide fixed-size inputs for NNs, while prefilling can introduce bias which limits model performance. Unlike these approaches, our framework is non-NN-based and does not require tensor-shape input/output, sliding window, or prefilling. BRITS and GP-VAE can handle high missing EHRs. However, they require tensor-shape inputs. As real-world EHRs often contain varied numbers of events across visits, we don't consider BRITS and GP-VAE as baselines in this work. Also, as BRITS, CATSI, and TAME are all bidrectional-RNNs-based among which TAME has achieved the best performance, and DETROIT has been recognized as a strong baseline in~\cite{yan2019detroit}, we use TAME and DETROIT as baselines in this study.              

\subsubsection{Approaches designed towards supervised learning tasks}
Missing indicator (MI) \cite{little:stat} shows great success in disease progression modeling~\cite{ho2014septic,fagerstrom2019lisep,lipton:missing}. However, it only indicates whether a value is observed or missing, thus cannot be directly used for imputation. In this work, we investigate incorporating imputed data with MI for septic shock prediction. Recently, TBM~\cite{kim2018temporal} and TGBA-F~\cite{yang2018time} impute the data concurrent with their classifier training. However, as we have discussed earlier, they cannot be standalone for missing EHRs imputation.     


% Existing approaches of multivariate time series imputation can be clustered into three main types: 

% 1) \textit{Handling longitudinal dependencies only}. 
% These approaches propose longitudinal imputation by modeling temporal trends among measurements of a given feature on related time-steps of missing values (e.g., \cite{rasmussen2010gaussian, he2011longitudinal}). For example, He \emph{et al.} propose time trajectory functions based on Gibbs sampling to impute values missing completely at random \cite{he2011longitudinal}. However, these approaches rely on regularly sampled time series to model longitudinal dependencies, while real-world clinical data can contain multivariate dependencies and be highly sparse with mixed types of missingness when merging irregular collections together.    

% 2) \textit{Handling multivariate dependencies only}.
% These approaches impute missing values on an event by modeling multivariate dependencies among related features (e.g., \cite{buuren2010mice, mattei2019miwae}). For example, Mattei and Frellsen propose an autoencoder-based imputation approach, by approximating conditional expectation of missing features using importance sampling from observed features \cite{mattei2019miwae}. However, these approaches generally capture feature dependencies thus may not be well-fit into clinical applications, as real-world clinical data usually consists of time series and contains temporal trajectories among events. 

% 3) \textit{Handling both multivariate and longitudinal dependencies}. These approaches captures multivariate dependencies and partial 
% %(i.e., temporal perspective across time-steps or time-aware perspective across time-intervals)
% longitudinal dependencies, either within-visit or across-visits (e.g., \cite{luo20183d,yin2020context,yin2020identifying}). For instance, \cite{yin2020context} design a neural network based framework to capture multivariate and temporal dependencies across-visits. \cite{yin2020identifying} propose an auto-encoder based method to capture multivariate and time-aware dependencies within-visit. These approaches have achieved promising results. However, there still remain potentials for clinical imputation approaches by exploiting dependencies across features, time-steps, and time-intervals, both within-visit and across-visits.       

%%% Ge: move some to results to discuss
% 3) \textit{Handling both multivariate and longitudinal dependencies but data-specifically}.
% These approaches capture both multivariate and longitudinal dependencies but are designed toward data with specific underlying characteristics (e.g., number of events across samples) thus limit their application in clinical data (e.g., \cite{cao2018brits, yan2019detroit, zhang2020predicting, fortuin2020gpvae}). For example, tensor-based approaches, such as GP-VAE \cite{fortuin2020gpvae}, require a fixed number of events across visits. They exclude visits that contain fewer events and truncate the visits that contain more events, while in clinical practice visits under different health conditions can have a varied number of events. Window-based approaches, such as DETROIT\cite{yan2019detroit}, require a lower bound on the number of events to form a sliding window and specific density of observed neighboring measurements to predict missing values within the window. However, these approaches are data-driven that are designed for datasets with known characteristics, while clinical data across medical systems can vary dramatically \cite{khoshnevisan2020adversarial}. Deep-learning based imputation approaches, such as BRITS \cite{cao2018brits}, achieve promising results. However, these approaches rely on high-quality representations that are extracted from substantial data, while their imputation performance can be marked attenuate with limited training data in practice as discussed in \cite{xu2020multi}.






==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/conclusion.tex <==


In this work, we present \textit{TA-DualCV}, a non-Neural Network-based imputation framework towards both unsupervised and supervised learning tasks in EHRs. TA-DualCV TA-DualCV integrates both cross-visit and within-visit dependencies, by exploiting dependencies among features, time-interval, and time-steps. The robustness of TA-DualCV is evaluated on two tasks: \emph{unsupervised imputation task} and \emph{supervised 24-hour septic shock early prediction task} using EHRs from three different medical systems. In both tasks, TA-DualCV is compared to state-of-the-art baselines. Among the different baselines, 3D-MICE consistently outperformed other baselines on the unsupervised learning tasks, while on the supervised task of early septic shock prediction, there was no clear winner. TA-DualCV, on the other hand, shows its robustness to handle high missing rates of EHRs across medical systems by achieving the best performance on both imputation and septic shock early prediction tasks on all evaluation metrics. 

It is also important to note that we cannot produce results in our experiments with some popular imputation approaches, which are data-driven to a specific type of missingness or data characteristic (e.g., ICU lab analytes data with a small native missing rate). Mayo, for example, can have events ranging from 1 to 5,000 across different visits. Consequently, approaches including Mix-MI \cite{xue2019mixture} and GP-VAE \cite{fortuin2020gpvae} that require tensor-shape inputs cannot be utilized. For approaches relying on sliding windows, including DETROIT\cite{yan2019detroit}, a lower bound on the number of events is needed to compute a sliding window, and a specific density of neighboring measurements must be observed to predict missing values. They are not be able to produce certain results in our experiments. Additionally, our experiments on CCHS and Mayo have fewer training data but higher average native missing rates (up to $73\%$) than those used the existing literature. In practice, as discussed in \cite{xu2020multi}, deep learning relies on high-quality representations of the output of substantive data, whereas their imputation performance dwindles with limited training data. 

%In this work, we present \textit{TA-DualCV}, a general, robust missing  value  imputation  method for handling multivariate time series clinical data. TA-DualCV captures both \textit{multivariate} and \textit{longitudinal} dependencies by integrating dependencies among features, time intervals, and time-steps, both \textit{within-visit} and \textit{across-visits}. The effectiveness of TA-DualCV is evaluated on two tasks: \emph{unsupervised imputation task} and \emph{supervised 24-hour septic shock early prediction task} using EHRs from three different medical systems. Our overall results show that TA-DualCV is compared to the state-of-the-art baselines on both tasks . Among different baselines, our results showed that 3D-MICE consistently outperforms other baselines on the unsupervised learning tasks while on the supervised task of sepsis early prediction, there is no clear winner among the baselines. On the other hand, TA-DualCV presents its generalizability and robustness in handling high missing rates within clinical data across medical systems by achieving the best performance in both imputation and septic shock prediction tasks on almost all measures. 


 %In other words,  TA-DualCV presents its generalizability and robustness in handling high missing rates within clinical data across medical systems by achieving the best performance in both imputation and septic shock prediction tasks. Furthermore, we observe the baselines in our experiments still present strengths with their originally targeted tasks, either unsupervised or supervised learning. Specifically, 3D-MICE designed towards imputations performs better than the approaches designed towards disease prediction, in our imputation experiments. And ECF designed towards disease predictions can perform better than approaches designed towards imputations on MIMIC-III data, in our septic shock prediction experiments. TA-DualCV outperforms all baselines in both experiments, which indicates TA-DualCV could be more capable of different tasks.      
% The methods in the imputation task are evaluated with missing values that are masked randomly, while in the prediction task they are mainly evaluated based on the imputed data containing a great amount of native missing values with the mixed type of missing mechanisms. 
% As opposed to TA-DualCV, for example, TAME performs well in imputation task but the worst in the prediction task as compared to all baselines as it is designed towards missingness at random. 


%Moreover, some imputation approaches, which are data-driven toward a specific type of missingness or underlying data characteristics (e.g., ICU lab analytes data with a small native missing rate), cannot produce results with the datasets in our experiments. For instance, in Mayo, the number of events can vary from 1 to 5,000 across visits. Under such a situation, tensor-based approaches, such as Mix-MI \cite{xue2019mixture} and GP-VAE \cite{fortuin2020gpvae}, that require a fixed number of events across visits, cannot be implemented in our study. Window-based approaches, such as DETROIT\cite{yan2019detroit}, require a lower bound on the number of events to form a sliding window and specific density of observed neighboring measurements to predict missing values within the window. They can be incapable in our experiments. Moreover, the training data is limited in our experiments compared to existing related works. For example, CCHS contains 1,124 visits including only 9 features and 85.7\% missing rate. Deep learning based methods BRITS \cite{cao2018brits} cannot produce results in our experiments. The possible reason is the deep learning methods rely on high-quality representations that are extracted from substantial data, while their imputation performance can be marked attenuate with limited training data in practice as discussed in \cite{xu2020multi}. 


% We propose a general imputation method TA-DualCV to impute multivariate time series clinical data. TA-DualCV captures both multivariate and longitudinal dependencies by integrating dependencies among features, time intervals, and time-steps from both \textit{within-visit} and \textit{across-visits} perspectives. The effectiveness and robustness of TA-DualCV is compared against state-of-the-art baselines using three real-world EHRs on two tasks: \emph{unsupervised imputation task} and \emph{supervised 24-hour septic shock early prediction task}. In general, our results show that imputation methods towards unsupervised learning can outperform the imputation methods towards supervised learning, and TA-DualCV outperforms both. Imputation methods with MI can always outperform their corresponding methods without MI, and TA-DualCV with MI has the best performance across methods in prediction tasks. Integrating MI with imputation methods can be further explored in future work.  



==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/exp-old.tex <==


In this work, we mainly validate our imputation model from two aspects: 1) capability, which represents what types of measurements can be imputed by our model; 2) accuracy, which represents how accurate our model can impute the data with varied missing rates. We compare our model with 3 state-of-the-art approaches (3D-MICE \cite{luo20183d}, MICE \cite{buuren2010mice}, GP \cite{rasmussen2003gaussian}) and 1 expert baseline \cite{kim2018temporal}.

%%%% dataset
\subsection{Three Datasets: MIMIC-III, CCHS, and Mayo} collected from different hospitals were involved.  with different characteristics shown in Table \ref{tab:char}. To validate the capacity of our model with two main categories (lab analytes and vital signs) of measurements, we selected 13 lab analytes from MIMIC-III, 9 vital signs from CCHS, and 9 vital signs from Mayo according the specific characteristic of each dataset. We describe the details of selection in the followings.

\subsubsection{MIMIC-III} The MIMIC-III database contains 53,423 admissions of adult patients (i.e., age $>$ 16) who are admitted to intensive care units (ICU) at a tertiary referral hospital between 2001 and 2012 \cite{johnson2016mimic}. Specifically, it contains $\sim$331 million charted observations for patients and 753 laboratory items. Within the MIMIC-III database, we selected 13 laboratory analyte items (shown in Table~\ref{table:char-mimic}) that contain low original missing rates and are measured quantitatively. We also listed the identification codes we use for measurements of interests in MIMIC-III database (see Table \ref{tab:char-mimic}), as the same name of a measurement can have different Item IDs.

In this work, one objective is to validate our imputation method in the context where a large range of masking rates occurs, i.e. $20\% \sim 90\%$. The native missing rates of MIMIC-III is relatively high (i.e. $26.7\%$ on average), thus we applied exclusion criteria for data sampling: i) Exclude records that had less than 11 events; ii) Exclude data from events that contained more than $50\%$ missing rate; iii) Exclude data from laboratory items that contained more than $50\%$ missing rate. Our final data consists of $\sim$17 million record of 19,693 patients. The average missing rate after applying the above criteria is $5.78\%$. The minimum and maximum number of events across records are 11 and 1191, respectively. The mean and median number of events across records are 33.4 and 22, respectively. Aside from the native missing values, we masked values with rates $20\% - 90\%$. Both native and masked values will be imputed to form final complete data. %Therefore, the final imputed data is complete without any missing values so that machine learning techniques that rely on complete data can be applied to the data. The distribution of time points is shown in Fig.~\ref{fig:time-dist-mimic}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.12]{sections/figure/timedist-mimic.jpg}
%     \caption{Distribution of Number of Events in Final Data of MIMIC-III}
%     \label{fig:time-dist-mimic}
% \end{figure}

%% moved to supplementary
% \begin{figure}[t]
%     \centering
%     \includegraphics%[scale=0.4]
%     [width=8.5cm,height=3.4cm]{sections/figure/heatmap.png}
%     \caption{Heatmap of 3 Datasets. (A: MIMIC-III. B: Mayo. C: CCHS.)}
%     \label{fig:heatmap}
% \vspace{-0.2 in}
% \end{figure}



%%% Need more information regarding the 2 datasets 
\subsubsection{Christiana Care Health System (CCHS)} This dataset contains 210,289 visit records of adult patients (i.e. age $>$ 18) admitted to Christiana Care hospital from July, 2013 to December, 2015. The CCHS dataset contains partial types of lab results as compared to MIMIC-III, but greater native missing rates (i.e. $\sim$ 85.7\% on average). This is caused by the nature of this data, as it includes the records of patients at different locations from emergency department to ICU, which is different from MIMIC-III that only includes ICU visits. We selected 9 measurements with the least native missing rates, which belong to vital signs. Due to the large sparsity of the CCHS data, we only impute the native missing values without masking. As the main goal of imputation is to generate complete data to be used by machine learning techniques, we propose to validate our imputation approach by applying a septic shock prediction model on the imputed data. 

We firstly apply one exclusion criteria by excluding events with all missing values. Then we preprocess the data in three steps: 1) aggregate data into 30 minutes window by taking median values on both measurement and recorded time; 2) If a visit contains less than 5 events, carry forward the last value within a fixed length time window (i.e., 8 hours) to fill missing values, and use mean value of corresponding measurement to fill the remaining missing values; 3) OxygenFlow, which is measured every $\sim$45-minute, contains the highest missing rate (i.e. 97.4\%) but stable range of values within records. We carry forward the last value within 8 hours to fill missing values of OxygenFlow and mean values to fill the remaining. After that, we apply the other exclusion criteria by excluding the records that contain less than 2 records of each measurement. Finally, we get $\sim$400 thousands events for 3,240 visits (1,349 shock positive and 1,891 shock negative). The average missing rate is 40.4\%. The minimum and maximum number of evens across records are 1 and 2,277, respectively. The mean and median value of events are 131 and 83, respectively.


\subsubsection{Mayo} This dataset contains 106,844 visit records of adult patients (i.e. age $>$ 18) admitted to Mayo Clinic hospital from July, 2013 to December, 2015. It contains most types of lab results and vital signs compared to MIMIC-III, but similar to CCHS, it has large native missing rates (i.e. $\sim$ 85.6\% on average). We select the same 9 measurements as CCHS with the least original missing rates, which belong to the category of vital signs. Following the aforementioned exclusion and preprocessing criteria with CCHS data, we include $\sim$1.55 million records of 6,850 visits (3,457 shock positive and 3,393 shock negative). The average missing rate is 33.8\%. The minimum and maximum number of evens across records are 3 and 10,663, respectively. The mean and median value of events are 226 and 212, respectively.

%% baseline
%\subsection{Baselines}

%% normalization
\subsection{Normalization}
The proper operation of GP imputation requires normalization while it has little effect on MICE imputation \cite{luo20183d}. Therefore, we normalize our data such that all measurements are scaled to be within [0, 1] interval throughout time points before imputation and de-normalize it to obtain the final complete data after imputation. 
% Specifically, on a time point $t_i$, the normalize value $nv_{ij}$ of a measurement $m_j$ is calculated by the following equation:

% \begin{equation}
%     nv_{ij} = \frac{ov_{ij} - min(ov_{:j})}{max(ov_{:j}) - min(ov_{:j})}
% \end{equation}

% where $ov_{ij}$ represents original value of a measurement $m_j$ at time point $t_i$, and $ov_{:j} = \{ov_{1j},ov_{2j},...,ov_{nj}\}$, $n \in 	\mathbb{R}$.

%%%% Setups: 1) Baselines, 2) Various missing rates
\subsection{Validation}
To assess the performance of 3M-MICE in comparison with the benchmarks and in various circumstances, we validated our model in two experimental settings:

    % \item \textbf{Cross models validation:} We compared our model with 3 baselines, MICE, GP, and Mean imputation. Specifically, we employed MICE package in R \cite{buuren2010mice}. In calling the MICE package, the default number of multiple imputations was 5. To show the lowest possible bound of our model imputation efforts, we used only 1 iteration for multiple imputation in MICE package for both our approach and MICE baseline. We also employed GPfit package in R \cite{macdonald2015gpfit} as another baseline. The parameters used in GP of both our approach and baseline were all default ones except the parameter used in computing the nugget. The details regarding the nugget will be discussed in the following paragraph. Moreover, we employed the balanced parameter 0.5 for both $w_{11}$ and $w_{12}$. In future approaches, the values of $w_{11}$ and $w_{12}$ can be adjusted according to the training performance on target data. 
\textbf{Various Masking Rates on Obervations:} To explore the performance with various missing rates, we conducted 6 sub-samples of MIMIC-III by randomly masking 20\%, 50\%, 60\%, 70\%, 80\%, and 90\% of the observed values. We compare our model with 4 baselines for each measurement and overall data.

\textbf{Septic Shock Early Prediction:} To measure the capabilities of our approach, we utilize the imputed data by different imputation approaches to build an LSTM network to predict a challenging condition in practice, septic shock, 8 hours before its onset, which has been adopted in previous approaches \cite{yang2018time}. Considering the imbalanced ratio between shock positive and negative visits, we employ stratified random sampling on both positive and negative visits. Finally, the CCHS data contains 1300 visits for each group with $\sim$340 thousands events in total, and Mayo data contains 3200 visits for each group with $\sim$1.5 million events in total. Also, we compare our model with baselines by adding missing indicators on measurements to explore whether and what extent missing indicator can affect prediction results.
    
    % Specifically, in GP, the ill-conditioning $R$ (introduced in Eq.~\ref{eq:R-matrix}, Section III.B) might occur if any pair of points ($t_{ik}$ and $t_{jk}$) were too close or $\theta_k$'s were close to 0. To fix such issue, Ranjan et al. introduced a nugget computing a well-behaved $R$ to substitute the ill-conditioning one, and they set a parameter to be the boundary for nugget \cite{ranjan2011computationally}. In this approach, various missing rate of the data could require various values of the nugget-related parameter in single-task GP as higher sparsity of data may introduce ill-conditioning correlation matrix. 


\subsection{Baselines}
We employ 3 state-of-the-art baselines and 1 expert baseline. The state-of-the-art baselines are 3D-MICE \cite{luo20183d}, sampling-based MICE \cite{buuren2010mice}, and GP with RBF kernel. We also employ an expert baseline which is defined by the domain experts and has been adopted in previous research \cite{kim2018temporal}. The expert baseline fills the missing values with the last value within a fixed length window (i.e. 24 hours for lab analytes and 8 hours for vital signs), and fills the remains with the mean value of the corresponding measurements. The expert baseline performs better in clinical data imputation and prediction compared to traditional baselines (e.g. mean/median, carry forward, etc.) in both previous \cite{kim2018temporal} and our work, thus we don't present the results of traditional baselines here. For fair comparison, we adopt the same experimental settings for baselines as our model. 


%%%% Performance evaluation: nRMSE
\subsection{Performance Evaluation}
We evaluated the performance of our model and baselines on imputing masked values by calculating the normalized root-mean-square error (nRMSE). RMSE is frequently employed to measure the differences between estimated values and observed values. It assigns large residuals with a disproportionately large effect, thus more sensitive to outliers \cite{pontius2008components}. Normalizing the RMSE can help in comparing among datasets or models that contain different scales of values. The normalization has different calculation in different approaches. In this study, we used the common choice regarding normalization that was the range of the measured data. Therefore, the nRMSE of a variable $v$ was calculated by the following equation:

\begin{equation}
    nRMSE_v = \sqrt{\frac{\sum_{p,t}(\frac{(\hat{Y}_{v,p,t} - Y_{v,p,t})}{max(Y_{v,p}) - min(Y_{v,p})})^2}{\mid T \mid}}
\end{equation}

where $p \in [1, P]$, $t \in T$. $P$ is the total number of patient in the data, $T$ is a list of time points with missing values of variable $v$ for patient $p$. $\hat{Y}$ represents the estimated value while $Y$ represents the actual value. 

We evaluate the performance of our model and baselines on predicting septic shock by calculating evaluation metrics of accuracy (Acc), recall, precision, $F_1$ score (F1), and area under ROC curve (AUC) obtained from 5 cross-validation. Accuracy is the proportion of correctly classified visits over all visits. Recall is the proportion of correctly identified positive visits over all visits that actually have septic shock. Precision is the proportion of correctly identified positive visits over all visits that are identified as positive. F1 is the harmonic mean of the precision and recall. AUC calculates the trade-off between recall and specificity, where specificity is the proportion of correctly identified negative visits over all visits that are identified as negative.

%%%% settings
In this work, we impute the data with all methods on a 12-core machine. We use 1 iteration on multiple imputation with MICE R package \cite{buuren2010mice} for 3M-MICE, 3D-MICE, and MICE methods, and 0.02 $\alpha$ on RBF kernel with GP \cite{rasmussen2003gaussian}. In 2-step MICE, we assign $0.5$ to both $w_{11}$ and $w_{12}$ to ensure the fairness and balance the effect of MICE through cross-sectional and longitudinal view. In LSTM, we use 1 hidden layer with 128 hidden neurons, 0.005 initial learning rate, and 200 maximum sequence-length. We adopt Adam optimizer \cite{kingma2014adam} with 64 batches and 25 epochs.

==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/exp.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[scale=0.4]{sections/figure/nrmse.png}
    \caption{nRMSE by Measurement and Imputation Method. X-Axis: Masking Rates; Y-Axis: nRMSE.}
    \label{fig:nrmse}
    \vspace{-0.2 in}
\end{figure*}

In this work, we mainly validate our proposed imputation model from two aspects: 1) capability, which represents what types of measurements can be imputed by our model; 2) accuracy, which represents how accurate our model can impute the data with varied missing rates. We compare our model with four baselines (i.e., \cite{luo20183d ,buuren2010mice, rasmussen2003gaussian, kim2018temporal}).

\vspace{-0.1 in}



\vspace{-0.1 in}

\subsection{Various Masking Rates on Observations}
To explore the performance with various missing rates, we conducted 6 sub-samples of MIMIC-III by randomly masking 20\%, 50\%, 60\%, 70\%, 80\%, and 90\% of the observed values. We compare our model with four baselines for each measurement and overall data.

\vspace{-0.1 in}

\subsubsection{Dataset:} \textbf{MIMIC-III} contains 53,423 admissions of adult patients (i.e., age $>$ 16) who are admitted to intensive care units (ICU) at a tertiary referral hospital between 2001 and 2012 \cite{johnson2016mimic}. Specifically, it contains $\sim$331 million charted observations for patients and 753 laboratory items. Within the MIMIC-III database, we selected 13 laboratory analyte items that contain low native missing rates (ranging from $18.1\%$ to $30.9\%$) and are measured quantitatively. The selected items are Chloride, Potassium, Bicarb, Sodium, Hematocrit, Hemoglobin, MCV, Platelet, WBC, RDW, BUN, Creatinine, and Glucose.
We validate our imputation method in the context where a large range of masking rates occurs, i.e. $20\% \sim 90\%$. The native missing rates of MIMIC-III is relatively high ($26.7\%$ on average), thus we applied exclusion criteria for data sampling: i) Exclude records that had less than 11 events; ii) Exclude data from events that contained more than $50\%$ missing rate; iii) Exclude data from laboratory items that contained more than $50\%$ missing rate. Our final data consists of $\sim$17 million record of 19,693 patients. The average missing rate after applying the above criteria is $5.78\%$. The number of events across visits vary from 11 to 1191 with the mean and median of 33.4 and 22, respectively. Aside from the native missing values, we masked values with rates $20\% - 90\%$. Both native and masked values will be imputed to form the final complete data \footnote{Numeric missing rates are attached in supplementary materials in detail}.

\noindent\textbf{Normalization:}
The proper operation of GP imputation requires normalization while it has little effect on MICE imputation \cite{luo20183d}. Therefore, we normalize our data such that all measurements are scaled to be within [0, 1] interval throughout time points before imputation and de-normalize it to obtain the final complete data after imputation. 

\vspace{-0.1 in}

\subsubsection{Performance Evaluation}
We evaluate the performance of methods on imputing masked values by calculating the normalized root-mean-square error (nRMSE). RMSE is frequently employed to measure the differences between estimated values and observed values. It assigns large residuals with a disproportionately large effect, thus more sensitive to outliers \cite{pontius2008components}. Normalizing the RMSE can help in comparing among datasets or models that contain different scales of values. The normalization has different calculation in different approaches. In this study, we used the common choice regarding normalization that was the range of the measured data. Therefore, the nRMSE of a variable $v$ was calculated by the following equation:

\begin{equation}
    nRMSE_v = \sqrt{\frac{\sum_{p,t}(\frac{(\hat{Y}_{v,p,t} - Y_{v,p,t})}{max(Y_{v,p}) - min(Y_{v,p})})^2}{\mid T \mid}}
\end{equation}

\noindent where $p \in [1, P]$, $t \in T$. $P$ is the total number of patient in the data, $T$ is a list of time points with missing values of variable $v$ for patient $p$. $\hat{Y}$ represents the estimated value while $Y$ represents the actual value. 

\vspace{-0.1 in}

\subsection{Septic Shock Early Prediction}
To measure the robustness of our approach, we utilize the imputed data by different imputation methods to build an LSTM network to predict a challenging condition in practice, septic shock, 8 hours before its onset, which has been adopted in previous approaches \cite{yang2018time}. We select 9 measurements with the least native missing rates (ranging from $51.9\%$ to $77.7\%$ for CCHS and $23.5\%$ to $97.4\%$ for Mayo) on both datasets. The 9 measurements include Temperature, FiO2, MAP, DiastolicBP, SystolicBP, PulseOx, RespiratoryRate, HeartRate, and OxygenFlow, which all belong to vital signs. Due to the large sparsity of both datasets, we only impute the native missing values without masking.

\vspace{-0.1 in}

\subsubsection{Datasets:}

\textbf{1) Christiana Care Health System (CCHS)} contains 210,289 visit records of adult patients (i.e. age $>$ 18) admitted to Christiana Care hospital from July, 2013 to December, 2015. The CCHS dataset contains partial types of lab results as compared to MIMIC-III, but greater native missing rates (i.e., $\sim$ 85.7\% on average). This is caused by the nature of this data, as it includes the records of patients at different locations from emergency department to ICU, which is different from MIMIC-III that only includes ICU visits. 

\noindent\textbf{2) Mayo} contains 106,844 visit records of adult patients (i.e. age $>$ 18) admitted to Mayo Clinic hospital from July, 2013 to December, 2015. It contains most types of lab results and vital signs compared to MIMIC-III, but similar to CCHS, it has large native missing rates (i.e. $\sim$ 85.6\% on average).

\subsubsection{Labeling}
The targeted population of CCHS and Mayo datasets are patients with suspected infection, which can be identified by presence of antiviral, antibiotic, etc. To label our records, we adopt our domain experts identification rule \cite{yang2018time}, which is a combination of International Classification of Diseases, Ninth Revision (ICD-9) and the Third International Consensus Definitions for Sepsis and Septic Shock \cite{singer2016third}.

\vspace{-0.1 in}

\subsubsection{Exclusion Criteria and Preprocessing}
For both datasets, we firstly apply one exclusion criteria by excluding events with all missing values. Then we preprocess the data in three steps: 1) aggregate data into 30 minutes window by taking median values on both measurement and recorded time; 2) If a visit contains less than 5 events, we carry forward the last value within a fixed length time window (i.e., 8 hours) to fill missing values, and use mean value of corresponding measurement to fill the remaining missing values; 3) OxygenFlow, which is measured every $\sim$45-minute, contains the highest missing rate (i.e., $97.4\%$) but stable range of values within records. We carry forward the last value within 8 hours to fill missing values of OxygenFlow and mean values to fill the remaining. After that, we apply the other exclusion criteria by excluding the records that contain less than 2 records of each measurement. For CCHS, we get $\sim$400 thousands events for 3,240 visits (1,349 shock positive and 1,891 shock negative). The average missing rate is 40.4\%. The number of events per visit ranges from 1 to 2,277, with the mean and median value of 131 and 83, respectively. For Mayo, we include $\sim$1.55 million records of 6,850 visits (3,457 shock positive and 3,393 shock negative). The average missing rate is 33.8\%. The minimum and maximum number of evens across records are 3 and 10,663, respectively. The mean and median value of events are 226 and 212, respectively.

Considering the imbalanced ratio between shock positive and negative visits, we employ stratified random sampling on both positive and negative visits. Finally, the CCHS data contains 1,300 visits for each group with $\sim$340 thousands events in total, and Mayo data contains 3,200 visits for each group with $\sim$1.5 million events in total. Also, we compare our model with baselines by adding missing indicators on measurements to explore whether and to what extent the missing indicator can affect the prediction results.

\vspace{-0.1 in}

\subsubsection{Performance Evaluation}
We evaluate the methods on predicting septic shock by calculating various evaluation metrics including accuracy, recall, precision, $F_1$ score (F1), and area under ROC curve (AUC) obtained from 5-fold cross-validation. Accuracy is the proportion of correctly classified visits over all visits. Recall is the proportion of correctly identified positive visits over all visits that actually have septic shock. Precision is the proportion of correctly identified positive visits over all visits that are identified as positive. F1 is the harmonic mean of the precision and recall. AUC calculates the trade-off between recall and specificity, where specificity is the proportion of correctly identified negative visits over all visits that are identified as negative.

\vspace{-0.1 in}

\subsection{Baselines}
We employ 3 state-of-the-art baselines and 1 expert baseline. The state-of-the-art baselines are 3D-MICE \cite{luo20183d}, sampling-based MICE \cite{buuren2010mice}, and GP with RBF kernel. We also employ an expert baseline which is defined by the domain experts and has been adopted in previous research \cite{kim2018temporal}. The expert baseline fills the missing values with the last value within a fixed length window (i.e. 24 hours for lab analytes and 8 hours for vital signs), and fills the remains with the mean value of the corresponding measurements. The expert baseline performs better in clinical data imputation and prediction compared to traditional baselines (e.g. mean/median, carry forward, etc.) in both previous \cite{kim2018temporal} and our work, thus we don't present the results of traditional baselines here. For fair comparison, we adopt the same experimental settings for baselines as our model. 

\begin{table*}[h!]
% \label{tab:pred}
\centering
\caption{Septic Shock Prediction Performance (mean$\pm$ std) by Imputation Method on CCHS and Mayo.}
\label{tab:pred}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{l|lllll|lllll}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{CCHS}                                                                                                                                       & \multicolumn{5}{c}{Mayo}                                                                                                \\ \cline{2-11} 
                        & \multicolumn{1}{c}{Accuracy}        & \multicolumn{1}{c}{Recall}          & \multicolumn{1}{c}{Precision}       & \multicolumn{1}{c}{F1}              & \multicolumn{1}{c|}{AUC}            & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC}    \\ \hline
Expert                  &         .691$\pm$.027                            &     .685$\pm$.039                                &       .716$\pm$.044**                              &        .698$\pm$.044                             &     .744$\pm$.023                                &        .808$\pm$.009**                      &         .815$\pm$.019                   &     \textbf{.797$\pm$.018}                          &         .806$\pm$.018**                   &   .879$\pm$.009**                         \\
GP                      & .700$\pm$.017**           & .703$\pm$.042          & .703$\pm$.027          & .702$\pm$.027**          & .757$\pm$.011          &           .803$\pm$.009                   &    .819$\pm$.021**                        &       .779$\pm$.020                        &    .798$\pm$.020                        &          .877$\pm$.007                  \\
MICE                    & .689$\pm$.020          & .686$\pm$.026          & .701$\pm$.032          & .693$\pm$.032          & .743$\pm$.015          & .788$\pm$.013   & .804$\pm$.014 & .760$\pm$.023    & .781$\pm$.023 & .865$\pm$.018 \\
3D-MICE                 & .697$\pm$.012          & .706$\pm$.042**          & .684$\pm$.037          & .693$\pm$.037          & .768$\pm$.016**          & .794$\pm$.011   & .806$\pm$.037 & .776$\pm$.024    & .790$\pm$.024 & .876$\pm$.010 \\
3M-MICE                 & \textbf{.717$\pm$.019}          & \textbf{.711$\pm$.034}          & \textbf{.729$\pm$.022}          & \textbf{.720$\pm$.022}          & \textbf{.777$\pm$.016}          & \textbf{.812$\pm$.006}   & \textbf{824$\pm$.009} & \.795$\pm$.006**   & \textbf{.809$\pm$.006} & \textbf{.889$\pm$.007} \\ \hline

Expert+MI               &       .736$\pm$.019                              &    .742$\pm$.047                                 &      .730$\pm$.036                               &        .734$\pm$.036                             &      .790$\pm$.008                               &                 \textbf{.842$\pm$.024}             &          .838$\pm$.026**                  &      \textbf{.846$\pm$.042}                         &    \textbf{.842$\pm$.042}                        &    \textbf{.915$\pm$.014}                        \\
GP+MI                   & .730$\pm$.012          & .731$\pm$.021          & .727$\pm$.026          & .729$\pm$.026          & .788$\pm$.016          &          .826$\pm$.016                    &    .823$\pm$.030                        &        .831$\pm$.015                       &   .827$\pm$.015                         &        .906$\pm$.012**                   \\
MICE+MI                 & .739$\pm$.011          & .739$\pm$.026          & .739$\pm$.015          & .739$\pm$.015          & .792$\pm$.003          & .809$\pm$.018   & .816$\pm$.025 & .795$\pm$.023    & .806$\pm$.023 & .890$\pm$.012 \\
3D-MICE+MI              & .746$\pm$.028**          & .748$\pm$.045**          & .742$\pm$.028**          & .745$\pm$.028**          & .809$\pm$.022**          & .830$\pm$.011   & .828$\pm$.015 & .834$\pm$.017**    & .831$\pm$.017 & .899$\pm$.008 \\
3M-MICE+MI              & \textbf{.754$\pm$.012} & \textbf{.758$\pm$.031} & \textbf{.748$\pm$.021} & \textbf{.752$\pm$.021} & \textbf{.814$\pm$.012} & .834$\pm$.007**   & \textbf{.841$\pm$.011} & .824$\pm$.018    & .832$\pm$.018** & .905$\pm$.006 \\ \hline
\end{tabular}
\begin{tablenotes}
      \small
      \item - The best and the second-best performance are labeled with \textbf{bold} and **.
      \item +MI: The method is combined with missing indicators.
    \end{tablenotes}
\end{threeparttable}
}
\vspace{-0.1 in}
\end{table*}



\noindent\textbf{Implementation Details:}
All experiments are conducted on a 12-core machine. We use 1 iteration on multiple imputation with MICE R package \cite{buuren2010mice} for 3M-MICE, 3D-MICE, and MICE methods, and  $\alpha=0.02$ on RBF kernel with GP \cite{rasmussen2003gaussian}. In 2-step MICE, we assign $0.5$ to both $w_{11}$ and $w_{12}$ to ensure the fairness and balance the effect of MICE through cross-sectional and longitudinal view. For LSTM, we use 1 hidden layer with 128 hidden neurons, 0.005 initial learning rate, and 200 maximum sequence-length. We adopt Adam optimizer \cite{kingma2014adam} with 64 batches and 25 epochs.

==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/intro.tex <==





Sepsis,  defined as life-threatening organ dysfunction in response to infection, is the leading cause of mortality and the most expensive condition associated with in-hospital stay, accounting for more than \$24 billion in annual costs in the United States \cite{liu2014hospital}. In particular, \emph{Septic shock}, the most advanced complication of sepsis due to severe abnormalities of circulation and/or cellular metabolism \cite{bone1992definitions},  reaches a mortality rate as high as 50\% \cite{martin2003epidemiology} and the annual incidence keeps rising \cite{dellinger2008surviving}. It is estimated that as many as 80\% of sepsis deaths could be prevented with early diagnosis and intervention; indeed  prior studies have demonstrated that \emph{early diagnosis} and treatment of septic shock can significantly decrease patients' mortality and shorten their length of stay \cite{kumar2006duration,coba2011resuscitation,henry2015targeted}. Formerly, multiple complex patient health scoring systems have been defined and employed for early diagnosis and early intervention of sepsis, such as SOFA score \cite{vincent1996sofa} and MEDS \cite{shapiro2003mortality}. Despite these efforts, early diagnosis of septic shock is still a challenging problem, because of subtle but fast progression of sepsis/septic shock at early stages with lack of information.  

On the other hand, the rapid growth in volume and diversity of Electronic Health Records (EHRs), makes it possible to apply many machine learning and data mining methods for disease diagnosis. %EHRs presents great potential to guide interventions in public health and facilitates clinical decision-making such as disease management \cite{birkhead2015uses}. 
EHRs are collections of multivariate time series clinical events recorded during patients' visits. \emph{Each visit} consists of a sequence of events pertaining to the changing health status of the patient during the visit. EHRs typically acquire measurements irregularly. For example, vital signs are measured every 8 hours while lab values are measured only every 24 hours. Hence there may not be available readings for lab results when a new event is created for vital signs. Due to this integration of irregular data, EHRs usually contain high missing rates.
 % Generally speaking, there exists a variety of missing mechanisms in EHRs, such as missing completely at random (e.g., equipment failed to collect a patient's data), missing at random (e.g., patients with good vital signs may not have certain lab tests), and missing not at random (e.g., a depressed patient might refuse a depression screening) \cite{little:stat}. As a result, missing rates in EHRs can be high, 
For example, in this work, EHRs collected from general medical system, Christiana Care Health System and Mayo Clinic, have \emph{$73\%$ and $68\%$ missing rates, which are fairly typical of most real-world EHRs}. This missingness in EHRs can severely limit the application of most data mining techniques that require complete data as inputs. 

Our work further differentiates between two types of missing rates: \emph{within-visit missing rate} and \emph{cross-visit missing rate}. Essentially, the former refers to the average value of the missing portion of the data within one visit, while the latter refers to the average value of the missing portion of the data across all visits, and most existing missing rates in literature are cross-visit rates.  Table~\ref{tab:mssingrate} in section~\ref{sec:task1} shows, in EHRs some features have a higher average within-visit missing rate while others have a higher cross-visit missing rate. Our goal here is to  maximize the information extracted from limited observable records in EHRs by spontaneously leverages various dependencies  both \textit{within- and cross-visit}. 
%In this work, we further define two types of missing rates:  \emph{within-visit missing rates} vs. \emph{cross-visit missing rates}. The former refers to the average value of the missing portion of data within one visit, while the latter refers to the overall missing portion of data across all visits and most of existing missing rate are cross-visit missing rates. 

%Table~\ref{tab:mssingrate} in section~\ref{sec:task1} shows, in EHRs from one medical system, some features' average missing rates within-visit are greater than the missing rates cross-visit, and vice versa. For example, in EHRs from Mayo Clinic, missing rates within- and cross-visit of MAP are 68\% and 63\%, which of Temperature are 88\% and 91\%. Hence the latent missing patterns of EHRs may vary within- and cross-visit. Motivated by such characteristic of EHRs, we handle missingness of EHRs by integrating information from both within- and cross-visit.  
 
 
 


% To handle missingness in EHRs, various missing values imputation approaches, such as DeEp impuToR Of mIssing Temporal data (DETROIT) \cite{yan2019detroit}, and Time-aware Multi-modal Auto-Encoder (TAME) \cite{yin2020identifying} have achieved well performance. However, they require assumptions of underlying data density characteristics (e.g., sufficient neighboring observations within a sliding window) to build models, and evaluate their work on EHRs with smaller missing rates. These may not be applicable to EHRs with high missing rates (i.e., greater than 85\%) or result in undesirable performance. For example, DETROIT imputes missing values based on neural networks using observed values within a 5-length sliding window and evaluate on EHRs with 7.5\% missing rate, thus may not applicable to EHRs with high missing rates that only contains a very small number of observations within the window. Recently, TAME achieves state-of-the-art performance by incorporating multi-modal inputs (e.g., demographics, medications, lab tests of patients) to impute missing values on EHRs with 53.5\% missing rates. Though it achieves desirable performance on some features with high missing rates by leveraging information from the rest features with smaller missing rates, it's still unclear how the model would perform when EHRs are highly sparse that the information can be obtained from all features are extremely limited.     

We propose a \textbf{\emph{Time-Aware Dual-Cross-Visit missing value imputation}} approach, named \textbf{\textit{TA-DualCV}}, to impute EHRs with high missing rates. Specifically, it takes advantages of all data points within EHRs by modeling \emph{longitudinal} and \emph{multivariate} dependencies both \emph{within-visit} and \emph{cross-visit}, to resolve the high missing rates in EHRs. \emph{Multivariate dependencies} are captured among measurements across features, and \emph{longitudinal dependencies} consider the time continuity of measurements. Longitudinal dependencies can be captured from two perspectives: \emph{temporal perspective} across time-steps and \emph{time-aware perspective} across time-intervals \emph (i.e., the elapsed time from a starting point till when each event occurs). Each type of dependencies can be modeled either \emph{within-visit} or \emph{cross-visit}. The core part of TA-DualCV is the \emph{dual-cross-visit imputation} (DualCV), with which missingness can be modeled jointly at features and time steps across-visits using chained equations. In particular, it leverages cross-visit information from both feature-perspective and temporal-perspective. Additionally, we design a time-aware imputation (TA) within-visit, which captures longitudinal dependencies across the time intervals. DualCV is combined with TA visit-by-visit to ensure that dependencies are modeled across visits as well as within visits.

% EHRs generally contain two primary types of dependencies:
% 1) \emph{multivariate dependencies} among measurements across features, and 2) \emph{longitudinal dependencies} which consider the time continuity of measurements. Specifically, longitudinal dependencies can be captured from two perspectives: \emph{temporal perspective} across time-steps and \emph{time-aware perspective} across time-intervals \emph (i.e., the elapsed time from a starting point till when each event occurs). Each type of dependencies can be modeled either \emph{within-visit} or \emph{across-visits}. Different imputation approaches have been proposed for leveraging different types of dependencies. For instance, MICE \cite{buuren2010mice} captures multivariate dependencies across-visits while Gaussian process (GP) \cite{macdonald2015gpfit} captures time-aware dependencies within-visit. Recent imputation approaches such as Time-aware Multi-modal Auto-Encoder (TAME) \cite{yin2020identifying} are proposed to capture both multivariate and time-aware dependencies modeled within-visit. There has been little research to our knowledge exploring both types of dependencies within-visits and across-visits. 

% We propose a \emph{Time-Aware Dual-Cross-Sectional missing value imputation} approach, named \textit{TA-DualCS}. Specifically, it models \emph{longitudinal} and \emph{multivariate} dependencies both \emph{within-visit} and \emph{across-visits}, to resolve the intrinsic various missing mechanisms as well as high missing rates in clinical data. The core part of TA-DualCS is the \emph{dual-cross-sectional imputation} (DualCS), with which missingness can be modeled jointly at features and time steps using chained equations. In particular, it leverages a cross-visits feature-perspective (CFP) module to capture multivariate dependencies across visits, as well as a cross-visits temporal-perspective (CTP) module to capture longitudinal dependencies across visits.  
%DualCS consists of two modules that model missingness across features and time-steps jointly using chained equations. One module of DualCS is the cross-sectional feature-perspective module (CFP) which captures multivariate dependencies across-visits, while the other is the cross-sectional temporal-perspective module (CTP) which captures longitudinal dependencies from time-steps perspective across-visits. 
%Although each module focuses on modeling either multivariate or longitudinal dependency, its modeling process considers observations from different features and time-steps by using chained equations, where we call \textit{cross-sectional}.
% Additionally, we design a time-aware imputation (TA) within-visit, which uses GP to capture longitudinal dependencies across the time intervals. DualCS is combined with TA visit-by-visit to ensure that dependencies are modeled across visits as well as within visits.
% Then we design a within-visit time-aware (TA) imputation to capture longitudinal dependencies across time-intervals using GP. We augment the DualCS result with GP visit-by-visit to balance the dependencies modeled across-visits and within-visit. 

%(CFP) using chained equations to capture multivariate dependencies across-visits. Unlike existing methods that impute using observations on neighboring time-steps across features, it models missingness across features and time-steps jointly, which is so-called cross-sectional.     

% We propose the dual-cross-sectional time-aware imputation approach (named \textit{TA-DualCS}) towards clinical data. Specifically, it models \emph{longitudinal} and \emph{multivariate} dependencies both \emph{within-visit} and \emph{across-visits}, to resolve the intrinsic various missing mechanisms as well as high missing rates in clinical data. We first propose a dual-cross-sectional imputation mechanism (DualCS) to capture across-visits dependencies in both feature space (i.e., measurements across features at the same time-step) and temporal space (i.e., measurements across time-steps on the same feature) using chained equations. It does not require data to follow specific underlying density distributions, as the missingness across time-steps and features can be modeled jointly. By exploiting the underlying dependencies from both the feature and temporal space, our method can tackle high missing rates in clinical data. On the other hand, the trade-off between across-visits and within-visit dependencies is a challenge in time series data imputation. For example, a measurement from one visit can be modeled using neighboring observations within the visit (e.g., across different time-steps), or using the same feature obtained at a similar time-step across other visits. To balance this, we design time-aware imputation within each visit by GP, which shows its success in capturing temporal dependencies of clinical data in existing works \cite{luo20183d}. We augment the DualCS result with GP to capture time-interval dependencies within-visit.% The mechanism is ``personalized'' as time-interval dependencies can be varied across different patients.   
Various imputation methods have been proposed previously to handle missingness in EHRs. Based on the purpose of tasks, these prior approaches can be divided into those evaluated on \emph{unsupervised learning tasks} and those designed towards \emph{supervised learning tasks including disease diagnosis}. In the former, different approaches can be categorized into non-Neutral Network (NN)- such as 3D-MICE \cite{luo20183d} and NN-based
approaches such as DeEp impuToR Of mIssing Temporal data (DETROIT) \cite{yan2019detroit}, Time-aware Multi-modal Auto-Encoder (TAME) \cite{yin2020identifying}. Our proposed TA-DualCV is a non-NN based approach using chained equations; as a result, it does not require specific characteristics or assumptions to be followed in EHRs, such as assumptions about the underlying density distributions. For the supervised learning tasks, missing indicator (MI) \cite{little:stat} show great success in disease progression modeling~\cite{ho2014septic, fagerstrom2019lisep, lipton:missing,gao2022gradient}. However, MI cannot be directly used for unsupervised learning tasks.

% Both categories, have achieved great performance in clinical data imputation with moderate missing rate. For unsupervised learning tasks, for example, DETROIT imputes missing values based on neural networks using observed values within a 5-length sliding window and evaluate on EHRs with 7.5\% missing rate. 
% As for missing data imputation approaches for supervised learning tasks, for example, missing indicator (MI) \cite{little:stat} show great success in disease progression modeling~\cite{ho2014septic, fagerstrom2019lisep, lipton:missing}. However, MI cannot be directly used for unsupervised learning tasks.

 Our proposed TA-DualCV can be applied to both unsupervised and supervised learning tasks. Consequently, its effectiveness is assessed against the existing state-of-the-art imputation baselines that can be applied to both types of tasks. For \emph{unsupervised learning tasks}, we assess imputation performance in terms of normalized root-mean-square error (nRMSE), by masking the observations with two commonly used strategies: masking with different rates, and masking one measurement per feature per visit. For \emph{supervised learning tasks}, we utilize the imputed data incorporating Long Short-Term Memory (LSTM) network to predict septic shock 24 hours before its onset. LSTM has been shown to achieve the state-of-the-art results in many real-word applications including disease diagnosis~\cite{khoshnevisan2018recent} through deep hierarchical feature construction. Moreover, it can capture long-range dependencies in time series data in an effective manner~\cite{kim2018temporal}.

Furthermore, the robustness of TA-DualCV is evaluated on EHRs from three different medical systems. Most existing methods are evaluated by using EHRs from single medical system, such as MIMIC-III (Medical Information Mart for Intensive Care) \cite{johnson2016mimic}. As EHR characteristics across different medical systems differ dramatically\cite{khoshnevisan2020adversarial}, it is yet unclear whether existing methods will hold up across different medical systems.  To summarize, our work has at least two main contributions: 
\begin{enumerate}
    \item To handle high missing EHRs, TA-DualCV integrates both cross-visit and within-visit dependencies, by exploiting dependencies among features, time-interval, and time-steps. As far as we know, TA-DualCV is the first \emph{non-NN-based framework} designed for both unsupervised and supervised learning tasks in EHRs. 
    
    \item The generalizability and robustness of TA-DualCV are evaluated on both unsupervised imputation tasks and a supervised task, 24 hours early prediction of septic shock, using EHRs from three different medical systems. The results show that TA-DualCV outperforms state-of-the-art both non-NN- and NN-based baselines in EHRs with high missing rates.
    %Our proposed VACCINE framework does not require assumptions over underlying data characteristics including events numbers across samples, sampling distribution, or substantial observed values. It outperforms imputation baselines on three real-world clinical datasets, containing different types of features and masking rates, for early prediction of septic shock.   
   % \item Our proposed work does not require assumptions over types of missingness (e.g., missing completely at random). As a result, it outperforms imputation baselines on the data with mixed types of missingness.  
\end{enumerate} 



\begin{table*}[t]
\caption{Characteristics of Existing Approaches vs. TA-DualCV}

\label{tab:prelim}
\centering
\begin{threeparttable}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lc|cccc}
\hline
Type & Approach      & Native Missing Rate                       & Tensor Shape                      & Sliding Window               & Prefill                 \\ \hline \hline
Non-NN-Based & MICE (2010)& 17\% & No & No & No \\
& 3D-MICE (2018) & 17\% & No & No & No \\ \hline
NN-Based & BRITS (2018) & 78\% & 	\cellcolor{Gray}Yes & No & \cellcolor{Gray}Yes \\
& DETROIT (2019) & 7\% & 	No & 	\cellcolor{Gray}Yes & \cellcolor{Gray}Yes \\
& GP-VAE (2020) & 78\% & \cellcolor{Gray}Yes &No & No \\
& CATSI (2020) & 7\% & No & No & \cellcolor{Gray}Yes \\
& TAME (2020) & 54\% & \cellcolor{Gray}Yes & No & No \\ \hline
Non-NN-Based & TA-DualCV (Ours)    & 73\% & No & No & No \\ \hline
\end{tabular}
% }
\begin{tablenotes}
\footnotesize
    \item - Native missing rate: it refers to the cross-visit native missing rate of the selected features in the original work. If the approach is evaluated on more than one EHRs, we report the highest one.
    \item - For NN-based approaches, BRITS, CATSI, and TAME are bidirectional NN-based approaches and TAME achieves the best performance. Also, DETROIT is recognized as a strong baseline in~\cite{yin2020identifying}. Thus we use TAME and DETROIT as NN-based baselines in this study. GP-VAE requires tensor-shape input, thus cannot produce results under our EHRs with varied numbers of events across visits.
\end{tablenotes}
\end{threeparttable}
\end{table*}


% Such missingness in EHRs can severely limit the application of most data mining techniques that require complete data as inputs and thus various missing data imputation approaches have been proposed. Based on the purpose of tasks, missing data imputation approaches can be divided into those designed towards \emph{supervised learning tasks} and those evaluated on \emph{unsupervised learning tasks} only. In the former, for example, mean-filling and missing indicator (MI) \cite{little:stat} show success in disease progression modeling (e.g., \cite{ho2014septic}). In the latter, 3D-MICE \cite{luo20183d} and DeEp impuToR Of mIssing Temporal data (DETROIT) \cite{yan2019detroit} have achieved promising performance in clinical data imputation. Despite the success, few of them are proposed towards and evaluated on both tasks in healthcare domain. 





    

% 1) masking 20\%, 50\%, 60\%, 70\%, 80\%, and 90\% of observed values as test sets respectively; 2) imputing native missing values to predict whether patients will get septic shock. 
%Our model is compared against three state-of-art approaches, 3D-MICE \cite{luo20183d}, MICE \cite{buuren2010mice}, and GP \cite{macdonald2015gpfit}, and one expert baseline. Our approach ensures higher levels of flexibility by considering both cross-sectional and longitudinal correlations within clinical data, without truncating data into a tensor. Meanwhile, our model outperforms the state-of-the-art benchmarks in terms of both nRMSE and septic shock early prediction performance.


%%% Brief intro of our result and contribution

%%%Ge: stress the 2-step mice -> traditional one is not enough (), GP: noise and uncertainty of data
%abstract + 1st paragraph: 2 terms contribute to the approach
%health care: missing at random, not random, ... <- EHR mixed
%little previous work in longitudinal + cross- in EHR, longitudinal: temporal irregular, cross-sectional: not considerable in state-of-art
%For example: EHR contains longi and cross characteristics 


%%% 
% The remainder of the paper is organized as follows. Section II presents a brief review of previous work by researchers to impute longitudinal multivariate missing data. Section III describes the design of our 3M-MICE model. In section IV, we show details of our experiments, including datasets, data preprocessing, and benchmark selection. Section V shows our experimental results, followed by section VI that concludes with a few remarks.

==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/method.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{sections/figure/TA-DualCS.png}
    \caption{Schematic of TA-DualCV. It consists of two parts: 1) Dual-cross-visit (DualCV) imputation that consists of cross-visits feature-perspective (CFP) and cross-visits temporal-perspective (CTP) modules. We get complete data from a compromise layer which combines two separate results from both modules; 2) Within-visit time-aware imputation (TA). The result from DualCV is augmented visit-by-visit with result from TA.}
    \label{fig:vaccine}
\end{figure}

% \subsection{VACCINE Framework Overview}
Figure~\ref{fig:vaccine} shows the architecture of TA-DualCV.
Specifically, a dual-cross-visit (DualCV) imputation method imputes the missing data using features and temporal dependencies, respectively, then the results from two streams are fused together. The results from DualCV are augmented with GPs which consider the within-visit time-aware dependencies, to constitute the final imputation results. We are releasing the source code of our implementation freely to the research community and it can be accessed at \texttt{\url{https://github.com/fay067/TA-DualCV}}. %Our architecture is designed to handle the following factors and challenges. 

\subsection{Problem Formulation}
\subsubsection{EHRs Imputation}
EHRs can be represented as  $\mathbf{X} = \{\mathbf{X}_1, ..., \mathbf{X}_N\}$, where $N$ is the total number of hospital visits. Each visit $\mathbf{X_i}$ consists of a sequence of events: $\mathbf{X_i} = \{\mathbf{{X}}_{i, 1, \cdot},..., \mathbf{{X}}_{i, T_i, \cdot}\}$ where $\mathbf{{X}}_{i, j, \cdot}\in\mathbb{R}^D$ represents an event recording measurements across $D$ features at time step $j$ in patient $i$'s record. $T_i$ is the number of events (i.e., time-steps) in visit $i$ that can vary across different visits. %Specifically, $\mathbf{{X}}_{i, j, \cdot}\in\mathbb{R}^D$, where $D$ is the number of features (measurements) recorded. 
Each visit $i$ is also associated with a vector $\mathbf{\mathcal{T}}_i = (\tau_{i,1},...,\tau_{i,T_i}) \in\mathbb{R}^{T_i}$ recording the time intervals (e.g., minutes) from a starting point (e.g., patient arrival time) till when each event occurs. Moreover, the events of $\mathbf{X_i}$ are in ascending order of the time intervals. In practice, $\mathbf{X}_i$ may contain unknown \textit{native missing values} due to the irregular data collection process. We apply additional masks to the observed data which introduce \textit{masked missing values} with known groundtruth. Our goal is to devise an imputation model $f$ which generates complete multivariate time series $\mathbf{\hat{X}}$: $\mathbf{\hat{X}} = f(\mathbf{X}, \mathbf{\mathcal{T}})$.

% \noindent1) We adapt chained equations to exploit underlying information from the feature space across visits to generate imputations capturing dependencies among features within the sample population. This approach does not require data to follow specific characteristics, such as the events numbers across different samples or assumptions over underlying density distributions, as the missingness across events and features can be modeled jointly.  

% \noindent2) One challenge in multivariate time series clinical data imputation is that EHRs from general emergency departments can be highly sparse while existing cross-visit temporal imputation techniques require substantial observed values within neighbors of a missing measurement \cite{zhang2020predicting, xu2020multi}. To address this, DualCV is designed to capture the temporal dependencies underlying missingness, as opposed to existing methods that only consider dependencies across features (e.g., MICE~\cite{buuren2010mice}). By exploiting the underlying information from both the feature and temporal space, our framework can work with data with high missing rates.

% \noindent3) Another challenge in time series data imputation is the trade-off between cross-visit and within-visit dependencies. For example, a measurement from one visit can be modeled using neighboring observations within the visit (e.g., across different time-steps), or using the same feature obtained at a similar time-step across other visits in the sample population. To balance this, we design time-aware imputation within each visit by GP, which shows its success in capturing temporal dependencies in existing works \cite{luo20183d, fortuin2020gpvae}, and augment the imputations output from DualCV accordingly.

% \subsection{Base Methods}
% \textbf{Chained Equations.}
% %% MICE
% Generally, chained equation methods address missing data issues by exploiting and modeling the dependencies among variables in features. \cite{van2000multivariate, buuren2010mice}. 
% % Its fully conditional specifications and sequential regression would create multiple imputations, as opposed to single imputations that accounts for the statistical uncertainty in the imputations. 
% They can be used to handle different types of variables (e.g., discrete or continuous) as well as complexities such as bounds or survey skip patterns. 
% % Different software implementations of MICE employ different distributions to impute the missing values. 
% Specifically, in this work, we consider multiple imputations with chained equations (MICE) which estimates missing data from a joint distribution by Gibbs sampler \cite{buuren2010mice}, as it provides faster convergence speed over other Markov Chain Monte Carlo based techniques \cite{van2006fully}. 
% % The sampling-based MICE assumes that 
% Specifically, the hypothetically complete data $M$ can be modeled as a random variable sampled from a $p$-variate multivariate distribution $P(M|\rho)$, where $\rho$ is a vector of unknown parameters. The chained equations obtain a posterior distribution of $\rho$ by sampling iteratively from $P(M_v|M_{-v}, \rho_v)$ for all $v=1,2,...,p$. The $i$th iteration of the chained equation is a Gibbs Sampler that takes:
% \begin{equation}
% \begin{aligned}
%     \rho_v^{*(i)} \sim P(\rho_v|M_v, M_1^{(i-1)},..., M_{v-1}^{(i-1)}, M_{v+1}^{(i-1)},..., M_p^{(i-1)}) \\
%     M_v^{*(i)} \sim P(M_v|M_v, M_1^{(i-1)},..., M_{v-1}^{(i-1)}, M_{v+1}^{(i-1)},..., M_p^{(i-1)}, \rho_v^{*(i)})
% \end{aligned}
% \end{equation}
% where $\hat{M}_v^{(i)}=(M_v, M_v^{*(i)})$ is the complete data of variable $v$ at iteration $i$.

% %Traditionally, MICE are only implemented from single perspective, while our approach dual-cross-sectionally utilize MICE on two dimensions cross sample population within multivariate time series clinical data, features and time-intervals. To avoid confounding between the conventional MICE implementation and our approach, we will describe our dual-cross-sectional MICE in details within the following sections.

% %% GP

% \noindent\textbf{Gaussian Process (GP).}
% % In this work, we follow the GP modeling approach by MacDonald et al. \cite{macdonald2015gpfit}. 
% % Taking continuous variables as input, GP modeling approach fits GP model to the output by scalar valued deterministic simulators. 
% GP is used to exploit the time-interval dependencies behind missingness.
% % assumes that the closer the data-points are, the feature values of them are also closer. 
% Specifically, for each visit, a univariate time series $\mathbf{\Delta t}_{i}=(\Delta t_{i,1},...,\Delta t_{i, t_i}), i=1,...,D,$ is a $t_i$-dimensional vector generated with each feature $i$. The simulator output $y(\Delta t_{i})$ is denoted as: 
% \begin{equation}\label{GP:1}
%     y(\Delta t_{i})=\mu + z(\Delta t_{i})
% \end{equation}
% where $\mu$ is overall mean and $z(\Delta t_{i})$ is a GP that we assume to reach a local optima on its covariance structure:
% \begin{equation}\label{GP:2}
%     Cov(z(\Delta t_{i}), z(\Delta t_{j}))=\sigma_{z}^2 R_{ij}
% \end{equation}
% In general, $y(T) = (y(\Delta t_{1}),...,y(\Delta t_{D}))^{\top}$ has a multivariate normal distribution. 
% % As what MacDonald et al. proposed in their work, 
% We specifically follow the Gaussian correlation function defined by Ranjan et al.~\cite{ranjan2011computationally}:
% \begin{equation}
%     R_{ij} = \prod_{k=1}^{t_i} exp\{-\alpha_{k} \mid \Delta t_{i,k}-\Delta t_{j,k} \mid ^2\}  \mbox{ for all }  i,j
% \label{eq:R-matrix}
% \end{equation}
% where $\alpha=(\alpha_1,...,\alpha_{t_i})$ is a vector of hyperparameters.



\subsection{DualCV Imputation}
%EHRs from general emergency departments can be highly sparse while existing cross-visit temporal imputation techniques require substantial observed values within neighbors of a missing measurement \cite{xu2020multi}. To address this, DualCV is designed to capture the temporal dependencies underlying missingness, as opposed to existing methods that only consider dependencies across features (e.g., \cite{buuren2010mice}). We adapt chained equations to exploit underlying information from the feature space cross-visit to generate imputations capturing dependencies among features. This approach does not require data to follow specific characteristics, such as the assumptions over underlying density distributions, as the missingness across events and features can be modeled jointly.

DualCV is designed to capture multivariate and temporal dependencies cross-visit, using chained equations. Chained equations are advantageous here because they do not require specific characteristics or assumptions to be followed, such as assumptions about the underlying density distributions. Specifically, we design two chained equation based modules, a CFP module to capture multivariate dependencies cross-visit, as well as a CTP module to capture longitudinal dependencies from temporal perspective cross-visit. We combine the results from the two modules to obtain imputation results, where we call dual-cross-sectional. 
% Instead, it models the missingness across time-steps and features jointly, where we call cross-sectional.    
%The strength of chained equations is it does not require data to follow specific characteristics, such as the assumptions over underlying density distributions, as the missingness across events and features can be modeled jointly.

\subsubsection{Cross-Visits Feature-Perspective Module (CFP)} 
\label{subsec:mice_feature}
To apply CFP, we first transform the data $\mathbf X$ into a single matrix $\mathbf{\Psi} = (\mathbf{X}_{1, \cdot, \cdot},$ $...,\mathbf{X}_{N, \cdot, \cdot})^{\top}$ by concatenating $N$ visits on all features, where we then denote $\mathbf{\Psi}_{j,\cdot}$ as the measurements on $j$-th event and $\mathbf{\Psi}_{\cdot, k}$ represents measurements on $k$-th feature (e.g., white blood cell count), as shown in the Figure \ref{fig:vaccine} (CFP). Each visit can contain different numbers of events and time-intervals between any pair of consecutive events can be different. $\mathbf{\Psi} = (\mathbf{\Psi}_{\cdot, 1},..., \mathbf{\Psi}_{\cdot, D})$ represents the observed part and $\mathbf{\Psi}^{imp} = (\mathbf{\Psi}_{\cdot, 1}^{imp},$ $...,$ $\mathbf{\Psi}_{\cdot, D}^{imp})$ represents the missing part of the visits to be imputed. The predictors of $\mathbf{\Psi}_{\cdot, k}$ is denoted as $\mathbf{\Psi}_{\cdot, -k}=(\mathbf{\Psi}_{\cdot, 1},..., \mathbf{\Psi}_{\cdot, k-1},$ $ \mathbf{\Psi}_{\cdot, k+1},$ $...,$ $\mathbf{\Psi}_{\cdot, D})$ showing the collection of measurements on the $(D-1)$ features except feature $k$. $\mathbf{\Psi}_{\cdot, -k}$ can be incomplete and the correlation between any pair of $\mathbf{\Psi}_{\cdot, k}$ and $\mathbf{\Psi}_{\cdot, -k}$ can be complex (e.g. nonlinear). Therefore, the hypothetically complete data $\mathbf{\hat{\Psi}}=(\mathbf{\hat{\Psi}}_{\cdot, 1},...,\mathbf{{\hat{\Psi}}}_{\cdot, D})$ can be sampled from the $D$-variate multivariate distribution $P(\mathbf{\Psi}_{\cdot, 1},$ $...,\mathbf{\Psi}_{\cdot, D} \mid \gamma)$ where $\gamma$ are parameters \cite{buuren2010mice}. Then the chain equations are designed to get the posterior distribution of $\gamma$ by sampling iteratively from the conditional distribution
\begin{equation} \label{e1.1}
\begin{aligned}
P(\mathbf{\Psi}_{\cdot, 1}\mid \mathbf{\Psi}_{\cdot, -1}, \gamma_1) 	\dots
P(\mathbf{\Psi}_{\cdot, D}\mid \mathbf{\Psi}_{\cdot, -D}, \gamma_D).
\end{aligned}
\end{equation}
% Similar to MICE \cite{buuren2010mice}
Specifically, the $t$-th iteration of chained equations is a Gibbs sampler which draws:
\begin{equation}
\begin{aligned}
& \gamma_1^{imp(t)} \sim P(\gamma_1 \mid \mathbf{\Psi}_{\cdot, 1}, \mathbf{\Psi}_{\cdot, -1}^{t-1}), \\
& \mathbf{\Psi}_{\cdot, 1}^{imp(t)} \sim P(\mathbf{\Psi}_{\cdot, 1} \mid \mathbf{\Psi}_{\cdot, 1}, \mathbf{\Psi}_{\cdot, -1}^{t-1}, \gamma_1^{imp(t)}), \\
& \vdots \\
& \gamma_D^{imp(t)} \sim P(\gamma_D \mid \mathbf{\Psi}_{\cdot, D}, \mathbf{\Psi}_{\cdot, -D}^{t-1}), \\
& \mathbf{\Psi}_{\cdot, D}^{imp(t)} \sim P(\mathbf{\Psi}_{\cdot, D} \mid \mathbf{\Psi}_{\cdot, D}, \mathbf{\Psi}_{\cdot, -D}^{t-1}, \gamma_k^{imp(t)}).
\end{aligned}
\end{equation}
$\mathbf{\hat{\Psi}}_{\cdot, k}^{t} = (\mathbf{\Psi}_{\cdot, k}, \mathbf{\Psi}_{\cdot, k}^{imp(t)})$ is defined as the complete data of $k$-th feature across visits at iteration $t$. Thus, $\mathbf{\hat{\Psi}}^{t} = (\mathbf{\hat{\Psi}}_{\cdot, 1}^{t},...,$ $\mathbf{\hat{\Psi}}_{\cdot, D}^{t})$ is the complete data after $t$-th iteration.

\subsubsection{Cross-Visits Temporal-Perspective Module (CTP)}
\label{subsec:mice_long}
To apply CTP, we then re-formulated the data $\mathbf X$ into $D$ matrices $\mathbf{\Phi}=\{\mathbf{\Phi}_1,...,\mathbf{\Phi}_D\}$ by transposing each visit $\mathbf{X}_i$ and concatenating $N$ visits over the time-steps (e.g., $1,...,T_i$) as shown in Figure ~\ref{fig:vaccine} (CTP). We fix the number of events for each visit to $T^{med}$, which denotes the median value of $\{T_i| i \in [1,N]\}$.  Thus, $\mathbf{\Phi}_j \in \mathbb{R}^{N \times T^{med}}$ denotes the matrix recording measurements on $j$-th feature, where $\mathbf{\Phi}_{j(i,\cdot)}$ represents measurements of $i$-th visit on $j$-th feature and $\mathbf{\Phi}_{j(\cdot,m)}$ represents measurements of the $m$-th time-step on $j$-th feature. If the number of time-steps within a record is less than $T^{med}$, the visit is padded to $T^{med}$ by filling with placeholder values representing missingness (e.g., NaN's). If the number of time-steps is greater than $T^{med}$, the length of the visit is truncated to $T^{med}$ from the front. The reason we use median values is that it is not sensitive to outliers. Also, as the computational complexity of chained-equation based algorithms is directly correlated with the number of variables~\cite{buuren2010mice}, by using median it can balance between efficiency and the number of variables.

Similar to the first step described in Section \ref{subsec:mice_feature}, we apply chained equations on each $\mathbf{\Phi}_j$ separately. Specifically, measurements on the $m$-th time-step of $j$-th feature is denoted by $\mathbf{\Phi}_{j(\cdot,m)}$ while its complementary part is denoted as $\mathbf{\Phi}_{j(\cdot,m)}^{imp}$ which is missing and subjected to imputation. The complete data (i.e., after imputation) on $j$-th feature is denoted as $\mathbf{\hat{\Phi}}_j=(\mathbf{\hat{\Phi}}_{j(\cdot,1)},...,$ $\mathbf{\hat{\Phi}}_{j(\cdot,T^{med})})$ which can be sampled from the $T^{med}$-variate multivariate distribution $P(\mathbf{\Phi}_{j(\cdot,1)},...,\mathbf{\Phi}_{j(\cdot,T^{med})} \mid \beta)$. The conditional distributions used to obtain the posterior distribution of $\mathbf{\Phi}_j$, parametrized by $\beta$, are
\begin{equation}
\begin{aligned}
& P(\mathbf{\Phi}_{j(\cdot, 1)}\mid \mathbf{\Phi}_{j(\cdot, -1)}, \beta_1)
,\dots, \\
& P(\mathbf{\Phi}_{j(\cdot, T^{med})}\mid \mathbf{\Phi}_{j(\cdot, -T^{med})}, \beta_{T^{med}}),
\end{aligned}
\end{equation}
where $\mathbf{\Phi}_{j(\cdot, -m)} = (\mathbf{\Phi}_{j(\cdot, 1)},...,\mathbf{\Phi}_{j(\cdot, m-1)},\mathbf{\Phi}_{j(\cdot, m+1)},...,$ $\mathbf{\Phi}_{j(\cdot, T^{med})})$. Then the Gibbs sampler is used to sample $\beta$ and $\mathbf{\Phi}_j$ iteratively following the chained equations, at the $s$-th iteration, as
\begin{equation}
\small
\begin{aligned}
& \beta_1^{imp(s)} \sim P(\beta_1 \mid \mathbf{\Phi}_{j(\cdot, 1)}, \mathbf{\Phi}_{j(\cdot, -1)}^{s-1}), \\
& \mathbf{\Phi}_{j(\cdot, 1)}^{imp(s)} \sim P(\mathbf{\Phi}_{j(\cdot, 1)} \mid \mathbf{\Phi}_{j(\cdot, 1)}, \mathbf{\Phi}_{j(\cdot, -1)}^{s-1}, \beta_1^{imp(s)}), \\
& \vdots \\
& \beta_{T^{med}}^{imp(s)} \sim P(\beta_{T^{med}} \mid \mathbf{\Phi}_{j(\cdot, T^{med})}, \mathbf{\Phi}_{j(\cdot, -T^{med})}^{s-1}), \\
& \mathbf{\Phi}_{j(\cdot, T^{med})}^{imp(s)} \sim P(\mathbf{\Phi}_{j(\cdot, T^{med})} \mid \mathbf{\Phi}_{j(\cdot, T^{med})}, \mathbf{\Phi}_{j(\cdot, -T^{med})}^{s-1}, \beta_{T^{med}}^{imp(s)}).
\end{aligned}
\end{equation}
$\mathbf{\hat{\Phi}}_{j(\cdot, m)}^{s} = (\mathbf{\Phi}_{j(\cdot, m)}, \mathbf{\Phi}_{j(\cdot, m)}^{imp(s)})$ is the complete data on $j$-th feature $m$-th time-step at iteration $s$. Then the complete (i.e., imputed) data on $j$-th feature, after the $s$-th iteration, is obtained as $\mathbf{\hat{\Phi}}_j^{s} = (\mathbf{\hat{\Phi}}_{j(\cdot, 1)}^{s},...,\mathbf{\hat{\Phi}}_{j(\cdot, T^{med})}^{s})$.


\subsubsection{Compromising Layer}
We now have two complete results, $\mathbf{\hat{\Psi}}$ and $\mathbf{\hat{\Phi}}$, obtained using CFP and CTP which considers the dependencies captured from the feature and temporal space respectively. Then $\mathbf{\hat{\Psi}}$ and $\mathbf{\hat{\Phi}}$ are fused together to constitute the complete data $\mathbf{\hat{X}}^{M}$. Specifically, the value on $i$-th visit, $j$-th time-step, and $k$-th feature of $\mathbf{\hat{X}}^{M}$, $\hat{X}_{i,j,k}^{M}$, is obtained as following
\begin{equation}
\begin{aligned}
\hat{X}_{i,j,k}^{M} = [w_1\hat{\Psi}_{\sum_{x=1}^{i-1}T_x, k}^t + w_2\hat{\Phi}_{k(i,j)}^s]\mathds{1}\{T_i \le T^{med}\} \\
+ \hat{\Psi}_{\sum_{x=1}^{i-1}T_x, k}^t\mathds{1}\{T_i > T^{med}\},
\end{aligned}
\end{equation}
where $\mathds{1}$ is indicator function, $w_1$ and $w_2$ are hyperparameters \textit{s.t.} $w_1 + w_2 = 1$. 



\subsection{Within-Visit Time-Aware Augmenting Mechanism}
%Another challenge in time series data imputation is the trade-off between cross-visit and within-visit dependencies. For example, a measurement from one visit can be modeled using neighboring observations within the visit (e.g., across different time-steps), or using the same feature obtained at a similar time-step across other visits in the sample population. To balance this, we design time-aware imputation within each visit by GP, which shows its success in capturing temporal dependencies of clinical data in existing works \cite{luo20183d}. It augments the imputations output from DualCV accordingly.
Besides DualCV, which captures the feature and temporal dependencies \textit{across} visits, we employ GP to perform time-aware imputations on each visit to capture patient-specific correlations \textit{within} each visit. The difference between CTP and within-visit time-aware imputation is that CTP focuses on ``outer" dependencies among time-steps of events across samples within population, while GP captures the ``inner" dependencies among time-intervals of events within each visit. 

Specifically, we apply single-task GP imputation over each feature on visit $\mathbf{X}_i$ individually. % For $\mathbf{X}_i$, a univariate time series $\mathbf{\mathcal{T}}_{i}=(\tau_{i,1},...,\tau_{i, T_i})$ is a $T_i$-dimensional vector generated with each visit $i$. 
% The simulator output $y(\mathbf{\mathcal{T}}_{i})$ is denoted as: 
% \begin{equation}\label{GP:1}
%     y(\mathbf{\mathcal{T}}_{i})=\mu + z(\mathbf{\mathcal{T}}_{i})
% \end{equation}
% where $\mu$ is overall mean and $z(\mathbf{\mathcal{T}}_{i})$ is a GP that we assume to reach a local optima on its covariance structure:
% \begin{equation}\label{GP:2}
%     Cov(z(\mathbf{\mathcal{T}}_{i}), z(\mathbf{\mathcal{T}}_{j}))=\sigma_{z}^2 R_{ij}
% \end{equation}
% In general, $y(\mathbf{\mathcal{T}}) = (y(\mathbf{\mathcal{T}}_{1}),...,y(\mathbf{\mathcal{T}}_D))^{\top}$ has a multivariate normal distribution. 
% We specifically follow the Gaussian correlation function defined by Ranjan et al.~\cite{ranjan2011computationally}:
% \begin{equation}
%     R_{ij} = \prod_{k=1}^{t_i} exp\{-\alpha_{k} \mid \tau_{i,k}-\tau_{j,k} \mid ^2\}  \mbox{ for all }  i,j
% \label{eq:R-matrix}
% \end{equation}
% where $\alpha=(\alpha_1,...,\alpha_{t_i})$ is a vector of hyperparameters.
The observed data on the $l$-th feature of visit $\mathbf{X}_i$ is denoted as $\mathbf{X}_{i,\cdot,l}$, with $\mathbf{X}_{i,\cdot,l}^{imp}$ representing its complementary missing part which is subject to be imputed. 
For $l$-th feature, we split the time-interval vector $\mathbf{\mathcal{T}}_i^{(l)}$ into $\mathbf{\mathcal{T}}_i^{obs(l)}$ and $\mathbf{\mathcal{T}}_i^{imp(l)}$, where $\mathbf{\mathcal{T}}_i^{obs(l)}$ and $\mathbf{\mathcal{T}}_i^{imp(l)}$ denote the time-intervals corresponding to $\mathbf{X}_{i,\cdot,l}$ and $\mathbf{X}_{i,\cdot,l}^{imp}$ respectively.
The target output $\mathbf{X}_{i,\cdot,l}^{imp}$ is modeled as:
\begin{equation}\label{GP:1}
    \mathbf{X}_{i,\cdot,l}^{imp}=\mu + z(\mathbf{\mathcal{T}}_i^{imp(l)})
\end{equation}
where $\mu$ is overall mean and $z(\mathbf{\mathcal{T}}_i^{imp(l)})$ is a GP that we assume to reach a local optima on its covariance structure:
\begin{equation}\label{GP:2}
    Cov(z(\mathbf{\mathcal{T}}_i^{imp(l)}), z(\mathbf{\mathcal{T}}_i^{imp(m)}))=\sigma_{z}^2 R_{lm}
\end{equation}
In general, $\mathbf{X}_{i,\cdot,l}^{imp} = (\mathbf{X}_{i,\cdot,1}^{imp},...,\mathbf{X}_{i,\cdot,D}^{imp})^{\top}$ has a multivariate normal distribution. 
We specifically follow the Gaussian correlation function defined by Ranjan et al.~\cite{ranjan2011computationally}:
\begin{equation}
    R_{lm} = \prod_{k=1}^{t_i} exp\{-\alpha_{k} \mid \mathbf{\mathcal{T}}_{i,k}^{imp(l)}-\mathbf{\mathcal{T}}_{i,k}^{imp(m)} \mid ^2\}  \mbox{ for all }  l,m
\label{eq:R-matrix}
\end{equation}
where $\alpha=(\alpha_1,...,\alpha_{t_i})$ is a vector of hyperparameters.

According to the Equations \ref{GP:1}, \ref{GP:2}, and \ref{eq:R-matrix}, we can use $(\mathbf{\mathcal{T}}_i^{obs(l)}, \mathbf{X}_{i,\cdot,l}^{obs})$ to fit GP and estimate the $\alpha$ following the negative profile log-likelihood \cite{macdonald2015gpfit} 
\begin{equation}
\small
\begin{aligned}
-2 & log(L_\alpha)  \propto \\
& log(\mid R\mid) + nlog [(\mathbf{X}_{i,\cdot,l}^{obs} - \mathbf{1_n}\hat{\mu}(\alpha))^\top R^{-1}(\mathbf{X}_{i,\cdot,l}^{obs} - \mathbf{1_n}\hat{\mu}(\alpha))],
\end{aligned}
\end{equation}
where $\mid$$R$$\mid$ denotes the determinant of the Gaussian correlation function R defined in~\eqref{eq:R-matrix}. Then we can get the predicted $\mathbf{X}_{i,\cdot,l}^{imp}$ by evaluating the GP model with input $\mathbf{\mathcal{T}}_i^{imp(l)}$. Finally, we can obtain the complete (i.e., imputed) data of visit $i$ as $\mathbf{\hat{X}}_i^G = (\mathbf{{X}}_i, \mathbf{X}_i^{imp})$ which constitutes the imputed dataset $\mathbf{\hat{X}}^G=(\mathbf{\hat{X}}_1^G,...,\mathbf{\hat{X}}_N^G)$.

Finally, we augment the results from DualCV with the outputs from GP through weighted averaging $\mathbf{\hat{X}}_i = \mathbf{\theta}_{i,1}\cdot\mathbf{\hat{X}}_i^M +  \mathbf{\theta}_{i,2}\cdot\mathbf{\hat{X}}_i^G$, where $\mathbf{\theta}_{i,1}=\frac{\sigma_{G_i}}{\sigma_{M_i} + \sigma_{G_i}}$,  $\mathbf{\theta}_{i,2}=\frac{\sigma_{M_i}}{\sigma_{M_i} + \sigma_{G_i}}$, $\sigma_{M_i}$ and $\sigma_{G_i}$ are the standard deviations of the imputations output from DualCV and within-visit time-aware imputations given visit $i$, respectively. Note the weight is designed to penalize the results (either from DualCV or GP) that are associated with the larger standard deviations. 





==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/prelim.tex <==

\begin{definition}[\textbf{Multivariate Time Series Clinical Data}]
\label{def:data}


\textit{
A multivariate time series clinical data can be represented as  $\mathbf{X} = \{\mathbf{X_1}, ..., \mathbf{X_N}\}$, where $N$ is the total number of hospital visits. Each visit $\mathbf{X_i}$ consists of a sequence of events: $\mathbf{X_i} = \{\mathbf{{X}}_{i, 1, \cdot},..., \mathbf{{X}}_{i, t_i, \cdot}\}$ where $\mathbf{{X}}_{i, j, \cdot}$ represents a patient $i$'s record at time step $j$ in $\mathbf{X_i}$ and $t_i$ is number of events in visit $i$ which can vary across different visits. Specifically, $\mathbf{{X}}_{i, j, \cdot}\in\mathbb{R}^D$, where $D$ is the number of features recorded. Each visit $i$ is also associated with a vector $\mathbf{\Delta t}_i\in\mathbb{R}^{t_i}$ recording the time interval (e.g., minutes) from a starting point (e.g., patient arrival time) till when each event occur. Moreover, $\mathbf{X_i}$ satisfies the condition that events are ordered increasingly according to time steps. 
}
\end{definition}


\begin{definition}[\textbf{Native and Masked Missing Values}]
\textit{
In practice, $\mathbf{X}_i$ may contain native missing values without groundtruth due to the irregular data collection process. To evaluate imputation performance, we apply additional masks to the observed data which introduce masked missing values with known grondtruth.
}
\end{definition}

\noindent\textit{Problem Statement.} \textbf{Multivariate Time Series Clinical Data Imputation.} Given a multivariate time series clinical data $\mathbf{X} = \{\mathbf{X_1}, ...,$ $\mathbf{X_N}\}$, which contain missing values, with the corresponding time-interval vectors $\mathbf{\Delta t}=\{\mathbf{\Delta t}_1,...,\mathbf{\Delta t}_N\}$, devise an imputation model $f$ which outputs complete multivariate time series $\mathbf{\hat{X}}$: $\mathbf{\hat{X}} = f(\mathbf{X}, \mathbf{\Delta t})$.


==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/result.tex <==


%%%% imputation result: MIMIC-III




% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.6]{sections/figure/ave-nrmse.png}
%     \caption{Imputation accuracy (average nRMSE) for the MIMIC-III dataset}
%     \label{fig:ave-nrmse}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.27]{sections/figure/scatter-hct.png}
%     \caption{Accuracy of Hematocrit predictions and prediction intervals width, scatter plot; Horizontal and vertical lines: normal reference limits; The less accurate predictions, the bluer color of the points}
%     \label{fig:hema}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.27]{sections/figure/scatter-hgb.png}
%     \caption{Hemoglobin}
%     \label{fig:hemo}
% \end{figure}




In this section, we compare the imputation performance of our proposed 3M-MICE approach against various baselines in two experimental settings: First, we evaluate the effectiveness of each model in imputation of the masked values by varying the masking ratio in terms of nRMSE. Second, we investigate the ability of 3M-MICE in capturing rich correlations among longitudinal and cross-sectional information in clinical data by assessing the performance of a prediction model trained on the imputed data generated by each algorithm.

\vspace{-0.1 in}

\subsection{Various Masking Rates on Observations}
In this setting, \textit{nRMSE} is used to evaluate the imputation of masked observations. We compare our approach to 4 baselines on one real-world data, MIMIC-III, with 6 masking rates. The results \footnote{Numeric results of nRMSE are attached in supplementary} in Fig.\ref{fig:nrmse} show that our imputation model outperforms the baselines with smaller nRMSE on each measurement and overall data across all masking rates. Specifically, our model is more capable with high masking rates (e.g., 90\%) with an average 0.227 nRMSE across measurements, which is 13\% better than 3D-MICE (i.e., 0.261), 23\% better than MICE (i.e., 0.296), 21\% better than GP (i.e., 0.288), and 18\% better than expert baseline (i.e., 0.278). 
%Also, from the Fig.\ref{fig:nrmse}, our model is more stable with increasing masking rates above 50\% masking rates with average nRMSE 

\vspace{-0.1 in}

\subsection{Septic Shock Early Prediction}
In this setting, evaluation metrics are used to evaluate the performance of each model for prediction of septic shock 8 hours before the onset on 2 real-world EHR datasets: CCHS and Mayo. We compare our approach against four imputation baselines and in two settings: with or without missing indicators (MI). The results in Table.\ref{tab:pred} show that 3M-MICE outperforms all the baselines in both experimental settings by achieving the highest accuracy, recall, precision, F1, and AUC on CCHS dataset, and outperforms all baselines be achieving highest accuracy, recall, F1, and AUC without missing indicator on Mayo dataset. Specifically, 3M-MICE always performs better on recall, which means it less miss-identifies shock positive patients as negative, while false negative can be costly in practice. This result further demonstrates the importance of capturing rich correlations among both longitudinal and cross-sectional information and the effectiveness of 3M-MICE in imputing missing values to prepare data for building complex prediction models.





==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/table/char.tex <==

\begin{table}[tbp]
 \scriptsize
\centering
\begin{threeparttable}
\caption{Missing Rates of Selected Measurement across Three Datasets}
\label{table:char}
\begin{subtable}{0.50\textwidth}
\begin{tabular}{l|lcc}
\hline
Lab Analytes & ItemID & OMR   & PMR   \\ \hline
Chloride   & 50902  & 0.258 & 0.022 \\
Potassium  & 50971  & 0.210 & 0.020 \\
Bicarb     & 50882  & 0.271 & 0.025 \\
Sodium     & 50983  & 0.244 & 0.021 \\
Hematocrit & 51221  & 0.181 & 0.116 \\
Hemoglobin & 51222  & 0.304 & 0.138 \\
MCV        & 51250  & 0.308 & 0.140 \\
Platelet   & 51265  & 0.279 & 0.134 \\
WBC        & 51301  & 0.303 & 0.136 \\
RDW        & 51277  & 0.309 & 0.000 \\
BUN        & 51006  & 0.259 & 0.000 \\
Creatinine & 50912  & 0.253 & 0.000 \\
Glucose    & 50931  & 0.297 & 0.000 \\ \hline
\end{tabular}
\caption{\footnotesize (MIMIC-III)}
\label{tab:char-mimic}
\end{subtable}

\begin{subtable}{0.48\textwidth}
\begin{tabular}{l|ll|ll}
\hline
\multirow{2}{*}{Vital Signs} & \multicolumn{2}{l|}{CCHS} & \multicolumn{2}{l}{Mayo} \\ \cline{2-5} 
                            & OMR         & PMR         & OMR         & PMR        \\ \hline
Temperature                 & 0.739       & 0.633       & 0.910       & 0.706      \\
FiO2                        & 0.663       & 0.467       & 0.940       & 0.739      \\
MAP                         & 0.660       & 0.544       & 0.632       & 0.349      \\
DiastolicBP                 & 0.658       & 0.544       & 0.632       & 0.349      \\
SystolicBP                  & 0.658       & 0.543       & 0.632       & 0.348      \\
PulseOx                     & 0.536       & 0.283       & 0.339       & 0.143      \\
RespiratoryRate             & 0.519       & 0.272       & 0.489       & 0.288      \\
HeartRate                   & 0.484       & 0.237       & 0.235       & 0.038      \\
OxygenFlow                  & 0.777       & 0.112       & 0.974       & 0.083      \\ \hline
\end{tabular}
\caption{\footnotesize (CCHS\&Mayo)}
\label{tab:char-cchs&mayo}
\end{subtable}

\begin{tablenotes}
      \scriptsize
      \item Item ID: Identification code of measurements, which is specific to MIMIC-III.
      \item NMR: Native missing rate.
      \item PMR: Missing rate after applying exclusion and preprocessing criteria.
    \end{tablenotes}
\end{threeparttable}
\vspace{-0.2 in}
\end{table}

% \begin{table}[tbp]
% \caption{Extracted Measurements from MIMIC-III Dataset. The Item ID Represents The Identification Code of A Measurement in MIMIC-III.}
% \label{table:char}
% \begin{tabular}{lcc}
% \hline
% \multicolumn{1}{l}{Measurements}       & \multicolumn{1}{c}{Item IDs} & Missing Rates \\ \hline
% Chloride                                & 50902                        & 0.258        \\
% Potassium                               & 50971                        & 0.210        \\
% Bicarb                                  & 50882                        & 0.271        \\
% Sodium                                  & 50983                        & 0.244        \\
% Hematocrit                              & 51221                        & 0.181        \\
% Hemoglobin                              & 51222                        & 0.304        \\
% Mean corpuscular volume (MCV)           & 51250                        & 0.308        \\
% Platelet Count                          & 51240                        & 0.279        \\
% White blood cells (WBC)                 & 51301                        & 0.303        \\
% Red blood cell distribution width (RDW) & 51277                        & 0.309        \\
% Blood urea nitrogen (BUN)               & 51006                        & 0.259        \\
% Creatinine                              & 50912                        & 0.253        \\
% Glucose                                 & 50931                        & 0.297        \\ \hline
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \begin{table*}[tbp]
% \centering
% \begin{threeparttable}
% \caption{Extracted Categories and Measurements from MIMIC-III, CCHS, and Mayo Datasets. The Item ID Represents The Identification Code of A Measurement in MIMIC-III.}
% \label{table:char}
% \begin{tabular}{l|lc|ccc}
% \hline
% \multirow{2}{*}{Category}     & \multirow{2}{*}{Measurement}            & \multirow{2}{*}{Item ID} & \multicolumn{3}{c|}{Missing Rate}                                                   \\ \cline{4-6} 
%                               &                                         &                          & \multicolumn{1}{l}{MIMIC-III} & \multicolumn{1}{l}{CCHS} & \multicolumn{1}{l}{Mayo} \\ \hline
% \multirow{15}{*}{Lab results} & Chloride                                & 50902                    & 0.258                         & X                        & -                        \\
%                               & Potassium                               & 50971                    & 0.210                         & X                        & -                        \\
%                               & Bicarb                                  & 50882                    & 0.271                         & X                        & X                        \\
%                               & Sodium                                  & 50983                    & 0.244                         & X                        & -                        \\
%                               & Hematocrit                              & 51221                    & 0.181                         & X                        & X                        \\
%                               & Hemoglobin                              & 51222                    & 0.304                         & X                        & -                        \\
%                               & Mean corpuscular volume (MCV)           & 51250                    & 0.308                         & X                        & -                        \\
%                               & Platelet Count                          & 51240                    & 0.279                         & 0.934                    & -                        \\
%                               & White Blood Cells (WBC)                 & 51301                    & 0.303                         & 0.935                    & -                        \\
%                               & Red blood cell distribution width (RDW) & 51277                    & 0.309                         & X                        & X                        \\
%                               & Blood urea nitrogen (BUN)               & 51006                    & 0.259                         & 0.933                    & -                        \\
%                               & Creatinine                              & 50912                    & 0.253                         & 0.933                    & -                        \\
%                               & Glucose                                 & 50931                    & 0.297                         & X                        & -                        \\
%                               & Bilirubin                               & \multicolumn{1}{l|}{}    & -                             & 0.979                    & -                        \\
%                               & Lactate                                 & \multicolumn{1}{l|}{}    & -                             & 0.972                    & -                        \\ \hline
% \multirow{7}{*}{Vital signs}  & Temperature                             & \multicolumn{1}{l|}{}    & -                             & 0.813                    & 0.889                    \\
%                               & Mean arterial pressure (MAP)            & \multicolumn{1}{l|}{}    & -                             & 0.774                    & 0.674                    \\
%                               & Diastolic blood pressure (DBP)          & \multicolumn{1}{l|}{}    & -                             & 0.721                    & 0.674                    \\
%                               & Systolic blood pressure (SBP)           & \multicolumn{1}{l|}{}    & -                             & 0.720                    & 0.674                    \\
%                               & Pulse oximetry (PulseOx)                & \multicolumn{1}{l|}{}    & -                             & 0.637                    & 0.342                    \\
%                               & Respiratory rate                        & \multicolumn{1}{l|}{}    & -                             & 0.626                    & 0.535                    \\
%                               & Heart rate                              & \multicolumn{1}{l|}{}    & -                             & 0.606                    & 0.211                    \\ \hline
% \end{tabular}
% \begin{tablenotes}
%       \small
%       \item -: the dataset contained the measurement but we didn't use it in our study. \\
%       X: the dataset didn't contain the measurement.
%     \end{tablenotes}
% \end{threeparttable}
% \end{table*}

==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/table/nrmse.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tbp]
% \scriptsize
% \small
\centering
\caption{Imputation results (nRMSE) with masking rates 60\%-90\% on 13 features of MIMIC-III.}
\label{tab:nrmse}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{lcccccccccccccc}
\hline                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{l|}{Model} & \multicolumn{1}{c}{CI} & \multicolumn{1}{c}{K} & \multicolumn{1}{c}{HCO3} & \multicolumn{1}{c}{Na} & \multicolumn{1}{c}{Hct} & \multicolumn{1}{c}{Hb} & \multicolumn{1}{c}{MCV} & \multicolumn{1}{c}{PLT} & \multicolumn{1}{c}{WBC} & \multicolumn{1}{c}{RDW} & \multicolumn{1}{c}{BUN} & \multicolumn{1}{c}{Cr} & \multicolumn{1}{c}{GLC} & \multicolumn{1}{c}{Average} \\ \hline

\multicolumn{14}{l}{Mask rate: 90\%}                                                                                                                                                               \\ \hline
\multicolumn{1}{l|}{MeanFill} & 1.296 & 1.208 & 1.143 & 1.120 & 4.227 & 2.729 & 2.337 & 8.754 & 5.065 & 4.721 & 3.368 & 3.398 & 4.488 & 3.373\\
\multicolumn{1}{l|}{ECF}                          & \textbf{0.270}                        & \textbf{0.256}                         & \textbf{0.272}                      & \textbf{0.267}                      & \textbf{0.275}                          & \textbf{0.278}                          & \textbf{0.295}                   & \textbf{0.294}                              & \textbf{0.279}                   & \textbf{0.304}                   & \textbf{0.283}                   & \textbf{0.280}                          & \textbf{0.260}                   & \textbf{0.278}    \\ \cline{2-15}
\multicolumn{1}{l|}{MICE}       & 0.283                        & 0.269                         & 0.287                      & 0.280                      & 0.282                          & 0.284                         & 0.310                   & 0.310                              & 0.295                   & 0.321                   & 0.304                   & 0.318                         & 0.271           & 0.293            \\ 
\multicolumn{1}{l|}{3D-MICE}    & \textbf{0.259}                        & \textbf{0.253}                         & \textbf{0.262}                      & \textbf{0.259}                      & \textbf{0.262}                 & \textbf{0.263}                 & \textbf{0.270}                  & \textbf{0.274}                              & \textbf{0.270}                   & \textbf{0.265}                   & \textbf{0.267}                   & \textbf{0.261}                          & \textbf{0.256}                  & \textbf{0.263}     \\  \cline{2-15}
\multicolumn{1}{l|}{DETROIT} & 4.457 & \textbf{0.289} & \textbf{0.311} & 2.855 & 0.421 & \textbf{0.371} & 0.981 & 0.578 & 2.121 & \textbf{0.303} & 1.720 & 2.014 & 1.585 & 1.385\\
\multicolumn{1}{l|}{TAME} & \textbf{0.381} & 0.388 & 0.318 & \textbf{0.323} & \textbf{0.387} & 0.380 & \textbf{0.734} & \textbf{0.436} & \textbf{0.465} & 0.441 & \textbf{0.482} & \textbf{1.290} & \textbf{0.365} & \textbf{0.491} \\ \hline
\multicolumn{1}{l|}{TA-DualCV$^{-C}$}                              & 0.284                        & 0.276                         & 0.285                      & 0.284                      & 0.288                          & 0.290                          & 0.296                   & 0.300                              & 0.296                   & 0.289                   & 0.292                   & 0.284                          & 0.279         & 0.288              \\
\multicolumn{1}{l|}{TA-DualCV$^{-I}$} & 0.254 & 0.264 & 0.255 & 0.257 & 0.258 & 0.261 & 0.266 & 0.267 & 0.277 & 0.257 & 0.257 & 0.260 & 0.267 & 0.261 \\
\multicolumn{1}{l|}{TA-DualCV}    & \textbf{0.221}**               & \textbf{0.225}**                & \textbf{0.224}**             & \textbf{0.222}**             & \textbf{0.229}**                          & \textbf{0.233}**                          & \textbf{0.232}**          & \textbf{0.236}**                     & \textbf{0.232}**          & \textbf{0.237}**          & \textbf{0.229}**          & \textbf{0.223}**                 & \textbf{0.218}**        & \textbf{0.228}**       \\ \hline




\multicolumn{14}{l}{Mask rate: 80\%}                                                                                                            \\ \hline
\multicolumn{1}{l|}{MeanFill} & 1.201 & 1.105 & 1.065 & 1.072 & 4.325 & 2.486 & 2.174 & 7.354 & 4.189 & 4.394 & 3.032 & 3.211 & 3.878 & 3.037\\
\multicolumn{1}{l|}{ECF}     & \textbf{0.267}                        & \textbf{0.254}                        & \textbf{0.268}                      & \textbf{0.265}                      & \textbf{0.273}                          & \textbf{0.276}                          & \textbf{0.292}                   & \textbf{0.289}                              & \textbf{0.276}                   & \textbf{0.299}                   & \textbf{0.279}                   & \textbf{0.276}                          & \textbf{0.258}        & \textbf{0.275}               \\ \cline{2-15} 
\multicolumn{1}{l|}{MICE}                            & 0.287                        & 0.270                         & 0.290                      & 0.283                      & 0.286                          & 0.289                          & 0.312                   & 0.313                              & 0.297                   & 0.322                   & 0.307                   & 0.324                          & 0.273             & 0.296          \\ 
\multicolumn{1}{l|}{3D-MICE}                         & \textbf{0.257}                        & \textbf{0.250}                         & \textbf{0.259}                      & \textbf{0.256}                      & \textbf{0.259}                          & \textbf{0.261}                          & \textbf{0.267}                   & \textbf{0.273}                              & \textbf{0.267}                   & \textbf{0.264}                   & \textbf{0.264}                   & \textbf{0.258}                          & \textbf{0.253}       & \textbf{0.260}                \\ \cline{2-15}
\multicolumn{1}{l|}{DETROIT} & \textbf{0.272} & \textbf{0.257} & \textbf{0.256} & \textbf{0.257} & \textbf{0.256} & \textbf{0.251} & \textbf{0.407} & \textbf{0.287} & \textbf{0.321} & \textbf{0.270} & \textbf{0.314} & 1.544 & \textbf{0.243} & \textbf{0.380}\\
\multicolumn{1}{l|}{TAME} & 0.317 & 0.294 & 0.314 & 0.317 & 0.389 & 0.402 & 0.513 & 0.527 & 0.602 & 0.624 & 0.343 & \textbf{0.484} & 0.389 & 0.424\\ \hline
\multicolumn{1}{l|}{TA-DualCV$^{-C}$}         & 0.277                        & 0.272                         & 0.280                     & 0.279                     & 0.283                          & 0.284                         & 0.290                   & 0.292                              & 0.290                   & 0.280                   & 0.286                  & 0.279                          & 0.274             & 0.282          \\
\multicolumn{1}{l|}{TA-DualCV$^{-I}$} & 0.246 & 0.251 & 0.250 & 0.247 & 0.242 & 0.242 & 0.268 & 0.262 & 0.262 & 0.271 & 0.256 & 0.259 & 0.257 & 0.255 \\
\multicolumn{1}{l|}{TA-DualCV}                         &\textbf{0.222}**               & \textbf{0.219}**                & \textbf{0.224}**             & \textbf{0.222}**             & \textbf{0.228}**                 & \textbf{0.231}**                 & \textbf{0.235}**          & \textbf{0.236}**                     & \textbf{0.233}**          & \textbf{0.234}**          & \textbf{0.225}**          & \textbf{0.226}**                 & \textbf{0.221}**    &  \textbf{0.227}**         \\ \hline












\multicolumn{14}{l}{Mask rate: 70\%}                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{l|}{MeanFill} & 0.847 & 0.787 & 0.789 & 0.764 & 2.611 & 1.752 & 1.726 & 4.394 & 3.225 & 3.247 & 2.170 & 2.674 & 2.159 & 2.088\\
\multicolumn{1}{l|}{ECF}     & \textbf{0.255}                        & \textbf{0.249}                         & \textbf{0.258}                      & \textbf{0.255}                      & \textbf{0.264}                          & \textbf{0.266}                          & \textbf{0.279}                   & \textbf{0.277}                              & \textbf{0.264}                   & \textbf{0.285}                   & \textbf{0.265}                   & \textbf{0.264}                          & \textbf{0.254}           & \textbf{0.264}            \\ \cline{2-15} 
\multicolumn{1}{l|}{MICE}       & 0.271                        & 0.264                         & 0.279                      & 0.269                      & 0.264                          & 0.265                          & 0.304                   & 0.302                              & 0.287                   & 0.314                   & 0.293                   & 0.310                          & 0.268            & 0.284           \\ 

\multicolumn{1}{l|}{3D-MICE}    & \textbf{0.243}                        & \textbf{0.242}                         & \textbf{0.248}                      & \textbf{0.245}                      & \textbf{0.244}                 & \textbf{0.243}                 & \textbf{0.251}                  & \textbf{0.256}                              & \textbf{0.254}                   & \textbf{0.246}                   & \textbf{0.250}                   & \textbf{0.245}                          & \textbf{0.246}   & \textbf{0.247}                    \\ \cline{2-15}
\multicolumn{1}{l|}{DETROIT} & \textbf{0.239} & \textbf{0.244} & 0.301 & 0.266 & \textbf{0.227} & \textbf{0.220}** & \textbf{0.258} & 0.361 & 0.449 & \textbf{0.238}** & 0.790 & 0.849 & \textbf{0.263} & 0.362 \\
\multicolumn{1}{l|}{TAME} & 0.274 & 0.320 & \textbf{0.281} & \textbf{0.265} & 0.237 & 0.235 & 0.497 & \textbf{0.326} & \textbf{0.370} & 0.410 & \textbf{0.330} & \textbf{0.509} & 0.444 & \textbf{0.346}\\ \hline
\multicolumn{1}{l|}{TA-DualCV$^{-C}$}         & 0.255                        & 0.249                         & 0.258                      & 0.255                      & 0.264                          & 0.266                         & 0.279                   & 0.277                              & 0.264                   & 0.285                   & 0.265                  & 0.264                          & 0.254       & 0.264                \\
\multicolumn{1}{l|}{TA-DualCV$^{-I}$} & 0.231 & 0.235 & 0.240 & 0.234 & 0.223 & 0.225 & 0.247 & 0.248 & 0.256 & 0.246 & 0.238 & 0.242 & 0.247 & 0.239  \\
 \multicolumn{1}{l|}{TA-DualCV}    &   \textbf{0.220}** & \textbf{0.221}** & \textbf{0.221}** & \textbf{0.229}** & \textbf{0.221}** & \textbf{0.222} & \textbf{0.235}** & \textbf{0.231}** & \textbf{0.229}** & \textbf{0.239} & \textbf{0.225}** & \textbf{0.224}** & \textbf{0.214}** & \textbf{0.225}**        \\ \hline
 
 
 
 




\multicolumn{14}{l}{Mask rate: 60\%}                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{l|}{MeanFill}  & 0.657 & 0.589 & 0.624 & 0.591 & 1.801 & 1.279 & 1.544 & 2.958 & 1.782 & 2.538 & 1.685 & 2.370 & 1.601 & 1.540 \\
\multicolumn{1}{l|}{ECF}     & \textbf{0.247}                        & \textbf{0.246}                         & \textbf{0.250}                      & \textbf{0.248}                      & \textbf{0.258}                          & \textbf{0.260}                          & \textbf{0.272}                   & \textbf{0.266}                              & \textbf{0.257}                   & \textbf{0.275}                   & \textbf{0.253}                   & \textbf{0.255}                          & \textbf{0.252}  & \textbf{0.257}                      \\ \cline{2-15}
\multicolumn{1}{l|}{MICE}       & 0.260                        & 0.261                         & 0.271                      & 0.259                      & 0.247                          & 0.247                          & 0.301                   & 0.298                              & 0.283                   & 0.310                   & 0.285                   & 0.296                          & 0.266  & 0.276                     \\ 

\multicolumn{1}{l|}{3D-MICE}    & \textbf{0.233}                        & \textbf{0.234}                         & \textbf{0.239}                      & \textbf{0.235}                      & \textbf{0.229}                 & \textbf{0.228}                 & \textbf{0.240}                  & \textbf{0.244}                              & \textbf{0.245}                   & \textbf{0.232}                   & \textbf{0.238}                   & \textbf{0.236}                          & \textbf{0.238}   & \textbf{0.236}                    \\ \hline
\multicolumn{1}{l|}{DETROIT} & \textbf{0.154}** & \textbf{0.241} & \textbf{0.168}** & \textbf{0.154}** & \textbf{0.149}** & \textbf{0.196}** & \textbf{0.164}** & 0.481 & 0.458 & \textbf{0.154}** & \textbf{0.216}** & \textbf{0.411} & \textbf{0.170}** & \textbf{0.240} \\
\multicolumn{1}{l|}{TAME} & 0.227 & 0.271 & 0.257 & 0.245 & 0.211 & 0.212 & 0.355 & \textbf{0.321} & \textbf{0.320} & 0.352 & 0.270 & 0.423 & 0.321 & 0.291 \\ \cline{2-15}
\multicolumn{1}{l|}{TA-DualCV$^{-C}$} & 0.271 & 0.275 & 0.271 & 0.274 & 0.281 & 0.283 & 0.284 & 0.281 & 0.285 & 0.269 & 0.271 & 0.275 & 0.282 & 0.277 \\  
\multicolumn{1}{l|}{TA-DualCV$^{-I}$} & \textbf{0.218} & 0.237 & 0.230 & \textbf{0.223} & \textbf{0.205} & \textbf{0.207} & 0.260 & 0.245 & 0.247 & 0.256 & 0.234 & 0.240 & 0.249 & 0.235 \\ 
\multicolumn{1}{l|}{TA-DualCV} &  0.219 & \textbf{0.223}** & \textbf{0.220} & 0.224 & 0.218 & 0.218 & \textbf{0.229} & \textbf{0.230}** & \textbf{0.223} & \textbf{0.222} & \textbf{0.225} & \textbf{0.223}** & \textbf{0.209} & \textbf{0.222}** \\ \hline
\end{tabular}
\begin{tablenotes}
      \small
      \item - For each block, the best approach is in \textbf{bold}; The best approach across ALL is labeled with **.
    \end{tablenotes}
\end{threeparttable}
}
\end{table*}

==> ICHI'22 Ge - EHRs Imputation_arxiv/sections/table/pred.tex <==
\begin{table*}[tbp]
\label{tab:pred}
\centering
\caption{Septic Shock 24-Hour Early Prediction Performance (mean$\pm$std) on CCHS Data.}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{l|lllll|lllll}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{Original}                                                                                                                                       & \multicolumn{5}{c}{+MI}                                                                                                \\ \cline{2-11} 
                        & \multicolumn{1}{c}{Accuracy}        & \multicolumn{1}{c}{Precision}          & \multicolumn{1}{c}{Recall}       & \multicolumn{1}{c}{F1}              & \multicolumn{1}{c|}{AUC}            & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC}    \\ \hline
Expert                  &         .691$\pm$.027                            &     .685$\pm$.039                                &       .716$\pm$.044                              &        .698$\pm$.044                             &     .744$\pm$.023                                &        .808$\pm$.009                      &         .815$\pm$.019                   &     \textbf{.797$\pm$.018}                          &         .806$\pm$.018                   &   .879$\pm$.009                         \\
GP                      & .700$\pm$.017           & .703$\pm$.042          & .703$\pm$.027          & .702$\pm$.027          & .757$\pm$.011          &           .803$\pm$.009                   &    .819$\pm$.021                        &       .779$\pm$.020                        &    .798$\pm$.020                        &          .877$\pm$.007                  \\
MICE                    & .689$\pm$.020          & .686$\pm$.026          & .701$\pm$.032          & .693$\pm$.032          & .743$\pm$.015          & .788$\pm$.013   & .804$\pm$.014 & .760$\pm$.023    & .781$\pm$.023 & .865$\pm$.018 \\
3D-MICE                 & .697$\pm$.012          & .706$\pm$.042          & .684$\pm$.037          & .693$\pm$.037          & .768$\pm$.016          & .794$\pm$.011   & .806$\pm$.037 & .776$\pm$.024    & .790$\pm$.024 & .876$\pm$.010 \\
3M-MICE                 & \textbf{.717$\pm$.019}          & \textbf{.711$\pm$.034}          & \textbf{.729$\pm$.022}          & \textbf{.720$\pm$.022}          & \textbf{.777$\pm$.016}          & \textbf{.812$\pm$.006}   & \textbf{824$\pm$.009} & \.795$\pm$.006   & \textbf{.809$\pm$.006} & \textbf{.889$\pm$.007} \\ \hline
Expert+MI               &       .736$\pm$.019                              &    .742$\pm$.047                                 &      .730$\pm$.036                               &        .734$\pm$.036                             &      .790$\pm$.008                               &                 \textbf{.842$\pm$.024}             &          .838$\pm$.026                  &      \textbf{.846$\pm$.042}                         &    \textbf{.842$\pm$.042}                        &    \textbf{.915$\pm$.014}                        \\
GP+MI                   & .730$\pm$.012          & .731$\pm$.021          & .727$\pm$.026          & .729$\pm$.026          & .788$\pm$.016          &          .826$\pm$.016                    &    .823$\pm$.030                        &        .831$\pm$.015                       &   .827$\pm$.015                         &        .906$\pm$.012                   \\
MICE+MI                 & .739$\pm$.011          & .739$\pm$.026          & .739$\pm$.015          & .739$\pm$.015          & .792$\pm$.003          & .809$\pm$.018   & .816$\pm$.025 & .795$\pm$.023    & .806$\pm$.023 & .890$\pm$.012 \\
3D-MICE+MI              & .746$\pm$.028          & .748$\pm$.045          & .742$\pm$.028          & .745$\pm$.028          & .809$\pm$.022          & .830$\pm$.011   & .828$\pm$.015 & .834$\pm$.017    & .831$\pm$.017 & .899$\pm$.008 \\
3M-MICE+MI              & \textbf{.754$\pm$.012} & \textbf{.758$\pm$.031} & \textbf{.748$\pm$.021} & \textbf{.752$\pm$.021} & \textbf{.814$\pm$.012} & .834$\pm$.007   & \textbf{.841$\pm$.011} & .824$\pm$.018    & .832$\pm$.018 & .905$\pm$.006 \\ \hline
\end{tabular}
\begin{tablenotes}
      \small
      \item - The bold number represents the best performance.
      \item +MI: The method is combined with missing indicators.
      \item - DETROIT and CATSI cannot be implemented properly due to its intrinsic limitation taking fixed-size non-missing inputs.
    \end{tablenotes}
\end{threeparttable}
}
\vspace{-0.1 in}
\end{table*}

==> sections/exp-old.tex <==


In this work, we mainly validate our imputation model from two aspects: 1) capability, which represents what types of measurements can be imputed by our model; 2) accuracy, which represents how accurate our model can impute the data with varied missing rates. We compare our model with 3 state-of-the-art approaches (3D-MICE \cite{luo20183d}, MICE \cite{buuren2010mice}, GP \cite{rasmussen2003gaussian}) and 1 expert baseline \cite{kim2018temporal}.

%%%% dataset
\subsection{Three Datasets: MIMIC-III, CCHS, and Mayo} collected from different hospitals were involved.  with different characteristics shown in Table \ref{tab:char}. To validate the capacity of our model with two main categories (lab analytes and vital signs) of measurements, we selected 13 lab analytes from MIMIC-III, 9 vital signs from CCHS, and 9 vital signs from Mayo according the specific characteristic of each dataset. We describe the details of selection in the followings.

\subsubsection{MIMIC-III} The MIMIC-III database contains 53,423 admissions of adult patients (i.e., age $>$ 16) who are admitted to intensive care units (ICU) at a tertiary referral hospital between 2001 and 2012 \cite{johnson2016mimic}. Specifically, it contains $\sim$331 million charted observations for patients and 753 laboratory items. Within the MIMIC-III database, we selected 13 laboratory analyte items (shown in Table~\ref{table:char-mimic}) that contain low original missing rates and are measured quantitatively. We also listed the identification codes we use for measurements of interests in MIMIC-III database (see Table \ref{tab:char-mimic}), as the same name of a measurement can have different Item IDs.

In this work, one objective is to validate our imputation method in the context where a large range of masking rates occurs, i.e. $20\% \sim 90\%$. The native missing rates of MIMIC-III is relatively high (i.e. $26.7\%$ on average), thus we applied exclusion criteria for data sampling: i) Exclude records that had less than 11 events; ii) Exclude data from events that contained more than $50\%$ missing rate; iii) Exclude data from laboratory items that contained more than $50\%$ missing rate. Our final data consists of $\sim$17 million record of 19,693 patients. The average missing rate after applying the above criteria is $5.78\%$. The minimum and maximum number of events across records are 11 and 1191, respectively. The mean and median number of events across records are 33.4 and 22, respectively. Aside from the native missing values, we masked values with rates $20\% - 90\%$. Both native and masked values will be imputed to form final complete data. %Therefore, the final imputed data is complete without any missing values so that machine learning techniques that rely on complete data can be applied to the data. The distribution of time points is shown in Fig.~\ref{fig:time-dist-mimic}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.12]{sections/figure/timedist-mimic.jpg}
%     \caption{Distribution of Number of Events in Final Data of MIMIC-III}
%     \label{fig:time-dist-mimic}
% \end{figure}

%% moved to supplementary
% \begin{figure}[t]
%     \centering
%     \includegraphics%[scale=0.4]
%     [width=8.5cm,height=3.4cm]{sections/figure/heatmap.png}
%     \caption{Heatmap of 3 Datasets. (A: MIMIC-III. B: Mayo. C: CCHS.)}
%     \label{fig:heatmap}
% \vspace{-0.2 in}
% \end{figure}



%%% Need more information regarding the 2 datasets 
\subsubsection{Christiana Care Health System (CCHS)} This dataset contains 210,289 visit records of adult patients (i.e. age $>$ 18) admitted to Christiana Care hospital from July, 2013 to December, 2015. The CCHS dataset contains partial types of lab results as compared to MIMIC-III, but greater native missing rates (i.e. $\sim$ 85.7\% on average). This is caused by the nature of this data, as it includes the records of patients at different locations from emergency department to ICU, which is different from MIMIC-III that only includes ICU visits. We selected 9 measurements with the least native missing rates, which belong to vital signs. Due to the large sparsity of the CCHS data, we only impute the native missing values without masking. As the main goal of imputation is to generate complete data to be used by machine learning techniques, we propose to validate our imputation approach by applying a septic shock prediction model on the imputed data. 

We firstly apply one exclusion criteria by excluding events with all missing values. Then we preprocess the data in three steps: 1) aggregate data into 30 minutes window by taking median values on both measurement and recorded time; 2) If a visit contains less than 5 events, carry forward the last value within a fixed length time window (i.e., 8 hours) to fill missing values, and use mean value of corresponding measurement to fill the remaining missing values; 3) OxygenFlow, which is measured every $\sim$45-minute, contains the highest missing rate (i.e. 97.4\%) but stable range of values within records. We carry forward the last value within 8 hours to fill missing values of OxygenFlow and mean values to fill the remaining. After that, we apply the other exclusion criteria by excluding the records that contain less than 2 records of each measurement. Finally, we get $\sim$400 thousands events for 3,240 visits (1,349 shock positive and 1,891 shock negative). The average missing rate is 40.4\%. The minimum and maximum number of evens across records are 1 and 2,277, respectively. The mean and median value of events are 131 and 83, respectively.


\subsubsection{Mayo} This dataset contains 106,844 visit records of adult patients (i.e. age $>$ 18) admitted to Mayo Clinic hospital from July, 2013 to December, 2015. It contains most types of lab results and vital signs compared to MIMIC-III, but similar to CCHS, it has large native missing rates (i.e. $\sim$ 85.6\% on average). We select the same 9 measurements as CCHS with the least original missing rates, which belong to the category of vital signs. Following the aforementioned exclusion and preprocessing criteria with CCHS data, we include $\sim$1.55 million records of 6,850 visits (3,457 shock positive and 3,393 shock negative). The average missing rate is 33.8\%. The minimum and maximum number of evens across records are 3 and 10,663, respectively. The mean and median value of events are 226 and 212, respectively.

%% baseline
%\subsection{Baselines}

%% normalization
\subsection{Normalization}
The proper operation of GP imputation requires normalization while it has little effect on MICE imputation \cite{luo20183d}. Therefore, we normalize our data such that all measurements are scaled to be within [0, 1] interval throughout time points before imputation and de-normalize it to obtain the final complete data after imputation. 
% Specifically, on a time point $t_i$, the normalize value $nv_{ij}$ of a measurement $m_j$ is calculated by the following equation:

% \begin{equation}
%     nv_{ij} = \frac{ov_{ij} - min(ov_{:j})}{max(ov_{:j}) - min(ov_{:j})}
% \end{equation}

% where $ov_{ij}$ represents original value of a measurement $m_j$ at time point $t_i$, and $ov_{:j} = \{ov_{1j},ov_{2j},...,ov_{nj}\}$, $n \in 	\mathbb{R}$.

%%%% Setups: 1) Baselines, 2) Various missing rates
\subsection{Validation}
To assess the performance of 3M-MICE in comparison with the benchmarks and in various circumstances, we validated our model in two experimental settings:

    % \item \textbf{Cross models validation:} We compared our model with 3 baselines, MICE, GP, and Mean imputation. Specifically, we employed MICE package in R \cite{buuren2010mice}. In calling the MICE package, the default number of multiple imputations was 5. To show the lowest possible bound of our model imputation efforts, we used only 1 iteration for multiple imputation in MICE package for both our approach and MICE baseline. We also employed GPfit package in R \cite{macdonald2015gpfit} as another baseline. The parameters used in GP of both our approach and baseline were all default ones except the parameter used in computing the nugget. The details regarding the nugget will be discussed in the following paragraph. Moreover, we employed the balanced parameter 0.5 for both $w_{11}$ and $w_{12}$. In future approaches, the values of $w_{11}$ and $w_{12}$ can be adjusted according to the training performance on target data. 
\textbf{Various Masking Rates on Obervations:} To explore the performance with various missing rates, we conducted 6 sub-samples of MIMIC-III by randomly masking 20\%, 50\%, 60\%, 70\%, 80\%, and 90\% of the observed values. We compare our model with 4 baselines for each measurement and overall data.

\textbf{Septic Shock Early Prediction:} To measure the capabilities of our approach, we utilize the imputed data by different imputation approaches to build an LSTM network to predict a challenging condition in practice, septic shock, 8 hours before its onset, which has been adopted in previous approaches \cite{yang2018time}. Considering the imbalanced ratio between shock positive and negative visits, we employ stratified random sampling on both positive and negative visits. Finally, the CCHS data contains 1300 visits for each group with $\sim$340 thousands events in total, and Mayo data contains 3200 visits for each group with $\sim$1.5 million events in total. Also, we compare our model with baselines by adding missing indicators on measurements to explore whether and what extent missing indicator can affect prediction results.
    
    % Specifically, in GP, the ill-conditioning $R$ (introduced in Eq.~\ref{eq:R-matrix}, Section III.B) might occur if any pair of points ($t_{ik}$ and $t_{jk}$) were too close or $\theta_k$'s were close to 0. To fix such issue, Ranjan et al. introduced a nugget computing a well-behaved $R$ to substitute the ill-conditioning one, and they set a parameter to be the boundary for nugget \cite{ranjan2011computationally}. In this approach, various missing rate of the data could require various values of the nugget-related parameter in single-task GP as higher sparsity of data may introduce ill-conditioning correlation matrix. 


\subsection{Baselines}
We employ 3 state-of-the-art baselines and 1 expert baseline. The state-of-the-art baselines are 3D-MICE \cite{luo20183d}, sampling-based MICE \cite{buuren2010mice}, and GP with RBF kernel. We also employ an expert baseline which is defined by the domain experts and has been adopted in previous research \cite{kim2018temporal}. The expert baseline fills the missing values with the last value within a fixed length window (i.e. 24 hours for lab analytes and 8 hours for vital signs), and fills the remains with the mean value of the corresponding measurements. The expert baseline performs better in clinical data imputation and prediction compared to traditional baselines (e.g. mean/median, carry forward, etc.) in both previous \cite{kim2018temporal} and our work, thus we don't present the results of traditional baselines here. For fair comparison, we adopt the same experimental settings for baselines as our model. 


%%%% Performance evaluation: nRMSE
\subsection{Performance Evaluation}
We evaluated the performance of our model and baselines on imputing masked values by calculating the normalized root-mean-square error (nRMSE). RMSE is frequently employed to measure the differences between estimated values and observed values. It assigns large residuals with a disproportionately large effect, thus more sensitive to outliers \cite{pontius2008components}. Normalizing the RMSE can help in comparing among datasets or models that contain different scales of values. The normalization has different calculation in different approaches. In this study, we used the common choice regarding normalization that was the range of the measured data. Therefore, the nRMSE of a variable $v$ was calculated by the following equation:

\begin{equation}
    nRMSE_v = \sqrt{\frac{\sum_{p,t}(\frac{(\hat{Y}_{v,p,t} - Y_{v,p,t})}{max(Y_{v,p}) - min(Y_{v,p})})^2}{\mid T \mid}}
\end{equation}

where $p \in [1, P]$, $t \in T$. $P$ is the total number of patient in the data, $T$ is a list of time points with missing values of variable $v$ for patient $p$. $\hat{Y}$ represents the estimated value while $Y$ represents the actual value. 

We evaluate the performance of our model and baselines on predicting septic shock by calculating evaluation metrics of accuracy (Acc), recall, precision, $F_1$ score (F1), and area under ROC curve (AUC) obtained from 5 cross-validation. Accuracy is the proportion of correctly classified visits over all visits. Recall is the proportion of correctly identified positive visits over all visits that actually have septic shock. Precision is the proportion of correctly identified positive visits over all visits that are identified as positive. F1 is the harmonic mean of the precision and recall. AUC calculates the trade-off between recall and specificity, where specificity is the proportion of correctly identified negative visits over all visits that are identified as negative.

%%%% settings
In this work, we impute the data with all methods on a 12-core machine. We use 1 iteration on multiple imputation with MICE R package \cite{buuren2010mice} for 3M-MICE, 3D-MICE, and MICE methods, and 0.02 $\alpha$ on RBF kernel with GP \cite{rasmussen2003gaussian}. In 2-step MICE, we assign $0.5$ to both $w_{11}$ and $w_{12}$ to ensure the fairness and balance the effect of MICE through cross-sectional and longitudinal view. In LSTM, we use 1 hidden layer with 128 hidden neurons, 0.005 initial learning rate, and 200 maximum sequence-length. We adopt Adam optimizer \cite{kingma2014adam} with 64 batches and 25 epochs.

==> sections/exp.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[scale=0.4]{sections/figure/nrmse.png}
    \caption{nRMSE by Measurement and Imputation Method. X-Axis: Masking Rates; Y-Axis: nRMSE.}
    \label{fig:nrmse}
    \vspace{-0.2 in}
\end{figure*}

In this work, we mainly validate our proposed imputation model from two aspects: 1) capability, which represents what types of measurements can be imputed by our model; 2) accuracy, which represents how accurate our model can impute the data with varied missing rates. We compare our model with four baselines (i.e., \cite{luo20183d ,buuren2010mice, rasmussen2003gaussian, kim2018temporal}).

\vspace{-0.1 in}



\vspace{-0.1 in}

\subsection{Various Masking Rates on Observations}
To explore the performance with various missing rates, we conducted 6 sub-samples of MIMIC-III by randomly masking 20\%, 50\%, 60\%, 70\%, 80\%, and 90\% of the observed values. We compare our model with four baselines for each measurement and overall data.

\vspace{-0.1 in}

\subsubsection{Dataset:} \textbf{MIMIC-III} contains 53,423 admissions of adult patients (i.e., age $>$ 16) who are admitted to intensive care units (ICU) at a tertiary referral hospital between 2001 and 2012 \cite{johnson2016mimic}. Specifically, it contains $\sim$331 million charted observations for patients and 753 laboratory items. Within the MIMIC-III database, we selected 13 laboratory analyte items that contain low native missing rates (ranging from $18.1\%$ to $30.9\%$) and are measured quantitatively. The selected items are Chloride, Potassium, Bicarb, Sodium, Hematocrit, Hemoglobin, MCV, Platelet, WBC, RDW, BUN, Creatinine, and Glucose.
We validate our imputation method in the context where a large range of masking rates occurs, i.e. $20\% \sim 90\%$. The native missing rates of MIMIC-III is relatively high ($26.7\%$ on average), thus we applied exclusion criteria for data sampling: i) Exclude records that had less than 11 events; ii) Exclude data from events that contained more than $50\%$ missing rate; iii) Exclude data from laboratory items that contained more than $50\%$ missing rate. Our final data consists of $\sim$17 million record of 19,693 patients. The average missing rate after applying the above criteria is $5.78\%$. The number of events across visits vary from 11 to 1191 with the mean and median of 33.4 and 22, respectively. Aside from the native missing values, we masked values with rates $20\% - 90\%$. Both native and masked values will be imputed to form the final complete data \footnote{Numeric missing rates are attached in supplementary materials in detail}.

\noindent\textbf{Normalization:}
The proper operation of GP imputation requires normalization while it has little effect on MICE imputation \cite{luo20183d}. Therefore, we normalize our data such that all measurements are scaled to be within [0, 1] interval throughout time points before imputation and de-normalize it to obtain the final complete data after imputation. 

\vspace{-0.1 in}

\subsubsection{Performance Evaluation}
We evaluate the performance of methods on imputing masked values by calculating the normalized root-mean-square error (nRMSE). RMSE is frequently employed to measure the differences between estimated values and observed values. It assigns large residuals with a disproportionately large effect, thus more sensitive to outliers \cite{pontius2008components}. Normalizing the RMSE can help in comparing among datasets or models that contain different scales of values. The normalization has different calculation in different approaches. In this study, we used the common choice regarding normalization that was the range of the measured data. Therefore, the nRMSE of a variable $v$ was calculated by the following equation:

\begin{equation}
    nRMSE_v = \sqrt{\frac{\sum_{p,t}(\frac{(\hat{Y}_{v,p,t} - Y_{v,p,t})}{max(Y_{v,p}) - min(Y_{v,p})})^2}{\mid T \mid}}
\end{equation}

\noindent where $p \in [1, P]$, $t \in T$. $P$ is the total number of patient in the data, $T$ is a list of time points with missing values of variable $v$ for patient $p$. $\hat{Y}$ represents the estimated value while $Y$ represents the actual value. 

\vspace{-0.1 in}

\subsection{Septic Shock Early Prediction}
To measure the robustness of our approach, we utilize the imputed data by different imputation methods to build an LSTM network to predict a challenging condition in practice, septic shock, 8 hours before its onset, which has been adopted in previous approaches \cite{yang2018time}. We select 9 measurements with the least native missing rates (ranging from $51.9\%$ to $77.7\%$ for CCHS and $23.5\%$ to $97.4\%$ for Mayo) on both datasets. The 9 measurements include Temperature, FiO2, MAP, DiastolicBP, SystolicBP, PulseOx, RespiratoryRate, HeartRate, and OxygenFlow, which all belong to vital signs. Due to the large sparsity of both datasets, we only impute the native missing values without masking.

\vspace{-0.1 in}

\subsubsection{Datasets:}

\textbf{1) Christiana Care Health System (CCHS)} contains 210,289 visit records of adult patients (i.e. age $>$ 18) admitted to Christiana Care hospital from July, 2013 to December, 2015. The CCHS dataset contains partial types of lab results as compared to MIMIC-III, but greater native missing rates (i.e., $\sim$ 85.7\% on average). This is caused by the nature of this data, as it includes the records of patients at different locations from emergency department to ICU, which is different from MIMIC-III that only includes ICU visits. 

\noindent\textbf{2) Mayo} contains 106,844 visit records of adult patients (i.e. age $>$ 18) admitted to Mayo Clinic hospital from July, 2013 to December, 2015. It contains most types of lab results and vital signs compared to MIMIC-III, but similar to CCHS, it has large native missing rates (i.e. $\sim$ 85.6\% on average).

\subsubsection{Labeling}
The targeted population of CCHS and Mayo datasets are patients with suspected infection, which can be identified by presence of antiviral, antibiotic, etc. To label our records, we adopt our domain experts identification rule \cite{yang2018time}, which is a combination of International Classification of Diseases, Ninth Revision (ICD-9) and the Third International Consensus Definitions for Sepsis and Septic Shock \cite{singer2016third}.

\vspace{-0.1 in}

\subsubsection{Exclusion Criteria and Preprocessing}
For both datasets, we firstly apply one exclusion criteria by excluding events with all missing values. Then we preprocess the data in three steps: 1) aggregate data into 30 minutes window by taking median values on both measurement and recorded time; 2) If a visit contains less than 5 events, we carry forward the last value within a fixed length time window (i.e., 8 hours) to fill missing values, and use mean value of corresponding measurement to fill the remaining missing values; 3) OxygenFlow, which is measured every $\sim$45-minute, contains the highest missing rate (i.e., $97.4\%$) but stable range of values within records. We carry forward the last value within 8 hours to fill missing values of OxygenFlow and mean values to fill the remaining. After that, we apply the other exclusion criteria by excluding the records that contain less than 2 records of each measurement. For CCHS, we get $\sim$400 thousands events for 3,240 visits (1,349 shock positive and 1,891 shock negative). The average missing rate is 40.4\%. The number of events per visit ranges from 1 to 2,277, with the mean and median value of 131 and 83, respectively. For Mayo, we include $\sim$1.55 million records of 6,850 visits (3,457 shock positive and 3,393 shock negative). The average missing rate is 33.8\%. The minimum and maximum number of evens across records are 3 and 10,663, respectively. The mean and median value of events are 226 and 212, respectively.

Considering the imbalanced ratio between shock positive and negative visits, we employ stratified random sampling on both positive and negative visits. Finally, the CCHS data contains 1,300 visits for each group with $\sim$340 thousands events in total, and Mayo data contains 3,200 visits for each group with $\sim$1.5 million events in total. Also, we compare our model with baselines by adding missing indicators on measurements to explore whether and to what extent the missing indicator can affect the prediction results.

\vspace{-0.1 in}

\subsubsection{Performance Evaluation}
We evaluate the methods on predicting septic shock by calculating various evaluation metrics including accuracy, recall, precision, $F_1$ score (F1), and area under ROC curve (AUC) obtained from 5-fold cross-validation. Accuracy is the proportion of correctly classified visits over all visits. Recall is the proportion of correctly identified positive visits over all visits that actually have septic shock. Precision is the proportion of correctly identified positive visits over all visits that are identified as positive. F1 is the harmonic mean of the precision and recall. AUC calculates the trade-off between recall and specificity, where specificity is the proportion of correctly identified negative visits over all visits that are identified as negative.

\vspace{-0.1 in}

\subsection{Baselines}
We employ 3 state-of-the-art baselines and 1 expert baseline. The state-of-the-art baselines are 3D-MICE \cite{luo20183d}, sampling-based MICE \cite{buuren2010mice}, and GP with RBF kernel. We also employ an expert baseline which is defined by the domain experts and has been adopted in previous research \cite{kim2018temporal}. The expert baseline fills the missing values with the last value within a fixed length window (i.e. 24 hours for lab analytes and 8 hours for vital signs), and fills the remains with the mean value of the corresponding measurements. The expert baseline performs better in clinical data imputation and prediction compared to traditional baselines (e.g. mean/median, carry forward, etc.) in both previous \cite{kim2018temporal} and our work, thus we don't present the results of traditional baselines here. For fair comparison, we adopt the same experimental settings for baselines as our model. 

\begin{table*}[h!]
% \label{tab:pred}
\centering
\caption{Septic Shock Prediction Performance (mean$\pm$ std) by Imputation Method on CCHS and Mayo.}
\label{tab:pred}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{l|lllll|lllll}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{CCHS}                                                                                                                                       & \multicolumn{5}{c}{Mayo}                                                                                                \\ \cline{2-11} 
                        & \multicolumn{1}{c}{Accuracy}        & \multicolumn{1}{c}{Recall}          & \multicolumn{1}{c}{Precision}       & \multicolumn{1}{c}{F1}              & \multicolumn{1}{c|}{AUC}            & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC}    \\ \hline
Expert                  &         .691$\pm$.027                            &     .685$\pm$.039                                &       .716$\pm$.044**                              &        .698$\pm$.044                             &     .744$\pm$.023                                &        .808$\pm$.009**                      &         .815$\pm$.019                   &     \textbf{.797$\pm$.018}                          &         .806$\pm$.018**                   &   .879$\pm$.009**                         \\
GP                      & .700$\pm$.017**           & .703$\pm$.042          & .703$\pm$.027          & .702$\pm$.027**          & .757$\pm$.011          &           .803$\pm$.009                   &    .819$\pm$.021**                        &       .779$\pm$.020                        &    .798$\pm$.020                        &          .877$\pm$.007                  \\
MICE                    & .689$\pm$.020          & .686$\pm$.026          & .701$\pm$.032          & .693$\pm$.032          & .743$\pm$.015          & .788$\pm$.013   & .804$\pm$.014 & .760$\pm$.023    & .781$\pm$.023 & .865$\pm$.018 \\
3D-MICE                 & .697$\pm$.012          & .706$\pm$.042**          & .684$\pm$.037          & .693$\pm$.037          & .768$\pm$.016**          & .794$\pm$.011   & .806$\pm$.037 & .776$\pm$.024    & .790$\pm$.024 & .876$\pm$.010 \\
3M-MICE                 & \textbf{.717$\pm$.019}          & \textbf{.711$\pm$.034}          & \textbf{.729$\pm$.022}          & \textbf{.720$\pm$.022}          & \textbf{.777$\pm$.016}          & \textbf{.812$\pm$.006}   & \textbf{824$\pm$.009} & \.795$\pm$.006**   & \textbf{.809$\pm$.006} & \textbf{.889$\pm$.007} \\ \hline

Expert+MI               &       .736$\pm$.019                              &    .742$\pm$.047                                 &      .730$\pm$.036                               &        .734$\pm$.036                             &      .790$\pm$.008                               &                 \textbf{.842$\pm$.024}             &          .838$\pm$.026**                  &      \textbf{.846$\pm$.042}                         &    \textbf{.842$\pm$.042}                        &    \textbf{.915$\pm$.014}                        \\
GP+MI                   & .730$\pm$.012          & .731$\pm$.021          & .727$\pm$.026          & .729$\pm$.026          & .788$\pm$.016          &          .826$\pm$.016                    &    .823$\pm$.030                        &        .831$\pm$.015                       &   .827$\pm$.015                         &        .906$\pm$.012**                   \\
MICE+MI                 & .739$\pm$.011          & .739$\pm$.026          & .739$\pm$.015          & .739$\pm$.015          & .792$\pm$.003          & .809$\pm$.018   & .816$\pm$.025 & .795$\pm$.023    & .806$\pm$.023 & .890$\pm$.012 \\
3D-MICE+MI              & .746$\pm$.028**          & .748$\pm$.045**          & .742$\pm$.028**          & .745$\pm$.028**          & .809$\pm$.022**          & .830$\pm$.011   & .828$\pm$.015 & .834$\pm$.017**    & .831$\pm$.017 & .899$\pm$.008 \\
3M-MICE+MI              & \textbf{.754$\pm$.012} & \textbf{.758$\pm$.031} & \textbf{.748$\pm$.021} & \textbf{.752$\pm$.021} & \textbf{.814$\pm$.012} & .834$\pm$.007**   & \textbf{.841$\pm$.011} & .824$\pm$.018    & .832$\pm$.018** & .905$\pm$.006 \\ \hline
\end{tabular}
\begin{tablenotes}
      \small
      \item - The best and the second-best performance are labeled with \textbf{bold} and **.
      \item +MI: The method is combined with missing indicators.
    \end{tablenotes}
\end{threeparttable}
}
\vspace{-0.1 in}
\end{table*}



\noindent\textbf{Implementation Details:}
All experiments are conducted on a 12-core machine. We use 1 iteration on multiple imputation with MICE R package \cite{buuren2010mice} for 3M-MICE, 3D-MICE, and MICE methods, and  $\alpha=0.02$ on RBF kernel with GP \cite{rasmussen2003gaussian}. In 2-step MICE, we assign $0.5$ to both $w_{11}$ and $w_{12}$ to ensure the fairness and balance the effect of MICE through cross-sectional and longitudinal view. For LSTM, we use 1 hidden layer with 128 hidden neurons, 0.005 initial learning rate, and 200 maximum sequence-length. We adopt Adam optimizer \cite{kingma2014adam} with 64 batches and 25 epochs.

==> sections/prelim.tex <==

\begin{definition}[\textbf{Multivariate Time Series Clinical Data}]
\label{def:data}


\textit{
A multivariate time series clinical data can be represented as  $\mathbf{X} = \{\mathbf{X_1}, ..., \mathbf{X_N}\}$, where $N$ is the total number of hospital visits. Each visit $\mathbf{X_i}$ consists of a sequence of events: $\mathbf{X_i} = \{\mathbf{{X}}_{i, 1, \cdot},..., \mathbf{{X}}_{i, t_i, \cdot}\}$ where $\mathbf{{X}}_{i, j, \cdot}$ represents a patient $i$'s record at time step $j$ in $\mathbf{X_i}$ and $t_i$ is number of events in visit $i$ which can vary across different visits. Specifically, $\mathbf{{X}}_{i, j, \cdot}\in\mathbb{R}^D$, where $D$ is the number of features recorded. Each visit $i$ is also associated with a vector $\mathbf{\Delta t}_i\in\mathbb{R}^{t_i}$ recording the time interval (e.g., minutes) from a starting point (e.g., patient arrival time) till when each event occur. Moreover, $\mathbf{X_i}$ satisfies the condition that events are ordered increasingly according to time steps. 
}
\end{definition}


\begin{definition}[\textbf{Native and Masked Missing Values}]
\textit{
In practice, $\mathbf{X}_i$ may contain native missing values without groundtruth due to the irregular data collection process. To evaluate imputation performance, we apply additional masks to the observed data which introduce masked missing values with known grondtruth.
}
\end{definition}

\noindent\textit{Problem Statement.} \textbf{Multivariate Time Series Clinical Data Imputation.} Given a multivariate time series clinical data $\mathbf{X} = \{\mathbf{X_1}, ...,$ $\mathbf{X_N}\}$, which contain missing values, with the corresponding time-interval vectors $\mathbf{\Delta t}=\{\mathbf{\Delta t}_1,...,\mathbf{\Delta t}_N\}$, devise an imputation model $f$ which outputs complete multivariate time series $\mathbf{\hat{X}}$: $\mathbf{\hat{X}} = f(\mathbf{X}, \mathbf{\Delta t})$.


==> sections/result.tex <==


%%%% imputation result: MIMIC-III




% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.6]{sections/figure/ave-nrmse.png}
%     \caption{Imputation accuracy (average nRMSE) for the MIMIC-III dataset}
%     \label{fig:ave-nrmse}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.27]{sections/figure/scatter-hct.png}
%     \caption{Accuracy of Hematocrit predictions and prediction intervals width, scatter plot; Horizontal and vertical lines: normal reference limits; The less accurate predictions, the bluer color of the points}
%     \label{fig:hema}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.27]{sections/figure/scatter-hgb.png}
%     \caption{Hemoglobin}
%     \label{fig:hemo}
% \end{figure}




In this section, we compare the imputation performance of our proposed 3M-MICE approach against various baselines in two experimental settings: First, we evaluate the effectiveness of each model in imputation of the masked values by varying the masking ratio in terms of nRMSE. Second, we investigate the ability of 3M-MICE in capturing rich correlations among longitudinal and cross-sectional information in clinical data by assessing the performance of a prediction model trained on the imputed data generated by each algorithm.

\vspace{-0.1 in}

\subsection{Various Masking Rates on Observations}
In this setting, \textit{nRMSE} is used to evaluate the imputation of masked observations. We compare our approach to 4 baselines on one real-world data, MIMIC-III, with 6 masking rates. The results \footnote{Numeric results of nRMSE are attached in supplementary} in Fig.\ref{fig:nrmse} show that our imputation model outperforms the baselines with smaller nRMSE on each measurement and overall data across all masking rates. Specifically, our model is more capable with high masking rates (e.g., 90\%) with an average 0.227 nRMSE across measurements, which is 13\% better than 3D-MICE (i.e., 0.261), 23\% better than MICE (i.e., 0.296), 21\% better than GP (i.e., 0.288), and 18\% better than expert baseline (i.e., 0.278). 
%Also, from the Fig.\ref{fig:nrmse}, our model is more stable with increasing masking rates above 50\% masking rates with average nRMSE 

\vspace{-0.1 in}

\subsection{Septic Shock Early Prediction}
In this setting, evaluation metrics are used to evaluate the performance of each model for prediction of septic shock 8 hours before the onset on 2 real-world EHR datasets: CCHS and Mayo. We compare our approach against four imputation baselines and in two settings: with or without missing indicators (MI). The results in Table.\ref{tab:pred} show that 3M-MICE outperforms all the baselines in both experimental settings by achieving the highest accuracy, recall, precision, F1, and AUC on CCHS dataset, and outperforms all baselines be achieving highest accuracy, recall, F1, and AUC without missing indicator on Mayo dataset. Specifically, 3M-MICE always performs better on recall, which means it less miss-identifies shock positive patients as negative, while false negative can be costly in practice. This result further demonstrates the importance of capturing rich correlations among both longitudinal and cross-sectional information and the effectiveness of 3M-MICE in imputing missing values to prepare data for building complex prediction models.





==> sections/table/char.tex <==

\begin{table}[tbp]
 \scriptsize
\centering
\begin{threeparttable}
\caption{Missing Rates of Selected Measurement across Three Datasets}
\label{table:char}
\begin{subtable}{0.50\textwidth}
\begin{tabular}{l|lcc}
\hline
Lab Analytes & ItemID & OMR   & PMR   \\ \hline
Chloride   & 50902  & 0.258 & 0.022 \\
Potassium  & 50971  & 0.210 & 0.020 \\
Bicarb     & 50882  & 0.271 & 0.025 \\
Sodium     & 50983  & 0.244 & 0.021 \\
Hematocrit & 51221  & 0.181 & 0.116 \\
Hemoglobin & 51222  & 0.304 & 0.138 \\
MCV        & 51250  & 0.308 & 0.140 \\
Platelet   & 51265  & 0.279 & 0.134 \\
WBC        & 51301  & 0.303 & 0.136 \\
RDW        & 51277  & 0.309 & 0.000 \\
BUN        & 51006  & 0.259 & 0.000 \\
Creatinine & 50912  & 0.253 & 0.000 \\
Glucose    & 50931  & 0.297 & 0.000 \\ \hline
\end{tabular}
\caption{\footnotesize (MIMIC-III)}
\label{tab:char-mimic}
\end{subtable}

\begin{subtable}{0.48\textwidth}
\begin{tabular}{l|ll|ll}
\hline
\multirow{2}{*}{Vital Signs} & \multicolumn{2}{l|}{CCHS} & \multicolumn{2}{l}{Mayo} \\ \cline{2-5} 
                            & OMR         & PMR         & OMR         & PMR        \\ \hline
Temperature                 & 0.739       & 0.633       & 0.910       & 0.706      \\
FiO2                        & 0.663       & 0.467       & 0.940       & 0.739      \\
MAP                         & 0.660       & 0.544       & 0.632       & 0.349      \\
DiastolicBP                 & 0.658       & 0.544       & 0.632       & 0.349      \\
SystolicBP                  & 0.658       & 0.543       & 0.632       & 0.348      \\
PulseOx                     & 0.536       & 0.283       & 0.339       & 0.143      \\
RespiratoryRate             & 0.519       & 0.272       & 0.489       & 0.288      \\
HeartRate                   & 0.484       & 0.237       & 0.235       & 0.038      \\
OxygenFlow                  & 0.777       & 0.112       & 0.974       & 0.083      \\ \hline
\end{tabular}
\caption{\footnotesize (CCHS\&Mayo)}
\label{tab:char-cchs&mayo}
\end{subtable}

\begin{tablenotes}
      \scriptsize
      \item Item ID: Identification code of measurements, which is specific to MIMIC-III.
      \item NMR: Native missing rate.
      \item PMR: Missing rate after applying exclusion and preprocessing criteria.
    \end{tablenotes}
\end{threeparttable}
\vspace{-0.2 in}
\end{table}

% \begin{table}[tbp]
% \caption{Extracted Measurements from MIMIC-III Dataset. The Item ID Represents The Identification Code of A Measurement in MIMIC-III.}
% \label{table:char}
% \begin{tabular}{lcc}
% \hline
% \multicolumn{1}{l}{Measurements}       & \multicolumn{1}{c}{Item IDs} & Missing Rates \\ \hline
% Chloride                                & 50902                        & 0.258        \\
% Potassium                               & 50971                        & 0.210        \\
% Bicarb                                  & 50882                        & 0.271        \\
% Sodium                                  & 50983                        & 0.244        \\
% Hematocrit                              & 51221                        & 0.181        \\
% Hemoglobin                              & 51222                        & 0.304        \\
% Mean corpuscular volume (MCV)           & 51250                        & 0.308        \\
% Platelet Count                          & 51240                        & 0.279        \\
% White blood cells (WBC)                 & 51301                        & 0.303        \\
% Red blood cell distribution width (RDW) & 51277                        & 0.309        \\
% Blood urea nitrogen (BUN)               & 51006                        & 0.259        \\
% Creatinine                              & 50912                        & 0.253        \\
% Glucose                                 & 50931                        & 0.297        \\ \hline
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \begin{table*}[tbp]
% \centering
% \begin{threeparttable}
% \caption{Extracted Categories and Measurements from MIMIC-III, CCHS, and Mayo Datasets. The Item ID Represents The Identification Code of A Measurement in MIMIC-III.}
% \label{table:char}
% \begin{tabular}{l|lc|ccc}
% \hline
% \multirow{2}{*}{Category}     & \multirow{2}{*}{Measurement}            & \multirow{2}{*}{Item ID} & \multicolumn{3}{c|}{Missing Rate}                                                   \\ \cline{4-6} 
%                               &                                         &                          & \multicolumn{1}{l}{MIMIC-III} & \multicolumn{1}{l}{CCHS} & \multicolumn{1}{l}{Mayo} \\ \hline
% \multirow{15}{*}{Lab results} & Chloride                                & 50902                    & 0.258                         & X                        & -                        \\
%                               & Potassium                               & 50971                    & 0.210                         & X                        & -                        \\
%                               & Bicarb                                  & 50882                    & 0.271                         & X                        & X                        \\
%                               & Sodium                                  & 50983                    & 0.244                         & X                        & -                        \\
%                               & Hematocrit                              & 51221                    & 0.181                         & X                        & X                        \\
%                               & Hemoglobin                              & 51222                    & 0.304                         & X                        & -                        \\
%                               & Mean corpuscular volume (MCV)           & 51250                    & 0.308                         & X                        & -                        \\
%                               & Platelet Count                          & 51240                    & 0.279                         & 0.934                    & -                        \\
%                               & White Blood Cells (WBC)                 & 51301                    & 0.303                         & 0.935                    & -                        \\
%                               & Red blood cell distribution width (RDW) & 51277                    & 0.309                         & X                        & X                        \\
%                               & Blood urea nitrogen (BUN)               & 51006                    & 0.259                         & 0.933                    & -                        \\
%                               & Creatinine                              & 50912                    & 0.253                         & 0.933                    & -                        \\
%                               & Glucose                                 & 50931                    & 0.297                         & X                        & -                        \\
%                               & Bilirubin                               & \multicolumn{1}{l|}{}    & -                             & 0.979                    & -                        \\
%                               & Lactate                                 & \multicolumn{1}{l|}{}    & -                             & 0.972                    & -                        \\ \hline
% \multirow{7}{*}{Vital signs}  & Temperature                             & \multicolumn{1}{l|}{}    & -                             & 0.813                    & 0.889                    \\
%                               & Mean arterial pressure (MAP)            & \multicolumn{1}{l|}{}    & -                             & 0.774                    & 0.674                    \\
%                               & Diastolic blood pressure (DBP)          & \multicolumn{1}{l|}{}    & -                             & 0.721                    & 0.674                    \\
%                               & Systolic blood pressure (SBP)           & \multicolumn{1}{l|}{}    & -                             & 0.720                    & 0.674                    \\
%                               & Pulse oximetry (PulseOx)                & \multicolumn{1}{l|}{}    & -                             & 0.637                    & 0.342                    \\
%                               & Respiratory rate                        & \multicolumn{1}{l|}{}    & -                             & 0.626                    & 0.535                    \\
%                               & Heart rate                              & \multicolumn{1}{l|}{}    & -                             & 0.606                    & 0.211                    \\ \hline
% \end{tabular}
% \begin{tablenotes}
%       \small
%       \item -: the dataset contained the measurement but we didn't use it in our study. \\
%       X: the dataset didn't contain the measurement.
%     \end{tablenotes}
% \end{threeparttable}
% \end{table*}

==> sections/table/pred.tex <==
\begin{table*}[tbp]
\label{tab:pred}
\centering
\caption{Septic Shock 24-Hour Early Prediction Performance (mean$\pm$std) on CCHS Data.}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{l|lllll|lllll}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{Original}                                                                                                                                       & \multicolumn{5}{c}{+MI}                                                                                                \\ \cline{2-11} 
                        & \multicolumn{1}{c}{Accuracy}        & \multicolumn{1}{c}{Precision}          & \multicolumn{1}{c}{Recall}       & \multicolumn{1}{c}{F1}              & \multicolumn{1}{c|}{AUC}            & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC}    \\ \hline
Expert                  &         .691$\pm$.027                            &     .685$\pm$.039                                &       .716$\pm$.044                              &        .698$\pm$.044                             &     .744$\pm$.023                                &        .808$\pm$.009                      &         .815$\pm$.019                   &     \textbf{.797$\pm$.018}                          &         .806$\pm$.018                   &   .879$\pm$.009                         \\
GP                      & .700$\pm$.017           & .703$\pm$.042          & .703$\pm$.027          & .702$\pm$.027          & .757$\pm$.011          &           .803$\pm$.009                   &    .819$\pm$.021                        &       .779$\pm$.020                        &    .798$\pm$.020                        &          .877$\pm$.007                  \\
MICE                    & .689$\pm$.020          & .686$\pm$.026          & .701$\pm$.032          & .693$\pm$.032          & .743$\pm$.015          & .788$\pm$.013   & .804$\pm$.014 & .760$\pm$.023    & .781$\pm$.023 & .865$\pm$.018 \\
3D-MICE                 & .697$\pm$.012          & .706$\pm$.042          & .684$\pm$.037          & .693$\pm$.037          & .768$\pm$.016          & .794$\pm$.011   & .806$\pm$.037 & .776$\pm$.024    & .790$\pm$.024 & .876$\pm$.010 \\
3M-MICE                 & \textbf{.717$\pm$.019}          & \textbf{.711$\pm$.034}          & \textbf{.729$\pm$.022}          & \textbf{.720$\pm$.022}          & \textbf{.777$\pm$.016}          & \textbf{.812$\pm$.006}   & \textbf{824$\pm$.009} & \.795$\pm$.006   & \textbf{.809$\pm$.006} & \textbf{.889$\pm$.007} \\ \hline
Expert+MI               &       .736$\pm$.019                              &    .742$\pm$.047                                 &      .730$\pm$.036                               &        .734$\pm$.036                             &      .790$\pm$.008                               &                 \textbf{.842$\pm$.024}             &          .838$\pm$.026                  &      \textbf{.846$\pm$.042}                         &    \textbf{.842$\pm$.042}                        &    \textbf{.915$\pm$.014}                        \\
GP+MI                   & .730$\pm$.012          & .731$\pm$.021          & .727$\pm$.026          & .729$\pm$.026          & .788$\pm$.016          &          .826$\pm$.016                    &    .823$\pm$.030                        &        .831$\pm$.015                       &   .827$\pm$.015                         &        .906$\pm$.012                   \\
MICE+MI                 & .739$\pm$.011          & .739$\pm$.026          & .739$\pm$.015          & .739$\pm$.015          & .792$\pm$.003          & .809$\pm$.018   & .816$\pm$.025 & .795$\pm$.023    & .806$\pm$.023 & .890$\pm$.012 \\
3D-MICE+MI              & .746$\pm$.028          & .748$\pm$.045          & .742$\pm$.028          & .745$\pm$.028          & .809$\pm$.022          & .830$\pm$.011   & .828$\pm$.015 & .834$\pm$.017    & .831$\pm$.017 & .899$\pm$.008 \\
3M-MICE+MI              & \textbf{.754$\pm$.012} & \textbf{.758$\pm$.031} & \textbf{.748$\pm$.021} & \textbf{.752$\pm$.021} & \textbf{.814$\pm$.012} & .834$\pm$.007   & \textbf{.841$\pm$.011} & .824$\pm$.018    & .832$\pm$.018 & .905$\pm$.006 \\ \hline
\end{tabular}
\begin{tablenotes}
      \small
      \item - The bold number represents the best performance.
      \item +MI: The method is combined with missing indicators.
      \item - DETROIT and CATSI cannot be implemented properly due to its intrinsic limitation taking fixed-size non-missing inputs.
    \end{tablenotes}
\end{threeparttable}
}
\vspace{-0.1 in}
\end{table*}
